A Spectral Representation of Power Systems with Applications to Adaptive Grid Partitioning and Cascading Failure Localization

Transmission line failures in power systems propagate and cascade non-locally. This well-known yet counter-intuitive feature makes it even more challenging to optimally and reliably operate these complex networks. In this work we present a comprehensive framework based on spectral graph theory that fully and rigorously captures how multiple simultaneous line failures propagate, distinguishing between non-cut and cut set outages. Using this spectral representation of power systems, we identify the crucial graph sub-structure that ensures line failure localization -- the network bridge-block decomposition. Leveraging this theory, we propose an adaptive network topology reconfiguration paradigm that uses a two-stage algorithm where the first stage aims to identify optimal clusters using the notion of network modularity and the second stage refines the clusters by means of optimal line switching actions. Our proposed methodology is illustrated using extensive numerical examples on standard IEEE networks and we discussed several extensions and variants of the proposed algorithm.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

A finer-grained tree-partition of the power grid creates more, smaller management regions whose operations can be isolated from each other in various aspects, bringing benefits such as disruption localizability, optimization parallelization, and more to the control and management of power systems. In this section, we present a collection of examples on how tree-partitions offer powerful analytical guarantees in different scenarios, and how we can leverage these properties to improve current practices in these situations.

{\color{green} [Adam: list the applications briefly here]}

\subsection{Real-time Failure Mitigation with Unified Controller}
Reliability is a crucial part for the development of sustainable modern power systems. Cascading failures, which are common in high voltage systems, have become the major threats to the grid reliability. Recent blackouts, for example, the 2003 and 2012 blackouts in Northwestern America and India, demonstrate the devastating economic and societal impact that a grid failure can incur. 

Cascading failures exhibit a complicated, non-local propagation pattern in power systems, which originates from the interplay between network topology and power flow physics. Such complexity, makes the analysis and mitigation for failures difficult. In particular, the design of distributed controller to reliably prevent and mitigate failures is open \lguo{this seems a slightly agressive claim to me...}.

Current industry practice mainly relies on simulation based failure analysis, where a subset of possible contingencies are simulated to establish a safe operating level to avoid cascading failures. However, this method is often limited by the computation power, thus it is not suitable for large scale networks. Furthermore, it is a preventive method, thus cannot provide real-time failure mitigation. Such drawbacks are further aggravated with the uncertainty introduced by the increasing penetration of renewable. 

The limitations of industry practice have motivated the analytical study and characterization of failure propagation in power systems. These approaches can be classified into roughly three categories: (i) using Monte-Carlo methods to analyze steady state power flow redistribution with DC (\cite{carreras2002critical,anghel2007stochastic,yan2015cascading,bernstein2014power}) and AC (\cite{nedic2006criticality,rios2002value,song2016dynamic}) model; (ii) applying pure topological models with simplified assumptions (e.g., failures propagate to adjacent components with high probability) to cascading dynamics, and inferring propagation patterns from graph-theoretic perspective (\cite{brummitt2003cascade,kong2010failure,crucitti2004topological}); (iii) investigating statistical propagation dynamics from historical or synthetic failure data (\cite{dobson2005probilistic,wang2012markov,rahnamay2014stochastic,hines2017cascading}).  In all of these approaches, however, the non-local failure propagation pattern often poses challenges for the inference and control of cascading failures.

A new approach has been proposed in recent years, which adopts the tree-partition properties for failure localization in \cite{Guo2018}. As introduced in Section~\ref{sec:tree}, a fine tree-partition leads to clear and well-defined boundaries through cells that isolate failures. This suggests \lguo{a new failure mitigation approach} to switch off certain transmission lines carefully for finer tree-partition and thus \lguo{exhibits} better failure localization property. Unfortunately, this method has failed to localize bridge failures, as well as to prevent successive failures from happening.

\cite{Guo2019} further proposed a distributed control strategy, which combines frequency control and tree-partition to offer strong failure mitigation and localization properties. It adopts a recent design in frequency regulation literature, the Unified Controller (UC) \cite{zhao2016unified} that achieves primary frequency contorl, secondary frequency control and congestion management simultaneously at the frequency regulation timescale. Such controller, together with the tree-partition, is guaranteed to (i) always prevent successive failures from happening; (ii) localize the impact of initial failures as much as possible.

In the rest of this section, we will review the aforementioned distributed control strategy proposed in \cite{Guo2019} and evaluate its performance over a large power network, i.e. the Polish 2736sp network.

\subsubsection{Frequency Regulation and the Unified Controller}

%\lguo{I feel we can move details of UC to appendix and emphasize more on the cascading failure aspect here?}
Frequency regulation balances the power generation and consumption in an electric grid. Such control is governed by the swing dynamics and is traditionally implemented in generators through droop control, automatic generation control and economic dispatch. In recent years, it has been widely realized in the community that the ubiquitous fast-acting distributed load-side frequency regulation is needed and becomes realizable since more and more ``grid-friendly" devices such as refrigerators, air conditioners, and plug-in electrical vehicles can help to participate in regulating the power imbalance. 

The Unified Controller (UC) is a distributed control framework recently proposed in \cite{zhao2016unified}. It is designed so that the closed-loop control system evolves as a projected primal-dual algorithm to solve the optimization problem~\eqref{eqn:uc_olc}, where the control cost is minimized to restore the nominal frequency~\eqref{eqn:uc_balance},\eqref{eqn:dcflow}, restore the inter-area flows~\eqref{eqn:uc_ace} and maintain safe branch flows~\eqref{eqn:line_limit} and generations~\eqref{eqn:control_limit}. If \eqref{eqn:uc_olc} is feasible, under mild conditions, UC is guaranteed to converge to the optimal point. Interested readers are referred to \cite{zhao2016unified} for the details of UC.
\begin{subequations}\label{eqn:uc_olc}
\begin{eqnarray}
\min_{f, d, \theta} & \quad& \sum_{j\in\calN}c_j(d_j) \label{eqn:uc_obj}\\
\text{s.t.} & &r - d - Cf = 0 \label{eqn:uc_balance}\\
& &f = BC^T\theta  \label{eqn:dcflow}\\
& &ECf = 0\label{eqn:uc_ace}\\
& &\ul{f}_{e}\le f_{e}\le \ol{f}_{e}, \quad e\in\calE \label{eqn:line_limit}\\
& &\ul{d}_{j}\le d_j\le \ol{d}_j, \quad j \in\calN \label{eqn:control_limit}
\end{eqnarray}
\end{subequations}

UC is designed to rebalance the power and restore nominal frequency against power injection disturbances \lguo{and has been extensively investigated in the frequency regulation literature. It is first reported in \cite{Guo2019} that...}, however, it is first introduced in \cite{Guo2019} that such framework turns out to be quite powerful for failure mitigation and localization. The key idea for the proposed strategy is to implement UC over the regions defined by a tree-partition of the network. To be more specific, the control strategy consists of two phases: in planning phase, the control areas for UC should be created so that a tree structure is formed; in operating phase, UC actively monitors and reacts to failures and disturbances.

During the planning phase, the goal is to create a finer tree-partition, and coincide the control areas of UC and the regions defined by the tree-partition. We could use the approaches described in Section~\ref{sec:optimization} to refine the tree-partition without affecting the operational condition significantly.

During the operating phase, UC operates as a real-time controller against contingencies as shown in Fig.~\ref{fig:flow_chart}. After an initial failure happens, UC tries to drive the system back to an equilibrium point which is an optimal solution of \eqref{eqn:uc_olc}. If \eqref{eqn:uc_olc} is not feasible, however, UC becomes unstable, indicating it is impossible to achieve all the control objectives after such failure. Certain constraints in \eqref{eqn:uc_olc} will then be lifted to stabilize the system. There are two ways to do so: (i) involving more control areas to participate in the failure mitigation process by lifting the zero area control error constraints \eqref{eqn:uc_ace} or (ii) allowing load shedding by enlarging the range $[\ul{d}_{j}, \ol{d}_j]$ for the corresponding load buses \eqref{eqn:control_limit}. 
\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{flow_chart}
\caption{Flowchart of the events after an initial failure under the proposed control strategy.}\label{fig:flow_chart}
\end{figure}

\subsubsection{Evaluation of Proposed Control Strategy}
We now evaluate the performance of the above control strategy over the Polish 2736sp network against failures. We first perform the aforementioned pruning methods \lguo{which pruning method?} to switch off 78 transmission lines for a partition of 4 regions, with sizes 1430, 818, 359 and 125. After switching off the lines, the maximal congestion level increases from 97.67\% to 97.81\%. This verifies\lguo{corroborates} our claim that the system congestion level will not significantly increase by carefully selecting lines to switch off.

%\lguo{Do we want to have a separate section specifically for numerical results? If we mention case studies here then we probably need similar experiments for all the remaining examples, which we may not have....}
The system robustness against failures is then evaluated in terms of the $N-1$ security standard. We iterate over every transmission line as the initial failure and simulate the cascading process thus triggered. To understand the robustness under different system congestion levels, we further scale down the line capacity by a factor $\alpha$ \lguo{that takes values} 95\%, 90\%, 85\% and 80\% (for those lines with flow exceeding the rescaled capacity, we reset their capacity as the absolute flow value) and repeat the simulation \lguo{for each of these $\alpha$}. This produces about 15,000 failure scenarios. 

Table~\ref{table:failure_case} illustrates the percentage of failures that can be mitigated with different levels of constraint lifting and the average load loss when load shedding is needed, under five congestion levels indicated by the line capacity factor $\alpha$. One can see there is a monotone behavior with respect to the congestion level. As the system becomes more congested, more failures will require the participation of other regions and even load shedding to prevent further failures. However, even when the congestion level is relatively high, more than 60\% single line failures can be mitigated and localized within the region itself. Moreover, the average load loss (30-50) is fairly small compared to the overall load demand ($1.8\times 10^4$). 

Fig.~\ref{fig:gen_dist} demonstrates the distribution for the number of regions where the generators are adjusted for failure mitigation with different levels of congestion. Similar monotone behavior is observed. As congestion level increases, more generator adjustments are needed to mitigate the failures. When the congestion level is low ($\alpha = 1$), one can see that more than 70\% single line failures can be localized without any generation adjustment, which indicates that the traditional industry practice such as droop control also works. However, as congestion level increases, more and more failures will require generation adjustments to stabilize the system. Thus, UC outperforms droop control and allows larger safe operational margins to achieve a better economical impact.

\chen{More detailed descriptions for the experiment? } {\color{green} [Adam: yes, maybe a little more is needed]}

\begin{table}[!h]
\centering
\begin{tabular}{p{2cm}|p{2.6cm}|p{3.5cm}|p{3cm}|p{2.2cm}}
Line capacity factor & failures mitigated within 1 region & failures mitigated with multiple regions & failures mitigated with load shedding& Average load loss \\
\hline \hline
0.8 & 63.27\% & 32.07\% & 4.66\% & 52.40 \\
\hline
0.85 & 72.17\% & 24.43\% & 3.40\% & 43.58 \\
\hline
0.9 & 73.77\% & 23.27\% & 2.96\% & 38.03 \\
\hline
0.95 & 85.25\% & 13.21\% & 1.54\% & 36.70 \\
\hline
1 & 90.57\% & 8.37\% & 1.07\% & 34.59
\end{tabular}
\caption{Distribution for the failures that can be mitigated with different levels of constraint lifting.}
\label{table:failure_case}
\end{table}

\begin{figure}
\centering
\input{gen_dist.tex}
\caption{Distribution for the number of regions that generators are adjusted. ``0" indicates that no generator adjustment is need.}
\label{fig:gen_dist}
\end{figure}


\subsection{Distributed AC OPF}
Introduce the SDP relaxation.

Introduce a few sufficient condition, and argue that these conditions are way easier to be satisfied with tree-partitions.

If the regions are chordal, then the $V\succeq 0$ condition can be equivalently solved separately by each region.

Argue that the method generalize to 3-phase Y-connected systems.

\subsection{SCOPF and Market}

\subsubsection{Tractable Market Price Manipulation}
Introduce the dynamical programming based method to solve the largest market price manipulation power.

Show that by having a tree-partition, assuming solving the sub-problem in each region is bounded by a constant (hopefully not too large if the graph is small), then we can generalize the above result to broader class of graphs.

\subsubsection{Accelerated Security-constrained OPF}
Security constrained OPF augments the conventional OPF by adding a set of contingencies and require the operating point to be safe under any of such contingency. This is usually achieved via the following:

Describe the two-step industry practice.

We now show that with a tree-partition, step 2 of the above can be significantly accelerated.

Describe a tree-partition based distributed solver for OPF.

Further, tree-partition induces a natural way to decompose this SCOPF problem. Compared to direct ADMM based method, this proposed method reduces the number of constraints and variables in each region by $O(k^2)$, and also decrease the number of messages necessary to pass across the agents by $O(k)$. As a result, the time for each agent to solve the local version of optimization is reduced by $O(k^6)$ (assume $O(N^3)$ complexity of LP solver) and the overall communication overhead is reduced by $O(k)$. From the simulation results, our method also reduces the number of iterations for convergence.

%\subsection{SLS for Frequency Regulation Controller Synthesis}
%It seems tree-partition allows easier synthesis of distributed controllers via SLS?

==> arxiv submission/applications.tex <==
\section{Applications}
\label{sec:applications}

A finer-grained tree-partition of the power grid creates more, smaller management regions whose operations can be isolated from each other in various aspects, bringing benefits such as disruption localizability, optimization parallelization, and more to the control and management of power systems. In this section, we present a collection of examples on how tree-partitions offer powerful analytical guarantees in different scenarios, and how we can leverage these properties to improve current practices in these situations.

{\color{green} [Adam: list the applications briefly here]}

\subsection{Real-time Failure Mitigation with Unified Controller}
Reliability is a crucial part for the development of sustainable modern power systems. Cascading failures, which are common in high voltage systems, have become the major threats to the grid reliability. Recent blackouts, for example, the 2003 and 2012 blackouts in Northwestern America and India, demonstrate the devastating economic and societal impact that a grid failure can incur. 

Cascading failures exhibit a complicated, non-local propagation pattern in power systems, which originates from the interplay between network topology and power flow physics. Such complexity, makes the analysis and mitigation for failures difficult. In particular, the design of distributed controller to reliably prevent and mitigate failures is open \lguo{this seems a slightly agressive claim to me...}.

Current industry practice mainly relies on simulation based failure analysis, where a subset of possible contingencies are simulated to establish a safe operating level to avoid cascading failures. However, this method is often limited by the computation power, thus it is not suitable for large scale networks. Furthermore, it is a preventive method, thus cannot provide real-time failure mitigation. Such drawbacks are further aggravated with the uncertainty introduced by the increasing penetration of renewable. 

The limitations of industry practice have motivated the analytical study and characterization of failure propagation in power systems. These approaches can be classified into roughly three categories: (i) using Monte-Carlo methods to analyze steady state power flow redistribution with DC (\cite{carreras2002critical,anghel2007stochastic,yan2015cascading,bernstein2014power}) and AC (\cite{nedic2006criticality,rios2002value,song2016dynamic}) model; (ii) applying pure topological models with simplified assumptions (e.g., failures propagate to adjacent components with high probability) to cascading dynamics, and inferring propagation patterns from graph-theoretic perspective (\cite{brummitt2003cascade,kong2010failure,crucitti2004topological}); (iii) investigating statistical propagation dynamics from historical or synthetic failure data (\cite{dobson2005probilistic,wang2012markov,rahnamay2014stochastic,hines2017cascading}).  In all of these approaches, however, the non-local failure propagation pattern often poses challenges for the inference and control of cascading failures.

A new approach has been proposed in recent years, which adopts the tree-partition properties for failure localization in \cite{Guo2018}. As introduced in Section~\ref{sec:tree}, a fine tree-partition leads to clear and well-defined boundaries through cells that isolate failures. This suggests \lguo{a new failure mitigation approach} to switch off certain transmission lines carefully for finer tree-partition and thus \lguo{exhibits} better failure localization property. Unfortunately, this method has failed to localize bridge failures, as well as to prevent successive failures from happening.

\cite{Guo2019} further proposed a distributed control strategy, which combines frequency control and tree-partition to offer strong failure mitigation and localization properties. It adopts a recent design in frequency regulation literature, the Unified Controller (UC) \cite{zhao2016unified} that achieves primary frequency contorl, secondary frequency control and congestion management simultaneously at the frequency regulation timescale. Such controller, together with the tree-partition, is guaranteed to (i) always prevent successive failures from happening; (ii) localize the impact of initial failures as much as possible.

In the rest of this section, we will review the aforementioned distributed control strategy proposed in \cite{Guo2019} and evaluate its performance over a large power network, i.e. the Polish 2736sp network.

\subsubsection{Frequency Regulation and the Unified Controller}

%\lguo{I feel we can move details of UC to appendix and emphasize more on the cascading failure aspect here?}
Frequency regulation balances the power generation and consumption in an electric grid. Such control is governed by the swing dynamics and is traditionally implemented in generators through droop control, automatic generation control and economic dispatch. In recent years, it has been widely realized in the community that the ubiquitous fast-acting distributed load-side frequency regulation is needed and becomes realizable since more and more ``grid-friendly" devices such as refrigerators, air conditioners, and plug-in electrical vehicles can help to participate in regulating the power imbalance. 

The Unified Controller (UC) is a distributed control framework recently proposed in \cite{zhao2016unified}. It is designed so that the closed-loop control system evolves as a projected primal-dual algorithm to solve the optimization problem~\eqref{eqn:uc_olc}, where the control cost is minimized to restore the nominal frequency~\eqref{eqn:uc_balance},\eqref{eqn:dcflow}, restore the inter-area flows~\eqref{eqn:uc_ace} and maintain safe branch flows~\eqref{eqn:line_limit} and generations~\eqref{eqn:control_limit}. If \eqref{eqn:uc_olc} is feasible, under mild conditions, UC is guaranteed to converge to the optimal point. Interested readers are referred to \cite{zhao2016unified} for the details of UC.
\begin{subequations}\label{eqn:uc_olc}
\begin{eqnarray}
\min_{f, d, \theta} & \quad& \sum_{j\in\calN}c_j(d_j) \label{eqn:uc_obj}\\
\text{s.t.} & &r - d - Cf = 0 \label{eqn:uc_balance}\\
& &f = BC^T\theta  \label{eqn:dcflow}\\
& &ECf = 0\label{eqn:uc_ace}\\
& &\ul{f}_{e}\le f_{e}\le \ol{f}_{e}, \quad e\in\calE \label{eqn:line_limit}\\
& &\ul{d}_{j}\le d_j\le \ol{d}_j, \quad j \in\calN \label{eqn:control_limit}
\end{eqnarray}
\end{subequations}

UC is designed to rebalance the power and restore nominal frequency against power injection disturbances \lguo{and has been extensively investigated in the frequency regulation literature. It is first reported in \cite{Guo2019} that...}, however, it is first introduced in \cite{Guo2019} that such framework turns out to be quite powerful for failure mitigation and localization. The key idea for the proposed strategy is to implement UC over the regions defined by a tree-partition of the network. To be more specific, the control strategy consists of two phases: in planning phase, the control areas for UC should be created so that a tree structure is formed; in operating phase, UC actively monitors and reacts to failures and disturbances.

During the planning phase, the goal is to create a finer tree-partition, and coincide the control areas of UC and the regions defined by the tree-partition. We could use the approaches described in Section~\ref{sec:optimization} to refine the tree-partition without affecting the operational condition significantly.

During the operating phase, UC operates as a real-time controller against contingencies as shown in Fig.~\ref{fig:flow_chart}. After an initial failure happens, UC tries to drive the system back to an equilibrium point which is an optimal solution of \eqref{eqn:uc_olc}. If \eqref{eqn:uc_olc} is not feasible, however, UC becomes unstable, indicating it is impossible to achieve all the control objectives after such failure. Certain constraints in \eqref{eqn:uc_olc} will then be lifted to stabilize the system. There are two ways to do so: (i) involving more control areas to participate in the failure mitigation process by lifting the zero area control error constraints \eqref{eqn:uc_ace} or (ii) allowing load shedding by enlarging the range $[\ul{d}_{j}, \ol{d}_j]$ for the corresponding load buses \eqref{eqn:control_limit}. 
\begin{figure}[t]
\centering
\includegraphics[width=0.35\textwidth]{flow_chart}
\caption{Flowchart of the events after an initial failure under the proposed control strategy.}\label{fig:flow_chart}
\end{figure}

\subsubsection{Evaluation of Proposed Control Strategy}
We now evaluate the performance of the above control strategy over the Polish 2736sp network against failures. We first perform the aforementioned pruning methods \lguo{which pruning method?} to switch off 78 transmission lines for a partition of 4 regions, with sizes 1430, 818, 359 and 125. After switching off the lines, the maximal congestion level increases from 97.67\% to 97.81\%. This verifies\lguo{corroborates} our claim that the system congestion level will not significantly increase by carefully selecting lines to switch off.

%\lguo{Do we want to have a separate section specifically for numerical results? If we mention case studies here then we probably need similar experiments for all the remaining examples, which we may not have....}
The system robustness against failures is then evaluated in terms of the $N-1$ security standard. We iterate over every transmission line as the initial failure and simulate the cascading process thus triggered. To understand the robustness under different system congestion levels, we further scale down the line capacity by a factor $\alpha$ \lguo{that takes values} 95\%, 90\%, 85\% and 80\% (for those lines with flow exceeding the rescaled capacity, we reset their capacity as the absolute flow value) and repeat the simulation \lguo{for each of these $\alpha$}. This produces about 15,000 failure scenarios. 

Table~\ref{table:failure_case} illustrates the percentage of failures that can be mitigated with different levels of constraint lifting and the average load loss when load shedding is needed, under five congestion levels indicated by the line capacity factor $\alpha$. One can see there is a monotone behavior with respect to the congestion level. As the system becomes more congested, more failures will require the participation of other regions and even load shedding to prevent further failures. However, even when the congestion level is relatively high, more than 60\% single line failures can be mitigated and localized within the region itself. Moreover, the average load loss (30-50) is fairly small compared to the overall load demand ($1.8\times 10^4$). 

Fig.~\ref{fig:gen_dist} demonstrates the distribution for the number of regions where the generators are adjusted for failure mitigation with different levels of congestion. Similar monotone behavior is observed. As congestion level increases, more generator adjustments are needed to mitigate the failures. When the congestion level is low ($\alpha = 1$), one can see that more than 70\% single line failures can be localized without any generation adjustment, which indicates that the traditional industry practice such as droop control also works. However, as congestion level increases, more and more failures will require generation adjustments to stabilize the system. Thus, UC outperforms droop control and allows larger safe operational margins to achieve a better economical impact.

\chen{More detailed descriptions for the experiment? } {\color{green} [Adam: yes, maybe a little more is needed]}

\begin{table}[!h]
\centering
\begin{tabular}{p{2cm}|p{2.6cm}|p{3.5cm}|p{3cm}|p{2.2cm}}
Line capacity factor & failures mitigated within 1 region & failures mitigated with multiple regions & failures mitigated with load shedding& Average load loss \\
\hline \hline
0.8 & 63.27\% & 32.07\% & 4.66\% & 52.40 \\
\hline
0.85 & 72.17\% & 24.43\% & 3.40\% & 43.58 \\
\hline
0.9 & 73.77\% & 23.27\% & 2.96\% & 38.03 \\
\hline
0.95 & 85.25\% & 13.21\% & 1.54\% & 36.70 \\
\hline
1 & 90.57\% & 8.37\% & 1.07\% & 34.59
\end{tabular}
\caption{Distribution for the failures that can be mitigated with different levels of constraint lifting.}
\label{table:failure_case}
\end{table}

\begin{figure}
\centering
\input{gen_dist.tex}
\caption{Distribution for the number of regions that generators are adjusted. ``0" indicates that no generator adjustment is need.}
\label{fig:gen_dist}
\end{figure}


\subsection{Distributed AC OPF}
Introduce the SDP relaxation.

Introduce a few sufficient condition, and argue that these conditions are way easier to be satisfied with tree-partitions.

If the regions are chordal, then the $V\succeq 0$ condition can be equivalently solved separately by each region.

Argue that the method generalize to 3-phase Y-connected systems.

\subsection{SCOPF and Market}

\subsubsection{Tractable Market Price Manipulation}
Introduce the dynamical programming based method to solve the largest market price manipulation power.

Show that by having a tree-partition, assuming solving the sub-problem in each region is bounded by a constant (hopefully not too large if the graph is small), then we can generalize the above result to broader class of graphs.

\subsubsection{Accelerated Security-constrained OPF}
Security constrained OPF augments the conventional OPF by adding a set of contingencies and require the operating point to be safe under any of such contingency. This is usually achieved via the following:

Describe the two-step industry practice.

We now show that with a tree-partition, step 2 of the above can be significantly accelerated.

Describe a tree-partition based distributed solver for OPF.

Further, tree-partition induces a natural way to decompose this SCOPF problem. Compared to direct ADMM based method, this proposed method reduces the number of constraints and variables in each region by $O(k^2)$, and also decrease the number of messages necessary to pass across the agents by $O(k)$. As a result, the time for each agent to solve the local version of optimization is reduced by $O(k^6)$ (assume $O(N^3)$ complexity of LP solver) and the overall communication overhead is reduced by $O(k)$. From the simulation results, our method also reduces the number of iterations for convergence.

%\subsection{SLS for Frequency Regulation Controller Synthesis}
%It seems tree-partition allows easier synthesis of distributed controllers via SLS?

==> arxiv submission/conclusion.tex <==
\section{Concluding remarks \& future directions}
\label{sec:conclusion}
%\alec{I think the various applications in this section can be shortened. Perhaps we can mention them as possible future works. Right now, they are too short to fully discuss some of the nuances, yet too detailed/definitive as suggested future works.}

In this paper, we proposed a novel spectral representation of power systems which captures the topological and physical interactions within a power grid. Particularly, we illustrated that the graph Laplacian is of importance to characterize the power distributions. This spectral perspective further provides a simple, exact and clear representation of the power redistribution after line failures, where we introduced the network block decomposition to precisely characterize the boundary of the region a line failure can impact.

A finer block decomposition of the power grid creates more, smaller management regions whose operations can be isolated from each other in various aspects, bringing benefits such as disruption localizability, optimization parallelization, and more to the control and management of power systems. Therefore, we introduced a two-stage procedure to optimally modify the network topology for a finer block decomposition. Specifically, we first identify the candidate power network blocks by solving a weighted version of the network modularity problem and then identify the line switching action that has the least impact on the surviving network with respect to line congestion. This two-stage procedure is validated with numerical experiments. %\chen{Fill in some numbers from Section 6}.

In the rest of this section, we present a collection of examples on how network block decomposition offers powerful analytical guarantees and benefits in different power system applications beyond the setting of this paper, and how we can leverage these properties to improve the current industry practices in these applications.


\paragraph{Real-time failure localization and mitigation.}
Reliability is a crucial part for the development of sustainable modern power systems. Current industry practice relies on simulations based contingency analysis which is usually constrained by computational power~\cite{song2016dynamic}. Since the cascading failures exhibit a complicated and non-local propagation pattern, such analysis tends to omit the structural properties of failures and may fail to control and mitigate the failure in real time. There are topological models adopted from complex network analysis, however, such models are relatively simple thus cannot reveal physical properties~\cite{Hines2010}. 

As introduced in Sections~\ref{sec:spectral} and \ref{sec:localization}, network block decomposition leads to clear and well-defined boundaries that can localize the impact of failures. This suggests a new technique for grid reliability by switching off a small number of transmission lines so that finer-grained network blocks are created. In~\cite{Guo2019}, a real-time distributed control strategy utilizing the localizability from network block decomposition is proposed. Such control strategy is guaranteed to (i) always prevent successive failures from happening; and (ii) localize the impact of initial failures as much as possible. Simulation results show that the controller significantly improves the overall grid reliability. 

\paragraph{Security constrained OPF.}   
Security constrained OPF (SC OPF) is another approach to improve grid reliability that works by adding a set of contingencies and requiring the operating point to be safe under any of such contingency. These additional constraints greatly increase the size of the problem~\cite{capitanescu2011state}. In practice, the SC OPF is solved with contingency filtering techniques \cite{capitanescu2008new} to reduce the problem size and/or iterative methods such as Alternating Direction Method of Multipliers (ADMM)~\cite{chakrabarti2014security} for distributed computations. 

With a finer network block decomposition, both approaches can be significantly accelerated. The block induces a natural way to decompose and decouple the SC OPF, reducing the number of constraints and variables in each region. In addition, the messages necessary to pass across are reduced, leading to a fast convergence for the local optimizations. Therefore, there is huge potential in accelerating the computation of SC OPF when the network can be decomposed into comparable blocks.

\paragraph{Distributed AC OPF.}
Optimal Power Flow (OPF) underlies the efficient and stable operation of power grids, reducing the generation cost and transmission loss while maintaining the system stability in steady state. AC OPF problems are challenging because of their highly non-convex nature stemming from the nonlinear relationship between voltages and the complex powers. To overcome this challenge, semidefinite programming (SDP) relaxation of the AC OPF problem, where the optimization variable is transformed to a matrix $\mathbf{V}$ that needs to be semidefinite positive, i.e. $\mathbf{V}\succeq 0$, has been proposed; see~\cite{MolzahnHiskens2019,lavaei2011zero} for surveys to a considerable literature.
% It has been shown in~\cite{lavaei2011zero} that under proper conditions, the SDP relaxation attains the same global optimal value as the original AC OPF problem, inducing a polynomial time solution.
However, the standard SDP solvers do not scale well with the network size, necessitating a distributed solution where multiple agents communicate with each other and solve the relaxed problem together. This has proved difficult because the $\mathbf{V}\succeq 0$ constraint is globally coupled, rendering ADMM to be inapplicable. Nevertheless, it is shown in \cite{dall2013distributed} that if the power grid exhibits a block decomposition and each block has an nonempty interior, then the partial matrix with known entries specified by these blocks is chordal
%\alec{Not sure what this means: do you need each block too be itself chordal for the whole network to be completeable?} 
and thus can be completed to a feasible global solution $\mathbf{V}\succeq 0$ (see. e.g.,~\cite{6815671}). This enables the application of ADMM if the SDP optimization is decomposed in accordance with the network block structure and allows the optimization to be distributed to each block. Therefore, a finer network block decomposition helps reduce the overall operation cost by allowing AC OPF to be solved more efficiently.

\paragraph{Monitoring of price manipulation.}
Aggregators are playing an increasingly important role in the construction of a morden power grid, especially with the higher penetration level of renewable energy resources. The aggregators install, monitor and manage household energy devices such as rooftop solar panels and electric vehicle charging stations, and coordinate with utilities and Idependent System Operators (ISOs) to provide renewable generation and demand response. In addition to the benefits of aggregators, however, aggregators have the potential to manipulate prices through strategic curtailment for more profit~\cite{ruhi2017opportunities}. 
To quantify the potential for aggregators to exercise market power, in~\cite{ruhi2017opportunities} an algorithmic framework is given to approximately solve a bilevel quadratic optimization problem. Their method relies on decomposing the optimization problem into local parts and solve approximately with dynamic programming, thus only works for radial networks. It can be shown that similar bound holds in general networks if the block size of the network is upper bounded. Therefore, it is possible to extend the analysis from radial networks to general networks with proper block decomposition.

% Introduce the dynamical programming based method to solve the largest market price manipulation power.

%\chen{Show that by having a tree-partition, assuming solving the sub-problem in each region is bounded by a constant (hopefully not too large if the graph is small), then we can generalize the above result to broader class of graphs.}

==> arxiv submission/intro.tex <==
% \alec{Terminology issues to be resolved:
% \begin{itemize}
%     \item node vs vertex, line vs edge
%     \item power system vs power network vs power grid
% \end{itemize}}

\section{Introduction}
\label{sec:intro}
Electrical power grids are among the most complex and critical networks in modern-day society, reliably bringing power from generators to end users, cities and industries, often very far away geographically from each other. 
Traditionally, power systems have been designed as one-directional networks, where electric energy travels over high-voltage transmission lines from big conventional and controllable generators to distribution networks and eventually to consumers. This paradigm is changing rapidly in recent years due to many concurrent trends. Firstly, more distributed energy resources are coming online and consumers are slowly becoming prosumers, shifting the conventional one-directional power flow paradigm to bi-directional. There are massive investments in renewable energy sources, whose power generation is geographically correlated, more volatile, and less controllable than traditional sources of generation. Moreover, we are electrifying our transportation systems, which is extremely important for reducing our greenhouse gas emissions. %and reduce our dependence on fossil fuels.
However, electric vehicles have high energy demands and the current grid design and operations will not be able to sustain a high penetration of EVs, especially in view of correlated charging patterns. 
Managing increasing and correlated loads while having more volatile and less controllable generation may seem to be an impossible task, especially when aiming to keep the same operational and reliability standards. 
%Lastly, the power system is deemed to be an indispensable component of future Internet of Things development, transforming into a cyber-physical network vertically spanning numerous network layers and providing more functions. 

Given these trends, power grids are becoming increasingly stressed and have less margin for maneuver, making failures more likely and harder to contain, increasing the chance of blackouts. The growing complexity and increasing stochasticity of these networks challenge the classical reliability analyses and strategies. For instance, preventing line failures and mitigating their non-local propagation will become ever harder, having to deal with a broader range of more variable power injection configurations and more bidirectional flows on transmission lines.

% trend: grid flexibility
To respond to these increasing challenges,  power systems infrastructure is becoming more adaptive and responsive. Power systems have been traditionally looked at as a static network, but in fact they are not, since many of the transmission lines can be remotely taken online/offline. Rapid control mechanisms and corrective switching actions are increasingly being used to improve network reliability~\cite{shao2005corrective} and reduce operational costs~\cite{fisher2008optimal,hedman2009optimal}, especially since it is possible to quickly and efficiently estimate the current status of the grid using new monitoring devices and data processing strategies~\cite{huang2012state}.

% switching actions potential
However, new transmission infrastructure can be expensive and its placement will not necessarily increase reliability. Therefore, we need to make optimal use of the existing system and its adaptability. Optimally and dynamically switching transmission lines is an inexpensive and promising option because it uses existing hardware to achieve increased grid robustness. The ability of the operator to adaptively change the topology of the grid depending on the current network configuration offers a great potential. However, even with perfect information about the system, finding the best switching actions in real time is not an easy task. The flows on the lines are fully determined by power flow physics and network topology (cf.~Kirchhoff's and Ohm's laws), which means that every switching action causes a global power flow redistribution. In view of the combinatorial nature of this problem and of the large scale of the network, it is clear that a brute force approach will fail. 

%also because it is the only way we can indirectly use to modify the routing of the power in the network, which is  fully determined by power flow physics and network topology .

% smart-grid clustering~\cite{PaganiAiello2014}

\subsection{Contributions of the paper}
% \alec{Contributions:
% \begin{itemize}
%     \item comprehensive spectral representation (S2) & failure localization results (S2-3-4)
%     \item identify BBD as key
%     \item clustering & switching to refine bridge-block decomposition (S5-6)
% \end{itemize}
% }

This paper aims to tackle the aforementioned challenges in power systems operations by taking full advantage of transmission line flexibility.  To accomplish this requires new mathematical tools to first understand and then optimally and reliably operate these increasingly complex systems. In particular, a new understanding of the role of the network topology, especially when it comes to non-local failure propagation, is needed. %a well-known challenge for power systems reliability and operations. 

To this end, we introduce new spectral graph theory tools to analyze and optimize power systems. In particular, we propose a new spectral representation of power systems that effectively captures complex interactions within power networks, for instance inter-dependencies between infrastructure components and failure propagation events.
% Furthermore, the spectral methods we introduce can be used to quickly find approximate solutions to network optimization problems, like the aforementioned challenge of identifying optimal switching actions.
%The first contribution of this paper is to introduce a novel spectral representation of power systems and to show how to use spectral graph theory to analyze and optimize them. 
The key observation underlying this representation is the fact that, under the DC power flow approximation, the linear relation between power injections and line flows can be expressed using the weighted graph Laplacian matrix, where the line susceptances are used as edge weights. The eigenvalues and eigenvectors of this matrix thus contain rich information about the topology of the network as well as on its physical and electrical properties. Starting from this observation, Section~\ref{sec:spectral} illustrates how the graph Laplacian and its pseudo-inverse can be used to characterize islands of the power network and the power balance conditions of each island. 

When using conventional representations, the impact of line failures is discontinuous and notoriously difficult to characterize or even approximate, but our spectral representation provides a simple and exact characterization. More specifically, in Section~\ref{sec:distfactor} we show how the impact of network topology changes on line flows, quantified using the so-called \textit{distribution factors}, can be exactly described using spectral quantities. The results, most of which already appeared in~\cite{TPS1,TPS2} cover not only the case of single line outage, but also the more general case of the simultaneous outage of multiple lines. The analysis distinguishes two fundamentally different scenarios depending on whether the network remains connected or not, namely \textit{cut set outages} and \textit{non-cut set outages}.

Leveraging the spectral representation and the distribution factors analysis, in Section~\ref{sec:localization} we identify which graph sub-structures affect power flow redistribution and fully characterize the line failure propagation. More specifically, our analysis reveals that the network line failure propagation patterns can be fully understood by focusing on network block and bridge-block decompositions, which are related, respectively, to the cut vertices and cut edges of the power network. 

Our failure localization results suggest the robustness of the network is often improved by reducing the redundancy of the network, which indirectly makes the aforementioned decomposition finer. Using this insight, we then suggest in Section~\ref{sec:optimization} a novel design principle for power networks and propose algorithms that leverage their pre-existing flexibility to increase their robustness against failure propagation. More specifically, we propose a new procedure that, by temporarily switching off transmission lines, can be used to optimally modify the network topology in order to refine the bridge-block decomposition. We accomplish this through solving a novel two-stage optimization problem that adaptively modifies the power network structure, using the current power injection configuration as input. 

In Subsection~\ref{sub:mod} we introduce the first step of this procedure, which identifies a target number of clusters in the power network by solving an optimization problem whose objective function is a weighted version of the classical \textit{network modularity} problem. Being an NP-hard problem to solve exactly, we show how spectral clustering methods can be used to quickly and effectively obtain good approximated solutions, i.e., nearly-optimal clusters. 
The second step of our procedure, presented in Subsection~\ref{sub:cut}, identifies line switching actions that transform the identified clusters into bridge-blocks, refining the bridge-block decomposition of the network. The optimal subset of line switches are selected using a combinatorial optimization problem which aims to minimize the congestion of transmission lines of the network while achieving the target network bridge-block decomposition. 

This two-step procedure, which we refer to as the one-shot algorithm, is summarized in Subsection~\ref{sub:pra}, where we also introduce a faster recursive variant that iteratively refines the bridge-block decomposition by bi-partitioning the biggest bridge-block. The numerical implementation of both algorithms is discussed in Section \ref{sec:numerics}, where we test their performance on a large family of IEEE test networks of heterogeneous size. As revealed by our extensive analysis, almost all these power networks have a trivial bridge-block decomposition consisting of a single giant bridge-block, suggesting that their robustness could be greatly improved by our procedure.

Most of the present paper focuses on reliability issues and, in particular, line failure propagation, but we conclude in Section~\ref{sec:conclusion} by highlighting some other promising applications of the network block and bridge-block decompositions. Specifically, we demonstrate how a finer-grained block decomposition of a power network can be leveraged to (a) design a real-time failure localization and mitigation scheme that provably prevents and localize successive failures; (b) accelerate the standard security constrained OPF by decomposing and decoupling the problem into smaller versions in each block; (c) enable more efficient distributed solvers for AC OPF by transforming a globally coupled constraint into their counterparts for each block; and (d) tractably quantify the market price manipulation power of aggregators.

\subsection{Related literature}
\label{sub:literature}
The deep interplay between the topology of a given power system and power flow physics is for some aspects unique in network theory and a large body of literature has been devoted to the challenge of finding effective representations and approximations for these complex networked systems. These are instrumental not only to understand and analyze the behavior of these networks, but also to develop fast and effective algorithms and optimization strategies. In this subsection we briefly review the existing related literature on this topic.

Our work uses tools from spectral graph theory, an established and vast field in which many good books are available, see e.g.~\cite{brouwer2011spectra,VanMieghem2011} and reference therein. Particularly relevant for our analysis is~\cite{RanjanZhangBoley2014}, which focuses on the efficient computation of the pseudo-inverse of the graph Laplacian and explores its intimate connection with effective resistances. 
Graph spectra-based methods have been extensively used in the context of power systems, in particular in the study of phase angles frequency dynamics~\cite{Dorfler2013,Dorfler2014,Dorfler2018,Pirani2017,Koeth2019,Koeth2019b}, but also for power system restoration~\cite{QuirosTortos2013} and to analyze of the geometry of power flows~\cite{Retire2019,caputo2019spectral}. A spectral characterization for the network bridges, which play a crucial role in our analysis, was already given in~\cite{Cetinay2018,Soltan2017b}.

Understanding the underlying structure of given graph using spectral graph methods (e.g., Cheeger's inequalities) is a classical problem that received great attention in both discrete math and computer science literature. A canonical problem is the minimum $k$-cut problem, which aims to find the best partition in $k$ clusters of a given graph~\cite{StoerWagner1997}. The same problem has then been rediscovered in other domains, e.g., computer vision~\cite{ShiMalik2000}, with more emphasis on how to quickly find approximated solutions for NP-hard $k$-way partitioning problems. In this context, several clustering techniques based on spectral methods have been proposed~\cite{ShiMalik2000,NgJordanWeiss2002}, whose properties have later been studied analytically in~\cite{vonLuxburg2007}. At the same time, there was an increasing interest in the physics literature to study large networks arising in various domain (among which the world wide web and epidemiology) and unveil their underlying community structure, see~\cite{Fortunato2016} for a review. It is in this context that the concept of network modularity~\cite{Newman2004b,Newman2004} that we use in this paper has been introduced. Besides network modularity, many other techniques developed for complex networks have been applied to power systems, in particular to capture their main topological features and assess their robustness~\cite{PaganiAiello2013,Cuadra2015}.

The approach we propose in this paper crucially exploits the fact that the network topology of power systems can be changed by means of line switching actions. The classical \textit{Optimal Transmission Switching} (OTS) problem leverages the same existing flexibility, but with different goals. This optimization problem was first introduced in~\cite{koglin1980overload,Glavitsch1985,mazi1986corrective} as a corrective strategy to alleviate line overloading due to contingencies. Afterwards, transmission switching has been explored in the literature as a control method for various problems such as voltage security~\cite{shao2006,khanabadi2012optimal}, line overloads~\cite{granelli2006,shao2006}, loss and/or cost reduction~\cite{bacher1988,Fliscounakis2007,schnyder1990,Han2016,fisher2008optimal,hedman2010coopt}, clearing contingencies~\cite{khanabadi2012optimal,korad2013robust}, improving system security~\cite{schnyder1988}, or a combination of these objectives \cite{bacher1986network,rolim1999,shao2005corrective}. The interested readers can also read~\cite{Hedman2011} for a comprehensive review of the OTS literature.

Power grids are naturally divided in control regions~\cite{Panciatici2018}, raising the issue of how to optimally cluster and operate these networks. For this reason, clustering recently received a lot of attention in the power systems literature.  A very diverse set of methodologies have been considered, ranging from spectral clustering~\cite{Bialek2014} to various heuristics based on the modularity score~\cite{Guerrero2017,Lin2017}. A substantial effort has been devoted to expand and augment classical clustering methods in order to account for specific features of power systems, for instance using the notion of electrical distance~\cite{Blumsack2009,Cotilla2013} or conductances~\cite{LuWen2013,LuWen2015}. 
In the context of cascading failure analysis, clustering and community detection methods have also been used on the abstract interaction graphs~\cite{Nakarmi2018,Nakarmi2019} rather than on the physical network topologies.

Many ad-hoc clustering algorithms have been developed in the power systems literature particularly in the context of \textit{intentional controlled islanding} (ICI), an extreme security mechanism against cascading failures in which the network is disconnected into several self-sustained ``islands'' to prevent further contingencies. 
The goal of the standard ICI problem is to find the optimal partition of the network into islands while including additional constraints to ensure generator coherency and minimum power imbalance. This inevitably makes the clustering problem even harder and nontrivial trade-offs arise, which is the reason why several heuristics and approximations methods have been developed for ICI in the recent literature, see~\cite{HassaniAhangar2020,Liu2020} for an overview.

%\alec{We probably don't want to cite all ICI papers, right?~\cite{Babaei2019,Babaei2021,Ding2013,Ding2017,Ding2018,FernandezPorras2018,Noebels2019,Pahwa2013,QuirosTortos2014,Tyuryukanov2017,Tyuryukanov2018,Tyuryukanov2019,Trodden2013,Teymouri2019,Tyuryukanov2020,Znidi2019,Vittal1998,Vittal2003,XuVittal2010,Sun2003,LiLiu2010,Kirschen2019}}

Intentional controlled islanding is a rather extreme response to large-scale cascading failures. In~\cite{Bialek2021} the author propose as an alternative emergency measure beside precisely on the core properties of the bridge-block decomposition. Several other mitigation strategies less drastic than ICI could be adopted, but they often require more detailed cascade models. However, modeling cascading failures mathematically in power systems is rather complex due to the underlying power flow physics. The book~\cite{Bienstock2015} gives a comprehensive overview of the various models that have been introduced in the literature to describe cascading failures in power systems as well as the various optimization approaches that have been devised to improve the robustness of these systems. Most cascading failure models usually consider line or generator failures as trigger events, but correlated stochastic fluctuations of the power injections have also been considered in~\cite{Nesti2018}.

Contingency analysis is a very commonly used tool for reliable operations of a power system that assesses the impact of either generator and transmission line outages~\cite{Wood2013}. Such an impact can be assessed by solving the AC power flow equations that describe the network after each contingency.  Due to the large number of contingencies that must be assessed in order to satisfy $N-k$ security for $k \geq 1$, it is a common practice to first use DC power flow models to quickly screen contingencies and select a much smaller subset that result in voltage or line limit violations for more detailed analysis using AC power flow models. Such a contingency screening uses the \textit{power transfer distribution factors} (PTDFs) and \textit{line outage distribution factors} (LODFs) for a DC power flow model, see~\cite[Chapter 7]{Wood2013} for more details. The main advantage of using these factors is that the impact of generator and transmission outages on the post contingency networks can be analyzed using the common pre-contingency topology across contingency scenarios.
LODFs for multi-line outages were first considered in~\cite{EnnsQuadaSackett1982} to study the impact of network changes on line currents using the network Laplacian matrix, obtained from the admittance matrix after the linearization of AC power flow equations. However, the refined proof approach using the matrix inversion lemma was introduced later in~\cite{AlsacStottTinney1983,StottAlsacAlvarado1985}. Note that the paper~\cite{StottAlsacAlvarado1985} allows for more general outages (e.g., generator outages) and proposes a methodology to quickly rank contingencies in security analysis.
Probably unaware of the results in~\cite{AlsacStottTinney1983, StottAlsacAlvarado1985}, some of the formulas for generalized LODF (GLODF) have been re-discovered in \cite{ GulerGross2007,GulerGrossLiu2007,GuoShahidehpour2009} using different approaches based on the Power Transfer Distribution Factors (PTDF). More specifically, line outages are emulated through changes in injections on the pre-contingency network by judiciously choosing injections at the endpoints of each outaged/disconnected line using PTDF. 
Distribution factors for linear flows have been studied extensively in the recent literature~\cite{Horsch2018,Kaiser2020c,Ronellenfitsch2017,Ronellenfitsch2017b,Strake2019}.
Some recent work~\cite{TPS1,TPS2,Guo2018,Guo2019,Kaiser2020a,Kaiser2020b} rigorously proves that the presence of specific graph sub-structures guarantees that some of these distribution factors are zero, hence showing the potential for localizing outages and avoiding a global propagation by means of optimal network reconfiguration. The localization effects of these graph substructures can be effectively visualized by means of an ad-hoc version of the so-called \textit{influence} (or \textit{interaction}) \textit{graph}~\cite{Hines2013,Hines2017,Nakarmi2018,Nakarmi2019}. In~\cite{Guo2019,Liang2021,TPS3} the authors also explore how carefully designed network substructures synergize well with other control mechanisms that provide congestion management in real time. 
LODFs are also studied more recently as a tool to quantify network robustness and flow rerouting \cite{Strake2019}. While PTDF and LODF determine the sensitivity of power flow solutions to parameter changes, one can also study the sensitivity of optimal power flow solutions to parameter changes; see, e.g., \cite{Gribik1990, Hauswirth2018}.

% \ale{\textbf{Random notes}

% Unweighted power grid partitioning with novel methods and modularity just as reference~\cite{ChenXie2014,ChenXie2015}

% Evolutionary method for comm detection in power grids (modularity, Germany GridKit) \cite{Guerrero2017}

% %Community detection conductance-based weighted graphs~\cite{LuWen2013,LuWen2015}

% Community detection on influence/interaction graph~\cite{Nakarmi2018,Nakarmi2019}

% %Multiway Spectral Partitioning and Higher-Order Cheeger Inequalities~\cite{LeeTrevisan2014}
% %
% %\[
% %\phi(G_r) = \max_{V_1,\dots,V_r} \min_{k=1,\dots,r} \phi(V_k), \qquad \text{ where } \quad \phi(V_k)=1-\frac{\mathrm{Cut}(V_k,V_k^c)}{\mathrm{Vol}(V_k)}
% %\]

% normalized Laplacian is better~\cite[Section 8.5]{vonLuxburg2007} normalized Laplacian first used in ~\cite{NgJordanWeiss2002}

% \cite{Blumsack2009} goal is just defining power network zones using a weird system fitness + PJM example using 3 methods (hierarchical agglomerating, k-means/spectral, genetic) -- new method for network clustering based on electrical distances

% Multi-Attribute Partitioning of Power Networks Based on Electrical Distance (effective resistance/reactance)+ weird system fitness~\cite{Cotilla2013}

% \cite{Holme2015} Community consistency and structure play a significant role in the synchronization of networks
% } 
% \ale{link-shedding useful short-term strategy for power networks affected by disruptions}
% \alec{Power grids is naturally segmented/divided in control regions REFS ~\cite{Panciatici2018}}

% \ale{\cite{bernstein2014power} Various papers~\cite{Soltan2014,Witthaut2015,Cetinay2018,Cetinay2018b,Cetinay2018c,Wang2015} analyze the failure propagation in power systems.}

% \alec{\cite{Kocuk2016OR} OR, \cite{Han2016} EU network 2016}

%More specifically, OTS has been studied either as a corrective mechanism in case of voltage violations and line overloads~\cite{khanabadi2012optimal,korad2013robust,li2016real,li2019enhanced} or as a way to further decrease energy dispatching costs and/or reduce line losses while maintaining reliability standards~\cite{fisher2008optimal,hedman2008optimal,hedman2009optimal,ruiz2012tractable,soroush2013accuracies,kocuk2017new}.
% This problem was first 
% \alec{First paper on TS with line overload as objective?~\cite{koglin1980overload}\\ \cite{Glavitsch1985} gives an overview of the use of transmission switching as a corrective mechanism in response to a contingency.
% \cite{mazi1986corrective} propose a method to alleviate line overloading due to a contingency by the use of transmission switching as a corrective mechanism and they employ a heuristic technique to solve the problem due to the computational challenges of solving such a difficult problem at that time
% \cite{bacher1986network} further examine transmission switching in the AC setting to relieve line overloads
% \cite{schnyder1988,schnyder1990} proposed a fast corrective switching algorithm to be used in response to a contingency.
% \cite{rolim1999} provide a review of past transmission switching methods, the solution techniques used, the objective at hand, etc. \cite{shao2005corrective} continued previous research on the use of transmission switching as a corrective mechanism to relieve line overloads and voltage violations. In \cite{shao2006} a binary integer programming technique is used for the same motivation: to use switching actions as a corrective mechanism to relieve line overloads and voltage violations.
% \cite{bacher1988} and \cite{Fliscounakis2007} both examined the problem of modifying the grid topology in order to minimize system losses.
% Transmission switching can even be used as a congestion management tool. \cite{granelli2006} propose transmission switching as a tool to manage congestion in the electrical grid. The objective of the model is to minimize the amount of overloads in the network. They discuss ways to solve this problem by genetic algorithms as well as deterministic approaches.

==> arxiv submission/localization.tex <==
\section{Localization results}
\label{sec:localization}

In this section we show how the block and bridge-block decompositions of the power network $G$ fully captures the power redistribution effects after a contingency and give a very transparent view of the global network robustness against failures. More specifically, we characterize when LODF and GLODF are nonzero in terms of these network structures. The highlight is that an outage line has only a local impact which is confined in the (bridge-)block to which it belongs. We present the results for non-cut set and cut set outages separately in the next two subsections.

\subsection{Non-cut set outages}
The goal of this subsection is to show that the block decomposition of the network $G$ induces a block-diagonal structure for the PTDF and LODF matrices. The key idea is using the representation of these factors in terms of spanning forest and the intimate relation between the block decomposition and the cycles in the graph $G$. Lastly, we show that when the considered outage $\calE$ is a non-cut set, the GLODF matrix $K^\calE$ inherits the block-diagonal structure of the PTDF matrix.

% By combining the distribution factor theory we outlined in Section~\ref{sub:noncut} with the network block decomposition introduced in Subsection~\ref{sub:basic}, we can obtained the following result, see~\cite[Theorem 10]{TPS1}.
The next lemma states the \textit{Simple Cycle Criterion}, which has been proved in~\cite[Theorem 8]{TPS1}. It provides a sufficient condition for the LODF to be zero expressed purely in topological terms, namely using the cycles of the power network $G$.
\begin{lem}[Simple Cycle Criterion] \label{lem:simple_cycle}
Consider a non-bridge line $\hat \ell \in E$ and any other line $\ell \in E$. If there is no simple cycle in $G$ that contains both $\ell$ and $\hat \ell$, then the LODF $K_{\ell \hat \ell}= 0$. 
%\alec{Keep it for LODF or write the more general result for GLODF $K^\calE_{\ell \hat \ell} = 0$?}
\end{lem}
Used in combination with the network block decomposition introduced in Section~\ref{sub:basic}, this criterion can be used to show that the PTDFs and LODFs are always zero when they refer to two lines that belong to different blocks of the power network $G$.
\begin{prop}[LODF and PTDF characterization for non-bridge single line failure]
\label{prop:zeroLODFPTDF}
Consider a single non-bridge line $\hat \ell = (\hat i, \hat j)$ outage. %trips so that the surviving network $(V, E\!\setminus\! \{\hat l\})$ remains connected. 
For any surviving line $\ell = (i, j) \neq \hat\ell$ the following statements hold:
\begin{itemize}
\item[(i)] The PTDF $D_{\ell \hat\ell} = 0$ if and only if the LODF $K_{\ell \hat\ell} = 0$.
\item[(ii)] If $\ell$ and $\hat \ell$ are in different blocks of $G$, then $K_{\ell \hat\ell} = 0$ and $D_{\ell \hat\ell} = 0$.
\end{itemize}
\end{prop}
%Note that the latter proposition readily implies that the network block decomposition also induces a block-diagonal structure for the PTDF matrix, since if $\ell$ and $\hat \ell$ are in different blocks of $G$, then $D_{\ell \hat\ell} = 0$.

To formally state the next results for the distribution factor matrices when $\calE$ is a non-cut set outage, we first need some preliminary definitions to partition outage lines in $\calE$ and surviving lines in $-\calE$ depending on which block they belong to. More specifically, let $E = E_1 \cup \cdots \cup E_k$ be the block decomposition of (the edge set $E$ of) the network $G$. We partition accordingly into $k$ disjoint subsets both the outaged line set $\calE$ and the surviving lines set $-\calE$ as follows:
\begin{subequations}
\begin{align}
    \calE &= \bigcup_{j} \calE_j \quad \text{ with } \quad \calE_j := \calE\cap E_j, \qquad j=1, \dots, k,\\
    -\calE &= \bigcup_{j} \calE_{-j}  \quad \text{ with } \quad \calE_{-j} := -\calE\cap E_j = E_j \!\setminus\! \calE_j, \qquad j=1, \dots, k.
\end{align}
\label{eq:-EEdecomposition}
\end{subequations}
Without loss of generality we assume that the lines in $\calE$ are indexed so that the outaged lines are ordered depending on which subset $\calE_j$ they belong to. Similarly, the surviving lines in $-\calE$ are indexed so that the surviving lines are ordered depending on which subset $-\calE_j$ they belong to. In view of the partition in~\eqref{eq:-EEdecomposition}, the submatrices $B_{-\calE}$, $B_\calE$, $C_{-\calE}$ and $C_\calE$ appearing in~\eqref{ch:cf; subsec:LODF; eq:BCpartitions.1} can be further decomposed as
\begin{align}
B  &=  \begin{bmatrix} B_{-\calE} & 0 \\ 0 & B_\calE \end{bmatrix} \ \ =: \ \ 
	\begin{bmatrix}  \text{diag} \left( B_{-j}, j = 1, \dots, k \right) & 0 \\ 
		0 &  \text{diag} \left( B_{j}, j = 1, \dots, k \right) \end{bmatrix},
\\
C  &=  \begin{bmatrix} C_{-\calE} & C_{\calE} \end{bmatrix}  \ \ =: \ \ 
	\begin{bmatrix} C_{-1} & \cdots & C_{-k} & \ & C_{1} & \cdots & C_{k} \end{bmatrix}.
\end{align}
In particular, $C_{j}$ and $C_{-j}$ are the incidence matrices for the lines $\calE_j$ and $\calE_{-j}$, respectively.

\begin{prop}[Block diagonal structure of LODF and PTDF submatrices]
\label{prop:blockDF}
Let $\calE$ be non-cut set outage for the power network $G=(V,E,\bm{b})$. Then the two submatrices $D_{-\calE\calE}$ and $D_{\calE\calE}$ of the PTDF matrix defined in~\eqref{ch:cf; subset:glodf; eq:decomposeD.1} decompose as follows:
\begin{subequations}
\begin{equation}
    D_{-\calE\calE} =:  \begin{bmatrix} 
	D_{-1} & 0 & \dots & 0  \\  0 & D_{-2} & \dots & 0 \\ \vdots & \vdots & \ddots & \vdots \\ 0 & 0 & \dots & D_{-k} 
	\end{bmatrix}
	\qquad \text{ and } \qquad
	D_{\calE\calE}  =:  \begin{bmatrix} 
	D_1 & 0 & \dots & 0  \\  0 & D_2 & \dots & 0 \\ \vdots & \vdots & \ddots & \vdots \\ 0 & 0 & \dots & D_k 
	\end{bmatrix}
\label{ch:cf; sec:localization; eq:K-FF.1a}
\end{equation}
where, for each $j = 1, \dots, k$, $D_{-j}$ is the $|\calE_{-j}|\times |\calE_j|$ matrix given by $D_{-j}  := B_{-j} C_{-j}^T L^\dag C_j$, and $D_{j}$ is the $|\calE_{j}|\times |\calE_j|$ matrix given by $D_{-j}  := B_{j} C_{j}^T L^\dag C_j$. 

Furthermore, also the LODF matrix $K_{-\calE\calE}$ defined as in~\eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}} has a block-diagonal structure, namely
\begin{equation}
K_{-\calE\calE}   =:  \begin{bmatrix} 
	K_1 & 0 & \dots & 0  \\  0 & K_2 & \dots & 0 \\ \vdots & \vdots & \ddots & \vdots \\ 0 & 0 & \dots & K_k 
	\end{bmatrix},
\label{ch:cf; sec:localization; eq:K-FF.1c}
\end{equation}
where $K_j$ is the $|\calE_{-j}|\times |\calE_j|$ matrix given by $K_{j} :=  D_{-j} \left( I - \mathrm{diag}(D_j) \right)^{-1}$, for $j=1,\dots,k$.
\label{ch:cf; sec:localization; eq:K-FF.1}
\end{subequations}
\end{prop}
\begin{proof}
Recall from \eqref{ch:cf; subset:glodf; eq:decomposeD.1} that $D_{-\calE\calE} = B_{-\calE}C_{-\calE}^T L^\dag C_\calE$ and $D_{\calE\calE} = B_\calE C_\calE^T L^\dag C_\calE$. Proposition~\ref{prop:zeroLODFPTDF} then implies that the PTDF submatrices $D_{-\calE\calE}$ and $D_{\calE\calE}$ decompose into a block-diagonal structure corresponding to the blocks of $G$, obtaining~\eqref{ch:cf; sec:localization; eq:K-FF.1a}.
Since $K_{-\calE\calE} = D_{-\calE\calE} ( I - \textrm{diag}(D_{\calE\calE}) )^{-1}$ in view of identity~\eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}, the LODF submatrix $K_{-\calE\calE}$ has the same block diagonal structure as $D_{-\calE\calE}$. The invertibility of $I - \mathrm{diag}(D_j) = \mathrm{diag}(1-D_{\hat\ell \hat\ell}, \ell \in \calE_j)$ follows from Proposition~\ref{ch:lm; prop:PTDF.2}(ii) and Corollary~\ref{ch:lm; corollary:PTDF.3}, since every line $\hat\ell \in \calE_j \subset \calE$ is not a bridge and thus $D_{\ell\ell}<1$.
\end{proof}

The block decomposition of the network $G$ is crucial for failure localization also when a non-cut set $\calE$ of lines are disconnected simultaneously. More specifically, the next result shows that even in this scenario the impacts of line outages are still contained in their own blocks.
\begin{prop}[GLODF characterization for non-cut set outage]
\label{prop:glodf_non_cut}
Let $\calE$ be non-cut set outage for the power network $G=(V,E,\bm{b})$. Then, the rectangular $|-\calE| \times |\calE|$ GLODF matrix $K^\calE$ has a block-diagonal structure, i.e.,
\begin{subequations}
\begin{equation}
K^\calE  =:  \begin{bmatrix} 
	K^\calE_1 & 0 & \dots & 0  \\  0 & K^\calE_2 & \dots & 0 \\ \vdots & \vdots & \ddots & \vdots \\ 0 & 0 & \dots & K^\calE_k
	\end{bmatrix},
\label{ch:cf; sec:localization; eq:K^E.1a}
\end{equation}
where each $K^\calE_j$ is $|\calE_{-j}|\times |\calE_j|$ and involves lines only in block $E_j$ of $G$, given by:
\begin{equation}
K^\calE_j  :=  B_{-j} C_{-j}^T L^\dag C_j \left( I-B_j C_j^T L^\dag C_j \right)^{-1}, \qquad j = 1, \dots, k,
\label{ch:cf; sec:localization; eq:K^E.1c}
\end{equation}
where the submatrices $B_j, B_{-j}, C_j$ and $C_{-j}$ have been obtained by partitioning the matrices $B$ and $C$ according to the block structures of both $-\calE, \calE$. Equivalently, we have
\begin{equation}
K^\calE_j  =  D_{-j} (I - D_j)^{-1} = K_{j} \left(I - \textup{diag}(D_j) \right) \left( I-D_j \right)^{-1}, \qquad j = 1, \dots, k.
\label{ch:cf; sec:localization; eq:K^E.1b}%
\end{equation}%
\label{ch:cf; sec:localization; eq:K^E.1}%
\end{subequations}%
where $D_j, D_{-j}, K_j$, $j=1,\dots,k$, are the submatrices defined in Proposition~\ref{prop:blockDF}.
Furthermore, for every $\ell \in -\calE$ and $\hat\ell \in \calE$, if $\ell$ and $\hat\ell$ are in different blocks of $G$, then the GLODF $K^\calE_{\ell\hat \ell} =0$.
\end{prop}
\begin{proof}
The proof of~\eqref{ch:cf; sec:localization; eq:K^E.1} readily follows from Theorem~\ref{ch:cf; thm:LODF.3} after rewriting all the various submatrices resulting from the block decomposition and using Proposition~\ref{prop:blockDF}. The last statement is an immediate consequence of~\eqref{ch:cf; sec:localization; eq:K^E.1}.
\end{proof}
%Again, since a bridge is a block, a non-cut set outage will not impact the power flow on any bridge.
%\alec{Shall we include the ``only if'' part with the $\mu$-perturbation of the susceptances?}

%When we specialize the results above in the case of a outage involving a single line which is not a bridge, we obtain the following characterization for distribution factors in the case of a non-bridge single line failure.

We remark that, differently for the case of a single non-bridge failure in Proposition~\ref{prop:zeroLODFPTDF}, the PTDFs and GLODFs are not always simultaneously zero. Specifically, when multiple lines fail simultaneously, the fact that GLODF $K_{\ell \hat\ell}^\calE = 0$ does not imply that the PTDF $D_{\ell\hat\ell}=0$ or vice versa. Consider the counterexample in Fig.~\ref{fig:counterexample} where two dashed lines $\ell_1$ and $\ell_2$ fail simultaneously, i.e., $\calE = \{\ell_1, \ell_2\}$. Assuming all the lines have unit susceptances, the resulting absolute values of PTDF and GLODF are computed as in Table.~\ref{table:counterexample}. In particular, $K_{\ell_6,\ell_1}^\calE=K_{\ell_3,\ell_2}^\calE = K_{\ell_4,\ell_2}^\calE = 0 $, while the corresponding PTDFs are non-zero. We remark that such counterexamples may happen when the outage set $\calE$ is such that the block decomposition of the surviving network has more blocks than the original network (in our example, they are $4$ and $1$, respectively). 

\begin{table}[!ht]
  \begin{minipage}[b]{0.5\textwidth}
    \centering
    \includegraphics[width=0.6\textwidth]{OR-example.pdf}
    \captionof{figure}{Counterexample with the lines in the non-cut\\outage set $\calE = \{\ell_1, \ell_2\}$ displayed as dashed.}
    \label{fig:counterexample}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{tabular}{c|c|c|c|c}
      \toprule
      \diagbox{$\hat\ell$}{$\ell$}& $\ell_3$ & $\ell_4$ & $\ell_5$ & $\ell_6$ \\
      \hline \hline
      $\ell_1$ & 3/11, 1 & 3/11, 1 & 2/11, 1& 1/11, 0 \\
      $\ell_2$ & 1/11, 0 & 1/11, 0 & 3/11, 1 & 4/11, 1 \\
      \bottomrule
    \end{tabular}
    \caption{The distribution factors for all the lines reported as pairs (PTDF $D_{\ell,\hat\ell}$, GLODF $K^\calE_{\ell,\hat\ell}$).}
    \label{table:counterexample}
  \end{minipage}
\end{table}
\FloatBarrier

Nonetheless, the following proposition lists sufficient conditions for both implications to hold.
\begin{prop}[Zero GLODF and PTDF characterization]
\label{prop:glodf_ptdf}
Consider a non-cut set outage $\calE$ and a surviving line $\ell=(i,j)\notin \calE$. The following statements hold:
\begin{itemize}
    \item[(i)] If the PTDF $D_{\ell \hat\ell} = 0$ holds for any set of susceptances $B$, then the GLODF $K_{\ell\hat\ell}^\calE = 0$.
    \item[(ii)] If the GLODF $K_{\ell\hat \ell}^\calE=0$, then either the PTDF $D_{\ell\hat\ell}=0$ or every cycle in pre-contingency network $G$ that containing $\ell$ and $\hat \ell$ pass through at least one outage line different from $\hat \ell$.
\end{itemize}
\end{prop}

%\chen{The idea here is that we must state the extra condition ``under any susceptance'', so that we can get rid of the special symmetric structure. In general, there are structures where $PTDF=0, GLODF \neq 0$, or $GLODF = 0, PTDF \neq 0$}

\subsubsection{Visualizing LODFs using influence graphs}
\label{sub:influence}

The analysis of the LODFs corroborates a well-known fact in power systems, namely how after a particular line outage the next line to fail may be very distant topologically and geographically, as illustrated by~\cite{Dobson2016}. Classical contagion model in which failures spread locally from a node to its immediate neighbors are thus not appropriate to describe cascading failures on power networks (also due to the fact that line failures are an order of magnitude more likely than node outages).

A better way to capture the interdependencies between (single) line failures in power networks is by means of a specific type of ``dual graph'', usually referred to as~\textit{(failure) influence graph}~\cite{Hines2013,Hines2017} or \textit{interaction graph}~\cite{Nakarmi2018,Nakarmi2019}. There are many possible ways to define such a graph, but the high-level idea is that an influence graph $\mathcal \calL(G)$ is derived from the original power network $G$ as follows: the vertex set of $\mathcal \calL(G)$ is in one-to-one correspondence with the set $E$ of the lines of the power network $G$ and the pair of vertices corresponding to the lines $\ell, \hat\ell$ are connected in $\mathcal \calL(G)$ if and only if the failure of line $\hat\ell$ has a severe impact and/or causes and/or is correlated the failure of line $\ell$. 
The edges (or the edge weights) of the influence graph $\mathcal \calL(G)$ can thus be inferred by historical data or by simulating cascades. In this paper, we consider a version of the influence graph defined using LODFs very similar to the one in~\cite{Panciatici2018}, which offers a powerful way to visualize the potential risk of failure propagation. More specifically, the vertices corresponding to the lines $\ell, \hat\ell$ are connected in $\mathcal \calL(G)$ if and only if LODF is larger than a desired threshold, i.e., $|K_{\ell \hat\ell}| > K_\mathrm{min}$. 
%\alec{a possible alternative is considering a complete graph and $\{|K_{e\hat{e}}|\}_{e,\hat{e} \in E}$ as weights?}

\begin{figure}[!ht]
\centering
\subfloat[][The influence graph (in gray) obtained using the threshold $K_\mathrm{min}=0.005$. Due to the presence of a block, the influence graph has two clearly visible disconnected components, since all the corresponding LODFs are zero.]{\makebox[\width]{\includegraphics[width=.95\textwidth]{pre118.png}}}\\
\subfloat[][Schematic representation of the block and bridge-block decompositions of the original IEEE 118-node test network. The nontrivial bridge-block is further decomposed by a cut vertex into two blocks (in two different shades of green)]{\makebox[1.9\width]{\includegraphics[width=.5\textwidth]{pre118_BBD.png}}}
\caption{Original IEEE 118-node test network. It has 9 bridges (in orange), one nontrivial bridge-block (in green), and 9 trivial bridge-blocks. Furthermore, it has 9 cut vertices (in red), one of which decomposes the nontrivial bridge-block into 2 blocks (in different shades of green).} \label{fig:influencegraph_pre}
\end{figure}

As illustrated for the IEEE 118-node test network in Fig.~\ref{fig:influencegraph_pre}(a), the influence graph of power network tend to be very dense and connecting many lines that are topologically far away, corroborating the non-local propagation of line failures.
Fig.~\ref{fig:influencegraph_pre}(b) shows the block and bridge-block decomposition of the same network. This network has a trivial bridge-block decomposition, consisting of a single nontrivial bridge-block and $9$ trivial ones. This bridge-block consists of two nontrivial blocks, separated by a cut vertex. As predicted by the theory (cf. Proposition~\ref{prop:zeroLODFPTDF}), the influence graph is not connected, since all the LODFs corresponding to pairs of lines in the two blocks are identically zero. 

By removing three lines from IEEE 118-node test network, we can make both the block and bridge-block decompositions of this network finer, as illustrated in Fig.~\ref{fig:influencegraph_post}. The influence graph of the pruned network is now less dense and have more disconnected components, showing a higher localization capability.
Fig.~\ref{fig:influencegraph_post}(b) shows the finer block and bridge-block decomposition of the pruned network. It has two nontrivial bridge-blocks, one of which further decomposes into four nontrivial blocks, separated by cut vertices.

\begin{figure}[!ht]
\centering
\subfloat[][The influence graph (in gray) of the pruned IEEE 118-node test network obtained using the threshold $K_\mathrm{min}=0.005$. Due to the presence of four blocks (in blue and three shades of green), the influence graph has four clearly visible disconnected components, since all the corresponding LODFs are zero.]{\makebox[\width]{\includegraphics[width=.95\textwidth]{post118.png}}}\\
\subfloat[][Schematic representation of the block and bridge-block decomposition of the pruned IEEE 118-node test network. The green bridge-block further is further decomposed by cut vertices into three blocks (in different shades of green). ]{\makebox[1.9\width]{\includegraphics[width=.5\textwidth]{post118_BBD.png}}}
\caption{The network obtained from the IEEE 118-node test network removing three lines (shown as dashed black edges). It has 10 bridges (in orange), two nontrivial bridge-block (in blue and green), and 9 trivial bridge-blocks. Furthermore, it has 13 cut vertices (in red), two of which decomposes the nontrivial green bridge-block into 3 blocks (in three different shades of green).} \label{fig:influencegraph_post}
\end{figure}
\FloatBarrier

%The various formulae are summarized in Table \ref{ch:cf; sec:localization; table:summary}.
%\begin{table*}[htbp]
%\centering
%\begin{tabular}{ || l || l | l | l ||}
%	\hline\hline
%	PTDF	& $D$		& $B C^T  L^\dag  C$ & Proposition \ref{ch:lm; prop:PTDF.2} \\
%			& $D_{-\calE\calE}$	& $B_{-\calE}C_{-\calE}^T L^\dag C_\calE$ 	& \eqref{ch:cf; subset:glodf; eq:decomposeD.1}	  \\
%			& $D_{\calE\calE}$	& $B_\calE C_\calE^T L^\dag C_\calE$		& \eqref{ch:cf; subset:glodf; eq:decomposeD.1}	 \\
%	\hline
%	GLODF	& $K^\calE$ 		& $D_{-\calE\calE} (I - D_{\calE\calE})^{-1}$ & Theorem \ref{ch:cf; thm:LODF.3} \\
%	\hline
%	LODF   	%& $K^{\hat \ell}$	& $D^{\hat \ell} \left( I - D_{\hat \ell\hat \ell} \right)^{-1}$ & Theorem \ref{ch:lm; prop:LODF.1} \\
%			& $K_{-\calE\calE}$	& $D_{-\calE\calE} \left( I - \textup{diag}(D_{\calE\calE}) \right)^{-1}$ & \eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}	\\
%	\hline \hline
%\end{tabular}
%\caption{Summary of key formulae.}
%\label{ch:cf; sec:localization; table:summary}
%\end{table*}

\subsection{Cut set outages: Power rebalance and redistribution}
% \aleb{Definition needed: participating node, participating island, participating grid.

% \begin{prop}[Non-zero GLODF and PTDF characterization for multiple line failures]
% \ale{...}
% \end{prop}

% \begin{cor}[LODF and PTDF characterization for bridge failures]
% \ale{...}
% \end{cor}}

% \chen{Participating node is defined in Section 3.3. We may not introduce the participating island/grid since our goal is to have simple path criterion and state when the flow will not change. It seems that it may be better to merge section 4 into Section 3.}

We now discuss the impact of cut set outages. As mentioned in Subsection~\ref{sub:cut}, we assume the post-contingency power balancing rule is decoupled for each island so that we can study the power redistribution in each of them separately. In particular, we consider the proportional control $\mathbb G_{\alpha}$ that the post-contingency power injection is adjusted proportionally to compensate the power imbalance caused by the cut set outages.

Consider an island $\calI$ and let $E_\calI:=\set{(i,j)\in E ~:~ i\in\calI \text{ and } j\in\calI }$ denote the set of edges whose both end points belong to $\calI$ before contingency. As outlined in Subsection~\ref{sub:cut}, we partition the failed lines into tie line failures $\calE_\textrm{tie}$ and internal line failures $\calE_\textrm{int}$.
Rewriting~\eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} for a specific surviving line $\ell \in E_\calI \setminus \calE_\textrm{int}$ in island $\calI$ yields
\begin{equation}
\Delta f_{\ell} = 
	\sum_{\hat \ell\in \calE_\textup{int}} K^{\calE_\textup{int}}_{\ell\hat \ell} \, f_{\hat \ell}   \ \ + \ 
	\sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k
		\Big( D_{\ell, k j(\hat \ell)} + \sum_{\hat \ell'\in \calE_\textup{int}} K^{\calE_\textup{int}}_{\ell\hat \ell'} D_{\hat \ell', k j(\hat \ell)} \Big).
\label{ch:cf; subsec:bridgeoutage; eq:DeltaP.l}
\end{equation}

It is observed that the impact of cut set outages consists of two terms, one capturing the impact of the internal line failures in $\calI$ and the other capturing the impact of the tie line failures, as shown in~\eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.l}. In order to describe the impact boundary of such cut set outages, we will study the conditions so that \eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.l} is zero. 

Decompose the pre-contingency subnetwork corresponding to the island $\calI$ into blocks. For any surviving line $\ell$ and failed internal line $\hat \ell \in \calE_\textrm{int}$ pair, Proposition~\ref{prop:glodf_non_cut} indicates that $K_{\ell \hat \ell}^{\calE_\textrm{int}} = 0$ if $\ell$ and $\hat\ell$ are in different blocks of $\calG_\calI$. Therefore, if a surviving line $\ell$ is not in the same block as any outaged internal lines, \eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.l} simplifies to \[
\Delta f_\ell = \sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k
		 D_{\ell, k j(\hat \ell)} 
\]
This suggests that the impact of multiple outaged tie lines is separable. 
In the following lemma we state the \textit{Simple Path Criterion}, cf.~\cite[Theorem 1]{TPS2}, which provides a sufficient condition for the PTDF introduced in Subsection~\ref{sub:PTDF} to be zero in purely topological terms.
\begin{lem}[Simple Path Criterion] \label{lem:simple_path}
For any line $\ell\in E$ and two nodes $j,k\in V$, if $\ell$ there is no simple path in the power network $G=(V,E,\bm{b})$ connecting nodes $j$ and $k$ that contains line $\ell$, then the PTDF $D_{\ell,jk}=0$.
\end{lem}
Leveraging this criterion and the notion of participating bus introduced in Subsection~\ref{sub:cut}, we can derive a sufficient condition, summarized in the following proposition~\cite[Corollary 6]{TPS2}, for a surviving line $\ell$ not to be impacted by a cut set outage. 

% \chen{We do not prove the following proposition and corollary formally in TPS, but it is straightforward from Simple Path/Cycle Criterion. Shall we include them in Appendix?} \alec{Yes. Can you also make sure that both Simple Loop and Simple Path Criterion are both stated in the right place and proved/referenced?}
% \chen{Added in Lemma~\ref{lem:simple_cycle}.}

\begin{prop}[Characterization for cut set failures]
\label{prop:glodf_cut}
Consider a cut set $\calE$ outage that disconnects the power network into two or more islands with decoupled power balancing rules. Let $\calI$ denote one such island under the proportional control $\mathbb G_{\alpha}$, and let $\calE_\calI = \calE_\textrm{tie} \cup \calE_\textrm{int}$ be the set of outaged lines with one or both endpoints in this island. For any surviving line $\ell$, if $\ell$ is not in the same block as any outaged internal lines $\hat \ell \in \calE_\textrm{int}$ and $\ell$ is not on any simple path connecting the endpoint of an outaged tie line $j(\hat \ell)$ and a participating bus $k$ with $\alpha_k > 0$ for any $\hat \ell \in \calE_\textrm{tie}$, then the post-contingency flow on line $\ell$ remains unchanged.
\end{prop}

We can reformulate the latter result in even simpler terms in the case of a single bridge line outage, obtaining the following simplified characterization for the surviving lines whose post-contingency flow remains unchanged, see~\cite[Corollary 2]{TPS2}.

\begin{cor}[Characterization for bridge failures]
Consider the outage of a bridge line $\hat \ell=(\hat i, \hat j)$ with nonzero flow $f_{\hat \ell}\neq 0$ that disconnects the power network into two islands. Let $\calI$ be the island that contains node $\hat j$.
Under the proportional control $\mathbb G_{\alpha}$, for any line $\ell$ in $\calI$ if there is no simple path in $\calI$ that contains $\ell$ from the node $\hat j$ to a participating bus $k\in \calI$ with $\alpha_{k}>0$, then the post-contingency flow on line $\ell$ remains unchanged.
\end{cor}

%\subsubsection{Single non-bridge failure and the Simple Loop Criterion}
%Let us consider first the scenario where only a single non-bridge line $\hat \ell$. The characterization of the distribution factors in spectral terms can be used to fully characterize when the LODF $K_{\ell \hat \ell}$ is zero or not in terms of graph structures and thus identify where the isolated failure of line $\hat \ell$ may possibly propagate in the network.
%
%\begin{prop}[Simple Loop Criterion (SLC)]
%Let $G=(V,E)$ be a connected power network and $\hat \ell \in E$ a non bridge, so that $G^{\{\hat \ell\}}$ is still connected. Then, for every $\ell \in E \setminus\{e\}$, $K_{\ell \hat \ell} \neq 0$ if and only if there exists a simple loop in $G$ that contains both $\ell$ and $\hat{\ell}$. 
%\end{prop}
%
%\begin{prop}[Simple Loop Criterion (SLC)]
%Let $G=(V,E)$ be a connected power network and $\hat \ell \in E$ a non bridge, so that $G^{\{\hat \ell\}}$ is still connected. Then, for every $\ell \in E \setminus\{e\}$, $K_{\ell \hat \ell} \neq 0$ if and only if there exists a simple loop in $G$ that contains both $\ell$ and $\hat{\ell}$. 
%\end{prop}
%
%\subsection{Cut set outages: Power Rebalance and Redistribution}
%
%\alew{
%For a detailed discussion and the proof of SLC see~\cite[Proposition 11]{TPS1}. From the SLC, it immediately follows that if $e$ and $\hat{e}$ are edges that belong to different tree-partition regions, then $K_{e\hat{e}}=0$, since there cannot be any simple loop containing both of them. The SLC also immediately applies to the finer block decomposition, since by construction there is no simple loop containing two edges belonging to different blocks. In fact, blocks are the minimal graph structure to which the SLC applies, making them the smallest components of the original network in which line failures are automatically confined.
%
%Therefore, $K_{e\hat{e}} \neq 0$ only if $e$ is not a bridge and both $e$ and $\hat{e}$ belong to the same block. Under mild conditions to avoid pathological cases, the converse is also true and the result can be extended to show that if $e$ is a bridge, then we always have $K_{e\hat{e}} \neq 0$, see~\cite{TPS2} for the precise statement. 
%
%This single-failure localization property can be effectively visualized using the influence graph. By removing three lines in the IEEE 118-node test network, we create a nontrivial tree partition with two regions (one of which then consists of three blocks). The resulting influence graph, shown in Fig.~\ref{fig:influencegraph_treepartition}, consists of four disconnected components, corroborating the theoretical results that failure cannot propagate outside the region (block) in which they occurred.
%
%\begin{figure}
%\centering
%\includegraphics[width=.83\textwidth]{inf_graph_ieee118_after.eps}
%\caption{IEEE 118 test network (in blue) after removing three lines (dashed orange) and the resulting influence graph (in gray) obtained connecting two transmission lines $e$ and $\hat{e}$ whenever $|K_{e\hat{e}}| > 0.005$} \label{fig:influencegraph_treepartition}
%\end{figure}
%\FloatBarrier
%
%In the next subsection, we extend this result and study failure localization properties of the network in the most general scenario where either (i) multiple lines fail simultaneously or (ii) failures create islands (and thus power balancing rules are triggered).
%
%%Fig. \ref{fig:butterfly} is a simple illustration of this concept, where we decompose the original butterfly network in Fig. \ref{fig:butterfly}(a) that contains a cut-vertex $c$ into two cells. Note that two different cells within a tree partition region may share a common vertex as the block decomposition is a partition of the graph edges. 
%%
%%\begin{figure}
%%\centering
%%\subfloat[]{\includegraphics[height=2cm]{butterfly.png}}
%%\hspace{1cm}
%%\subfloat[]{\includegraphics[height=2cm]{butterfly_decomp.png}}
%%\caption{(a) A butterfly network. (b) The block decomposition of the butterfly network into cells $\calC_1$ and $\calC_2$. \alec{Do we want to keep this figure?}}\label{fig:butterfly}
%%\end{figure}
%
%
%The first main result that connected the network structure as captured by the block decomposition and the GLODF is the following.
%\begin{thm}\label{thm:multi_line_no_cut}
%Consider a power network $G$ with block decomposition $B_1,\dots,B_k$. The generalized load outage distribution factor $K^\calE_{\ell \hat{\ell}}$ is non-zero ``if'' and only if the lines $\ell$ and $\hat{\ell}$ belong to the same block. 
%\end{thm}
%This result implies that line contingencies are automatically localized within the corresponding block.} \alec{Argue how having a power network with a finer block decomposition is more desirable in terms of reliability and robustness against failures}
%
%\alec{Tree partition is ``monotone'' during a cascading failure''}
%
%
%\alew{Suppose $\ell$ is not in the same block as any outaged internal lines $\hat \ell \in \calE_\textup{int}$ and is not on any simple path connecting $j(\hat \ell)$ and a participating node $k$ with $\alpha_k>0$ for any outaged tie line $\hat \ell\in \calE_\textup{tie}$. Then Theorem \ref{ch:cf; thm:K^Fblock.1} implies that $K^{\calE_\textup{int}}_{\ell\hat \ell} = 0$ for any $\hat \ell\in \calE_\textup{int}$ and Theorem \ref{ch:cf; subsec:bridgeoutage; theorem:simplepath} implies that $D_{\ell, k j(\hat \ell)} = 0$ for any $\hat \ell\in \calE_\textup{tie}$, and hence the power flow on line $\ell$ will remain unchanged.}
%%\subsection{Power flow redistribution}
%%In the rest of the section we illustrate the effect of network topology changes on power flows and show how it can be quantified using spectral quantities. 
%%
%%Consider a connected power network $G$ with balanced injections $\pp$. When a subset of lines $\calE \subset E$ trips or is removed from service, the network topology changes and, as a consequence, the power flow redistributes on the \textit{surviving network} $G^\calE :=(V,E \setminus \calE)$ as prescribed by power flow physics.%, possibly causing overloads in some of the other lines, not necessarily adjacent to the removed ones in $\calE$. 
%%
%%We denote by $\ff_\calE$ and $\ff_{-\calE}$ the original power flows in $\calE$ and in $E \bs \calE$ respectively and by $\hat{\ff}_{-\calE}$ the new flows on the surviving network. 
%%We are particularly interested to characterize how the flows changed after removing the set of lines $\calE$, by looking at the quantity $\Delta \ff_{-\calE} :=  \hat \ff_{-\calE} - \ff_{-\calE}$.
%%
%%To fully understand the power flow redistribution and unveil the impact of network topology on the flow changes, we distinguish two scenarios, depending on whether $\calE$ is a cut set or not for the power network $G$, and we treat them in two separate subsections. 
%%
%%\subsubsection{Non-cut set}
%%If the subset of removed lines $\calE$ is not a cut set for the power network $G$, then the surviving network $G^\calE$ is still connected. The injections $\pp$ are thus still balanced and the new power flows can be calculated directly from~\eqref{eq:flowsdc_model} after having updated the matrices $B$, $C$, and $L$. We now review this calculations in more details and introduce the global line outage distribution factors (GLODF), which more transparently show the impact of the removal of each line in $\calE$ to each of the survival lines.
%%
%%Consider the decomposition of $B, C$ into submatrices corresponding to the subset of removed lines $\calE$ and the remaining lines in $E \bs\calE$, i.e.:
%%\[
%%	B =: \textup{diag} (B_\calE, B_{-\calE}), \qquad C =: [C_\calE, C_{-\calE}].
%%\]
%%We can rewrite the power flow changes $\Delta \ff_{-\calE}$ on the surviving lines in terms of original flows $\ff_\calE$ on the removed lines as 
%%\begin{equation}\label{eqn:multi_line_lodf}
%%	\Delta \ff_{-\calE}  =  K^\calE \ff_\calE,
%%\end{equation}
%%where the $|E \bs \calE| \times |\calE|$ matrix $K^\calE$ in \eqref{eqn:multi_line_lodf} is known as the generalized line outage distribution factor (GLODF). It can be calculated as \ale{ADDREF}
%%\[
%%	K^{\calE} = B_{-\calE}C_{-\calE}^T L^\dag C_\calE(I-B_\calE C_{\calE}^T L^\dag C_\calE)^{-1}.
%%\]
%%\alec{GLODFs literature review from TPS2 to be integrated} \ale{The formula of $K^E$ can be derived by considering the pre-contingency network with changes $\Delta \pp$ in power injections that are judiciously chosen to emulate the effect of simultaneous line outages in $E$. The reference \cite{AlsacStottTinney1983} seems to be the first to introduce the use of matrix inversion lemma to study the impact of network changes on line currents in power systems. This method is also used in \cite{StottAlsacAlvarado1985} to derive the GLODF for ranking contingencies in security analysis. The GLODF has also been derived earlier, e.g., in \cite{EnnsQuadaSackett1982}, and re-derived recently in \cite{GulerGrossLiu2007, GulerGross2007}, without the simplification of the matrix inversion lemma.}
%%
%%From~\eqref{eqn:multi_line_lodf} it follows that the power flow change on specific surviving line $\hat e \in E \bs \calE$ depends on the original flows on \emph{all} the removed lines $e\in \calE$ and, more specifically,
%%\begin{equation}
%%	\Delta f_{\hat e} = K^\calE_{\hat ee}\, f_e,
%%\label{eqn:power_change_E}
%%\end{equation}
%%where $(\hat{e},e)$-th entry of the GLODF matrix $K^\calE$. 
%%In particular, similar to the single-line failure case, if $\hat e$ does not share a cell with any line $e\in E$ then its line flow will not be impacted. % $(\Delta f_{\hat e} = 0)$.
%%However, unlike the single-line failure case where $K_{\hat{e}e}\neq 0$ implies $f_{\hat{e}}\neq 0$, we do not necessarily have $\Delta f_{\hat e}\neq 0$ even when $\hat e$ is in the same cell as some $e\in E$. This is because the impact on $\hat{e}$ from different line failures in $E$ can potentially cancel each other. Nevertheless, it can be shown that under mild conditions on the topology of $\calG$ or by adding a perturbation to the system injection $\pp$ (similar to how we perturb the line susceptances $B$ with $\mu$), such a cancellation almost surely does not happen.
%
%%Structure and properties of power grids, also using effective resistance~\cite{Cotilla-Sanchez2012,Hines2010,Hines2010b}
%
%%%Topological and electrical distances on power networks~\cite{Cotilla-Sanchez2012}
%%
%%\alec{Argue here that most power systems have a trivial tree partition consisting of a large region to which (almost) every node belongs and possibly a few trivial regions, consisting of isolated nodes connected to the rest of the network by a single line? If so, add supporting statistics about IEEE test cases?}
%
%%In the case of the failure of a single line, i.e. $\calE=\{e\}$, if $G^\calE$ is still connected, then the branch flow change on any other line $\widetilde{e} \neq e$ is given as
%%$$
%%	\Delta f_{\hat{e}} = f_e \cdot K_{e\widetilde{e}},
%%$$
%%where $K_{e\widetilde{e}}$ is the \emph{line outage distribution factor} \cite{Wood1996} from $e$ to $\widetilde{e}$ \lguo{Do we want to do cut set and non-cut set failure here instead since $\calE$ is a set of edges? See part II of the TPS paper for the full theory in this case} \alec{Yes!}. It is known that the line outage distribution factors are independent of the original power injections $\pp$ and depend only on the network topology; in fact, they can be computed from the matrices $B$ and $C$ as showed in~\cite{Wood1996}.
%%\alec{Need to explain cascade mechanism here and typical non-local failure propagation}
%
%%Let $G=(V,E,w)$ be an undirected graph with $n=|V|$ nodes, $m=|E|$ edges and non-negative edge weights $\{w_{ij}\}_{i,j \in V}$, with the convention that absent edges have weight equal to zero. We henceforth assume that $G$ is connected and has no self-loops.
%%
%%For $k\in \{1,\dots,n\}$, let $\mathcal{V} = \{V_1,\dots,V_k\}$ be a $k$-partition of the vertex set, i.e., a collection of nonempty subsets $V_i \subseteq V$ to which we will refer as \textit{regions} such that $V_i \cap V_j = \emptyset$ for $i\neq j$ and $\bigcup_{i=1}^k V_i = V$. Given a partition, we refer to an edge as a \textit{cross edge} if its two endpoints belong to different regions and \textit{internal edge} otherwise. A partition $\mathcal{V}$ of the vertex set $V$ automatically induces a partition of the edge set $E$ into cross edges and internal edges, whose collections will be denoted as $E_c(\mathcal{V})$ and $E_i(\mathcal{V})$, respectively.
%
%%In the previous section we showed how, given a set of power injections, the power flow dynamics is uniquely determined by the network topology and line weights. Therefore, after any (set of) line failures, the power flows redistribute on the surviving lines depends only on the structure of the surviving network, possibly causing additional overloads and failures. 
%%
%%In this section we explore which network features and substructures are the most crucial to understand how failures can propagate and introduce the notion of \textit{tree partition} of a power network, 
%
%
%%\subsection{Failure Localization}
%%The tree partition and block decomposition of a power system encode rich information on the possible failure propagation patterns. More specifically, in this subsection we show that line failures are always confined inside the region or, even more precisely, within the block where the original failure happened. Furthermore, we prove a complementary result stating that failure propagation across different regions can only occur after a bridge fails. The rest of the section is devoted to rigorously establishing these failure localizability properties of tree partitions.
%%
%%Our main results strongly suggest that by identifying the power network tree partition leads to clear and well-defined boundaries that isolate failures and prevent long-distance impacts of such contingencies. In Section~\ref{sec:optimization} we precisely address the question of how to create a finer tree partition structure leveraging the existing flexibility in the power network topology.
%
%\aleb{
%\subsection{Cut set outages: Power Rebalance and Redistribution}
%Denote by $\ff_{\calE_\calI}$ the vector of original flows on internal lines of $\calI$ that failed and let $\Delta \pp_\calI$ be the vector of injection adjustment triggered by the balancing rule $\calB$. The following result shows that, as far as the net change of power flows $\Delta \ff_\calI$ on the surviving lines inside the island $\calI$ is concerned, the contributions due to balancing and redistribution described above decompose and can thus be studied separately.
%
%\begin{thm}{\cite[\ale{Proposition X}]{TPS2}}
%\label{prop:localization}
%Consider an island $\calI$ of the power network $G$ in which the subset $\calE$ of lines have been removed. The net change of the power flows $\Delta \ff_\calI$ on the surviving lines inside the island $\calI$ is given by
%\begin{equation}\label{eqn:new_flow_change_decomp}
%\Delta \ff_\calI = K^\calB \Delta \pp_\calI + K^\calR \ff_{\calE_\calI},
%\end{equation}
%where $K^\calB$ and $K^\calR$ are matrices independent of $\Delta \pp_\calI$ and $\ff_{\calE_\calI}$.
%\end{thm}
%
%In other words, the net power flow change $\Delta \ff_\calI$ on the surviving lines in $\calI$ are determined as a linear transformation of the power rebalance actions $\Delta \pp_\calI$ and of the original flows $\ff_{\calE_\calI}$ on the tripped lines. Further, the matrices $K^\calB$ and $K^\calR$ depend only on the graph structure, allowing us to apply the spectral view of power redistribution to study their properties. In the following subsections, we characterize the structures of $K^\calB$ and $K^\calR$.
%
%\subsubsection{Power Rebalance to Participating Nodes}
%We now focus on the power rebalance term appearing in~\eqref{eqn:new_flow_change_decomp} and give more details on the matrix $K^\calB$. Since by definition $\calE_{\partial \calI}$ is the subset of tripped lines that have exactly one endpoint in $\calI$, the subset $\calE_{\partial \calI}$ is a \emph{cut set} of $G$ that disconnects $\calI$ from the other network components. Furthermore, the fact that there was originally power flowing on the lines in $\calE_{\partial \calI}$ is the root cause of the (potential) power imbalance on $\calI$. To simplify our discussion, we assume without loss of generality that $\calE_{\partial \calI}$ consists of a single edge, and we denote by $u$ its endpoint in $\calI$ and refer to it as \textit{disconnection node}.
%
%To resolve a power imbalance on $\calI$, any balancing rule $\calB$ selects a subset of \emph{participating nodes} $\calN_\calB \subset V_\calI$ and adjust only the injections of those nodes by $\Delta \pp_\calI$. In other words, a node $j$ is participating if and only if  $(\Delta \pp_\calI)_j \neq 0$ under $\calB$. Under the DC model~\eqref{eq:dc_model}, it is clear that the resulting power flow change $\Delta \ff_\calI^\calB$ due to the balancing rule $\calB$ are linear in the vector $\Delta \pp_\calI$ and, in fact, it can be calculated using~\eqref{eq:flowsdc_model} as
%\[
%	\Delta \ff_\calI^\calB:= B_\calI C^T_\calI L^\dag_\calI \Delta \pp_\calI,
%\]
%where all the matrices refer to the subgraph $\calI$. The matrix $K^\calB$ is calculated exactly as the matrix product $B_\calI C^T_\calI L^\dag_\calI$, as proved in \cite[Proposition 15]{TPS2}. 
%
%The following result fully characterizes the nonzero components of $\Delta \ff_\calI^\calB$, the vector describing the net flow changes due to the balancing rule $\calB$, in view of the structure of the island $\calI$ and the positioning of the participating nodes.
%
%\begin{prop}\label{prop:cut_failure_par}
%For every surviving line $e \in E_\calI \setminus \calE_\calI$ in the island $\calI$, the power change on that line satisfies $(\Delta \ff_\calI^\calB)_{e}\neq 0$ ``if'' and only if there exists a path in $\calI$ from the disconnection node $u$ to a participating node $j \in \calN_\calB$ that contains line $e$.
%\end{prop}
%
%\textbf{Remark} \textit{The ``if'' part should be interpreted as an almost sure event with respect to a probability measure $\mu$ on $\R^m$ absolutely continuous with respect to the Lebesgue measure. The measure $\mu$ captures minor perturbations of the line susceptances (due for instance to manufacturing or measurement errors) and is instrumental to resolve pathological symmetry cases, see~\cite{TPS2} for more details.}
%% i.e., if $e$ and $\hat{e}$ belong to the same cell, then
%%$$
%%\mu(K_{e\hat{e}}^{\calE}\neq 0) = 1.
%%$$
%%We refer the readers to [TPS Part 2] for more details on $\mu$. 
%
%Proposition~\ref{prop:cut_failure_par} shows that the positions of participating nodes in $\calI$ play an important role in distributing imbalanced power within the island, since the balancing rule $\calB$ determines a change in the flow on every edge lying in a path connecting the disconnection node $u$ to the participating nodes. 
%%As a result, if $\hat{e}$ is a bridge that originally connects two islands $\calI_1$ and $\calI_2$ in $\calI$, then assuming $u\in\calI_1$, we see that $(\Delta \ff_\calI^\calB)_{\hat{e}}\neq 0$ ``if'' and only if $\calI_2$ contains a participating node since a path from $u$ to any node in $\calI_2$ must pass through $\hat{e}$.
%
%%\alec{REVISE} \lguo{Maybe we can just remove this paragraph} In fact, as shown in~\cite{TPS2}, for a typical power grid, the participating nodes often belong to different blocks of $\calI$, and, hence, for every edge $\hat{e}$ in $\calI$, we can find a participating node that passes through $\hat{e}$ and connects to $u$. In other words, for a typical grid, we have $(\Delta \ff_\calI^\calB)_{\hat{e}}\neq 0$ $\mu$-a.s.~for \emph{every} edge $\hat{e}$ in $\calI$, see~\cite{TPS2} for a more detailed discussion on this global propagation phenomenon.
%
%%\begin{defn}\label{defn:participating}
%%For a power grid $\calG$ with tree partition $\calP=\set{\calN_1,\calN_2,\cdots, \calN_k}$ operating under power balance rule $\calB$, a region $\calN_i$ with block decomposition $\set{\calC_{1}^i, \calC_2^i, \cdots, \calC_{m_i}^i}$ is said to be a \textbf{participating region} if $\calN_{\calB}\cap \calC^i_j$ contains a non-cut-vertex for $j=1,2,\ldots, m_i$. The grid $\calG$ is said to be a \textbf{participating grid} if $\calN_i$ is participating for  $i=1,2,\ldots,k$.
%%\end{defn}
%%A typical power grid does not contain single-point vulnerabilities such as cut vertices, which often suggests that the tree partition regions consist of single cells. In this case, a region is a participating region if there exists at least one node in this region that participates in power balancing and is not the endpoint of a bridge, which is often satisfied. It is thus reasonable to assume most tree partition regions are participating regions and hence most grids are participating. 
%%%For instance, if all generators participate in AGC, and load-side participation is implemented at all load nodes, then every node in the network is a participating node, and hence the grid is clearly participating. The following result shows that a region being participating implies all edges in this region are impacted when the original bridge $e$ is tripped.
%%\begin{prop}\label{prop:bridge_prop}
%%Consider a participating power network $\calG$ with island-free injection $\pp$. If $e$ is a bridge of $\calG$, then for any $\hat{e}\neq e$, we have
%%$$
%%\mu(K_{e\hat{e}}\neq 0)=1.
%%$$
%%\end{prop}
%%\lguo{I do not want to introduce the island-free concept here as this section is already too lengthy. Should we remove this proposition totally?}
%
%\subsubsection{Power Redistribution within Blocks}
%Lastly, we consider the second term in~\eqref{eqn:new_flow_change_decomp}, which is due to the redistribution of the power originally flowing on the failed lines. 
%
%Recall that, as far as this redistribution term is concerned, we can consider the island $\calI$ in isolation. Consider the block decomposition $E_1\cup E_2\cup\dots \cup E_k$ of the edges $E_\calI$ in that island, which is well-defined since $\calE_\calI$ is not a cut set and hence does not contain any bridge. Then, the following result holds:
%\begin{prop}\label{prop:multi_line_cell}
%Modulo rows/columns permutations, the matrix $K^\calR$ is a block-diagonal matrix of the form
%$$
%K^\calR=\begin{bmatrix}
%H_{1}& 0& \cdots& 0\\
%0 & H_{2} & \cdots & 0\\
%\vdots & \vdots & \ddots & \vdots\\
%0 & 0 &\cdots & H_{k}
%\end{bmatrix},
%$$
%where $H_{i}$ is a $\abs{E_i} \times \abs{E_i}$ matrix for every $i=1,2,\dots, k$. Moreover, each matrix $H_{i}$ has only nonzero entries $\mu$-a.s., namely for every $e_1,e_2=1,2,\dots, m_i$ we have
%$$
%\mu((H_{i})_{e_1 e_2}\neq 0) = 1.
%$$
%\end{prop}
%This result shows that the impact of power redistribution as captured by $K^\calR$ propagates exactly according to the block decomposition of $G$. In particular, the $(\hat{e}, e)$-th entry of $K^\calR$ is nonzero ``if'' and only if $e$ and $\hat{e}$ belong to the same block (where the ``if'' part should be interpreted as an almost sure event in $\mu$).
%
%Since the block decomposition is by construction finer than that of any tree partition, it immediately follows that failures can propagate only within the region they initially occurred.}
%
%\alew{
%The next result is analogous to the Simple Cycle Criterion for non-cut set outages.  It says that all ($\mu$-almost surely), and only, lines on a path between node $\hat j$ and every participating node $k\in N_{\hat j}$ with $\alpha_k>0$ will be impacted by the bridge $\hat \ell$ outage.  A simple path is a path that visits each node at most once.
%\begin{thm}[Simple Path Criterion: bridge outage]
%\label{ch:cf; subsec:bridgeoutage; theorem:simplepath}
%Suppose a single bridge $\hat \ell = (\hat i, \hat j)$ with $f_{\hat \ell}\neq 0$ trips and separates the network into two islands.
%For any line $\ell$ in the island $G_{\hat j}$ and under the proportional control $\mathbb G_\alpha$
%in \eqref{ch:cf; subsec:bridgeoutage; eq:Galpha.1}, $K_{\ell\hat \ell} \neq 0$ ``if'' and only if there exists
%a simple path in $G_{\hat j}$ from $\hat j$ to a participating node $k\in N_{\hat j}$ with $\alpha_k>0$ that
%contains $\ell$.
%\end{thm}
%
%The Simple Path Criterion prescribes exactly which lines in the island $G_{\hat j}$ will be impacted by a bridge $\hat \ell$ outage, as illustrated in Fig. \ref{ch:cf; sec:treepartitioning; fig:SimplePathCriterion} and its caption.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{figure}[!htbp]
%%\centering
%%   %\includegraphics[width=0.75\textwidth] {figures-ee135Notes/ee135Notes-fig-SimplePathCriterion.pdf}
%%\caption{Simple Path Criterion on the island $G_{\hat j}$ with node $\hat j$ in red.  Each shaded bubble denotes a non-bridge block of $G_{\hat j}$.  A block with a red boundary means that all lines in the block will be impacted $\mu$-almost surely by the outage of $\hat \ell$. Each node shaded in green in a bubble denotes a participating node. Node $v$ is a cut-vertex participating node. Line $\ell$ is in $E_{\text b}$ with the sub-island $G^\ell_{\hat j\hat j}$ as indicated.  The set $E^\ell_{\hat j\hat j}$ contains lines in block $B^v$ but not $E_{\hat j2}, \dots, E_{\hat j K}$ because no simple paths connecting node $\hat j$ and the participating node in $E_{\hat j 1}$ traverses blocks $E_{\hat j2}, \dots, E_{\hat j K}$. Cut vertex $v$ is in $N_{\textup{cv}}$ with sub-island $G^v_{\hat j\hat j}$ as indicated.  The set $E_{\hat j0}$ consists of all lines in $G^v_{\hat j\hat j}$ as well as lines connecting $G^v_{\hat j\hat j}$ and $v$, and in block $B^v$ as well as $\ell$, but not those in $E_{\hat j2}, \dots, E_{\hat j K}$ in the sub-island $G^\ell_{\hat j\hat j}$. Theorem \ref{ch:cf; subsec:bridgeoutage; theorem:simplepath} implies that all lines in $E_{\hat j0}$ and $E_{\hat j1}$ will be ($\mu$-almost surely) impacted and none in blocks $E_{\hat j2}, \dots, E_{\hat j K}$ will be as they contain no participating node.  Note that even though the block $G^v_{\hat j\hat j}$ contains no participating node, all lines in $G^v_{\hat j\hat j}$ will be impacted since they are on simple paths from $\hat j$ to some participating nodes.}
%%\label{ch:cf; sec:treepartitioning; fig:SimplePathCriterion}
%%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Let $E_{\text b} \subseteq E_{\hat j}$ be the set of all bridges $\ell$ in island $G_{\hat j}$ each of which 
%separates $G_{\hat j}$ into two sub-islands, $G^\ell_{\hat j\hat j}$ that contains node $\hat j$ and $G^\ell_{\hat j k}$ that contains a participating node $k$ with $\alpha_{k}>0$. There is a unique set of blocks in island $G^\ell_{\hat j\hat j}$ that every \emph{simple} path connecting nodes $\hat j$ and $k$ traverses. {\color{red} Is this claim true (it seems so)?  If it's true, is there a citation (it seems easy to prove too)?}
%Let $E^\ell_{\hat j}$ consist of all lines in these blocks as well as line $\ell$; see the caption of 
%Fig. \ref{ch:cf; sec:treepartitioning; fig:SimplePathCriterion} for illustration. Then since $G_{\hat j}$ is connected, for every line $\ell'\in E^\ell_{\hat j}$ (including $\ell' = \ell$), there is a simple path from $\hat j$ to the participating node $k$ that contains line $\ell'$ and hence Theorem \ref{ch:cf; subsec:bridgeoutage; theorem:simplepath} guarantees that $K_{\ell' \hat \ell}\neq 0$ $\mu$-almost surely.  
%Similarly let $N_\textup{cv} \subseteq N_{\hat j}$ consist of two types of nodes: (1) all cut vertices $v$ in island $G_{\hat j}$ each of which separates $G_{\hat j}$ into two sub-islands, $G^v_{\hat j\hat j}$ that contains node $\hat j$ and $G^v_{\hat j k}$ that contains a participating node $k$ with $\alpha_{k}>0$; and (2) all leaf nodes $k$ of island $G_{\hat j}$ that are participating nodes whose removal leaves $G_{\hat j}$ as a single connected component $G^v_{\hat j\hat j}$ that contains $\hat j$. Again there is a unique set of blocks in $G^v_{\hat j\hat j}$ that every simple path connecting nodes $\hat j$ and the participating node $k$ traverses. 
%Let $E^v_{\hat j}$ consist of all lines in these blocks as well as all lines connecting $G^v_{\hat j\hat j}$ to node $v$. Then, for every line $\ell'\in E^v_{\hat j}$, there is a simple path from $\hat j$ to a participating node $k$ that contains line $\ell'$ and hence Theorem \ref{ch:cf; subsec:bridgeoutage; theorem:simplepath} guarantees that $K_{\ell' \hat \ell}\neq 0$ $\mu$-almost surely. Let
%\[
%E_{\hat j 0} := \left( {\displaystyle\cup}_{\ell\in E_{\text b}} \, E^\ell_{\hat j} \right) \ \cup \ 
%		\left( {\displaystyle\cup}_{v\in N_{\textup{cv}}}\, E^v_{\hat j} \right)
%\]
%Hence every line in $E_{\hat j0}$ is on a simple path from $\hat j$ to a participating node that may contain a bridge in $E_{\text b}$ or a cut vertex in $N_{\textup{cv}}$ and therefore will be impacted by the outage of $\hat \ell$. Decompose the remaining lines $E_{\hat j}\!\setminus\! E_{\hat j 0}$ in island $G_{\hat j}$ into blocks $E_{\hat j1}, \dots, E_{\hat j K}$. Then Theorem \ref{ch:cf; subsec:bridgeoutage; theorem:simplepath} implies the following characterization of $K_{\ell\hat \ell}$.
%
%\begin{cor}
%\label{ch:cf; subsec:bridgeoutage; corollary:bridgeoutage}
%Suppose a single bridge $\hat \ell = (\hat i, \hat j)$ trips and separates the network into two islands. Partition the lines in island $G_{\hat j}$ into disjoint sets $E_{\hat j0}$, and blocks $E_{\hat j1}, \dots, E_{\hat j K}$ as described above. For any line $\ell$ in island $G_{\hat j}$ and under the proportional control $\mathbb G_\alpha$ in \eqref{ch:cf; subsec:bridgeoutage; eq:Galpha.1}, $K_{\ell\hat \ell}\neq 0$ ``if'' and only if $\ell\in E_{\hat j0}$ or $\ell$ is in a block $E_k$ that contains a participating node $i$ with $\alpha_i>0$ that is not a cut vertex. In particular, $K_{\ell\hat \ell}\neq 0$ ``if'' every block contains a participating node that is not a cut vertex. 
%\end{cor}
%}

==> arxiv submission/modeldescription.tex <==
\section{Power network model description}

We describe a power transmission network as a directed graph $G=(V,E)$, where $V=\set{1,\ldots, n}$ is the set of nodes (modeling \textit{buses}) and $E\subset V \times V$ is the set of edges (modeling \textit{transmission lines}). Denote by $n=|V|$ the number of nodes and by $m=|E|$ the number of edges of the network $G$. 

We assume $G$ to be connected and simple. Each edge $e=(i,j) \in E$ has a weight $\b_e=\b_{ij}$, which models the \textit{susceptance} of the corresponding line. Denote by $B$ the $m \times m$ diagonal matrix with entries $\b_1,\dots,\b_m$, where an arbitrary but fixed order has been chosen for the edge set $E$. The vertex-edge incidence matrix of $G$ is the $n\times m$ matrix $C$ defined as
$$
C_{ie}=\begin{cases}
  1 & \text{if vertex }i\text{ is the source of }e,\\
  -1 & \text{if vertex }i\text{ is the target of }e,\\
  0 &\text{otherwise.}
\end{cases}
$$
The \textit{weighted Laplacian matrix} of the graph $G$ is the symmetric $n \times n$ matrix $L$ defined as $L=C B C^T$ or equivalently as
\[
    L_{i,j} :=
    \begin{cases}
    		\sum_{k \neq i} \b_{i k} 		& \text{ if } i=j,\\
		- \b_{ij}  							& \text{ if } i \neq j.
	\end{cases}
\]
Denote by $\l_1, \l_2 , \dots, \l_{n}$ its eigenvalues and by $v_1,v_2,\dots,v_n$ the corresponding eigenvectors, which we can take to be pairwise orthogonal. It is well-known that $L$ is a real symmetric positive semi-definite matrix, which means that it has a real non-negative spectrum, i.e.,~$0 \leq \l_1 \leq \dots \leq \l_{n}$. All the rows of $L$ sum up to zero and thus the matrix $L$ is singular. 

If $G$ is connected, the eigenvalue $\l_1=0$ has multiplicity one and the corresponding eigenvector $v_1$ is the vector with all unit entries, which we denote by $\bm{1} \in \R^n$. In this case, using the eigenspace structure of $L$, the \textit{Moore-Penrose pseudoinverse} $L^+$ can be calculated as
\[
	L^+ :=\left  (L+ \frac{\bm{1}\bm{1}^T}{n}\right )^{-1} -\frac{\bm{1}\bm{1}^T}{n}.
\]
The matrix $L^+$ is also real, symmetric, and positive semi-definite and its spectrum is $0 < \l_n^{-1} \leq \dots \leq \l_2^{-1}$. For further spectral properties of graphs, we refer the reader to~\cite{RanjanZhangBoley2014,VanMieghem2011}.

In general, a power network $G$ may not be connected graph at all times (either by operational choice or in response to severe contingencies). In this case, in the power system literature the connected components $G_1,\dots, G_k$ of $G$ are usually referred to as \textit{islands}.

Denote by $p \in \R^{n}$ the vector of power injections, where the entry $p_i$ models the power generated (if $p_i>0$) or consumed (if $p_i<0$) at node $i$. We say that a power injection vector $p \in \R^n$ is \textit{balanced} if in every island of the power network, the net power injection is equal to zero, i.e., $\sum_{i \in G_j} p_i = 0$, for $i=1\dots,k$. %If $G$ is connected, the power injection vector is balanced if $\mathbf{1}^T p=0$. 

Given an oriented edge $e=(i,j)$, we denote the power flow on that line interchangeably as $f_e$ or $f_{ij}$. Note that the power flow on a given line is negative if the current flows in the opposite direction with respect to the edge orientation; therefore, with a minor abuse of notation we have $f_e=f_{ij}=-f_{ji}$.

The power flows on the lines are uniquely determined by the injections and physical properties of the network. More specifically, denoting by $f \in \R^m$ the power flow vector, the DC power flow model can be written as
\begin{equation}
\label{eqn:dc_model}
	f =BC^T L^+ p.
\end{equation}
The slack bus phase angle in $\theta$ is typically set to $0$ as a reference to other buses. With this convention, the DC model \eqref{eqn:dc_model} has a unique solution $\theta$ and $f$ for each balanced injection vector $p$.

%\begin{figure}
%\centering
%\includegraphics[width=.275\textwidth]{spanning_forest.png}
%\caption{An example element in $\calT(\calV_1,\calV_2)$, where circles correspond to elements in $\calV_1$ and squares correspond to elements in $\calV_2$. The two trees containing $\calV_1$ and $\calV_2$ are highlighted as solid lines.}\label{fig:spanning_forest}
%\end{figure}

Therefore, differently from many other man-made networks, the network operator does not directly control the power flows routing, but we can only indirectly change them by modifying the power injections or the network topology. This peculiar feature is one of the reason why is particularly challenging to study and improve the reliability of power systems and their robustness against failures. Indeed, when a subset of lines $\calE$ is tripped or fails, the network topology changes and, as a consequence, the power flow redistributes on the surviving graph $G'=(V,E\bs\calE)$, possibly causing overloads in other lines, not necessarily adjacent to the removed ones in $\calE$. 

If the power injections are still balanced for $G'$, the new power flows can be calculated directly from~\eqref{eqn:dc_model} after having updated the matrices $B$, $C$, and $L$. If the removal of the lines in $\calE$ created a new island, then the network operator has to intervene and modify some of the power injections to ensure that they are balanced again.

%In the case of the failure of a single line, i.e. $\calE=\{e\}$, if $G'$ is still connected, then the branch flow change on any other line $\widetilde{e} \neq e$ is given as
%$$
%	\Delta f_{\hat{e}} = f_e \cdot K_{e\widetilde{e}},
%$$
%where $K_{e\widetilde{e}}$ is the \emph{line outage distribution factor} \cite{Wood1996} from $e$ to $\widetilde{e}$ \lguo{Do we want to do cut set and non-cut set failure here instead since $\calE$ is a set of edges? See part II of the TPS paper for the full theory in this case} \alec{Yes!}. It is known that the line outage distribution factors are independent of the original power injections $p$ and depend only on the network topology; in fact, they can be computed from the matrices $B$ and $C$ as showed in~\cite{Wood1996}.
%\alec{Need to explain cascade mechanism here and typical non-local failure propagation}

==> arxiv submission/numerics.tex <==
\section{Numerical examples}
\label{sec:numerics}
%{\color{green} [Adam: I had been imagining this as the last subsection of the section 3, but this is okay too... Do you like it better separated out completely?]}
This section is devoted to the implementation of the bridge-block decomposition refinement strategy introduced in Section~\ref{sec:optimization}. In Subsection~\ref{sub:networkanalysis} we first review  the structural properties of several power grids used in the literature as test networks, from which it becomes evident the need of finer and more homogeneous bridge-blocks for these networks. In Subsection~\ref{sub:modnum} we introduce two fast approximations algorithms to find locally optimal solutions for the OBI problem~\eqref{eq:maxmodprob} and compare their performance on IEEE test networks in terms of the clusters' size and cross-edges. Then, in Subsection~\ref{sub:switchingnum}, we compare the performances of the one-shot algorithm and of its recursive variant for the same test networks.

%hose goal is to identify the candidate tree partition regions by finding a modularity-maximizing clustering of the network.

\subsection{Preliminary analysis of power systems topologies}
\label{sub:networkanalysis}
In order to show the potential benefits of applying our method for improving network reliability, it is important to first understand the relevant structural properties of typical power networks, in particular their bridge-block decomposition. In Table~\ref{tab:networkstatistics} below we report statistics about the original topologies of various standard test networks taken from~\cite{pglibopf,pglibopf_git}. For each of these networks, we find all its bridges and calculate its bridge-block decomposition. Modulo some minor variations, all the networks exhibit the same topological features, namely:
\begin{itemize}
    \item They have only one giant bridge-block that comprises a vast majority of the network nodes;
    \item They have substantial number of edges that are bridges (on average roughly $18\%$), each of them connecting a trivial bridge-block (consisting of one or two nodes) to the aforementioned giant bridge-block.
\end{itemize}
These features are also easily recognizable for the IEEE 118-bus network displayed in Fig.~\ref{fig:influencegraph_pre}. From these statistics it is clear that most power networks have an essentially trivial bridge-block decomposition and would thus perform very poorly in terms of failure localization. In particular, a line failure inside the unique giant bridge-block could propagate to roughly $80\%$ of the other lines (i.e., those in the same bridge-block).
Moreover, we note that all these networks already have a surprisingly large fraction (on average $\sim 18\%$) of lines that are bridges, which the switching actions prescribed by our method would increase only marginally.

\begin{table}[!ht]
    \centering
\begin{tabular}{c|r|r|C{2.35cm}|r|C{3.1cm}}
Test network case & \# of edges & \# of bridges & \% of edges that are bridges & \# of bridge-blocks &  Size(s) of non-trivial bridge-blocks \\
\hline \hline
case14\_ieee             &     20 &        1 &  5.00    &               2 &             13 \\
case30\_ieee             &     41 &        3 &  7.32    &               4 &             27 \\
case39\_epri             &     46 &       11 &  23.91   &               12 &             28 \\
case57\_ieee             &     80 &        1 &  1.25    &               2 &             56 \\
case73\_ieee\_rts        &    120 &        2 &  1.67    &               3 &             71 \\
case89\_pegase           &    210 &       16 &  7.62    &               17 &             73 \\
case118\_ieee            &    186 &        9 &  4.84    &               10 &             109 \\
case162\_ieee\_dtc       &    284 &       12 &  4.22    &             13 &             150 \\
case179\_goc             &    263 &       43 &  16.35   &             44 &             136 \\
case200\_activ           &    245 &       72 &  29.39   &             73 &             128 \\
case240\_pserc           &    448 &       58 &  12.95   &             59 &             182 \\
case300\_ieee            &    411 &       89 &  21.65   &             90 &             206, 3, 3 \\
case588\_sdet            &    686 &      229 &  33.38   &            230 &             357 \\
case793\_goc             &    913 &      290 &  31.76   &            291 &             500 \\
case1354\_pegase         &   1991 &      561 &  28.18   &            562 &             791 \\
case1888\_rte            &   2531 &      964 &  38.09   &            965 &             918, 5 \\
case2000\_goc            &   3633 &      445 &  12.25   &          446 &             1555 \\
case2736sp\_k            &   3273 &      627 &  19.16   &            628 &             2109 \\
case2737sop\_k           &   3274 &      627 &  19.15   &            628 &             2110 \\
case2746wp\_k            &   3281 &      637 &  19.41   &          638 &             2109 \\
case2746wop\_k           &   3309 &      607 &  18.34   &           608 &             2139 \\
case2848\_rte            &   3776 &     1410 &  37.34   &           1411 &             1421, 7, 5, 3 \\
case2869\_pegase         &   4582 &      778 &  16.98   &            779 &             2088 \\
case3120sp\_k            &   3693 &      731 &  19.79   &            732 &             2382, 8 \\
case3375wp\_k            &   4161 &      826 &  19.85   &            827 &             2536, 3 \\
case9241\_pegase         &  16049 &     1665 &  10.37   &           1666 &             7558, 7, 5, 3
\end{tabular}
    \caption{Summary of bridge and bridge-block statistics for various test networks. A bridge-block is considered to be non-trivial is it consists of strictly more than two nodes.}
    \label{tab:networkstatistics}
\end{table}

\subsection{Bridge-block candidate identification}
\label{sub:modnum}
The OBI problem that we introduced in Section~\ref{sub:mod} to find good candidate bridge-blocks is a variant of the well-known weighted network modularity maximization. However, this optimization problem cannot be solved exactly, being NP-hard, especially for large power networks and we need to resort to locally optimal partition. Before presenting our numerical findings, we first briefly review the two approximation algorithms that we implemented, namely the \textit{fastgreedy method} and the \textit{spectral clustering}.\\

\textbf{Fastgreedy.} A very fast approximation algorithm for optimizing modularity on large networks was proposed by~\cite{Clauset2004}. It uses a bottom-up hierarchical approach that tries to optimize the modularity in a greedy manner. Initially, every vertex belongs to a separate community, and communities are merged iteratively such that each merger is locally optimal (i.e., yields the largest increase in the current value of modularity). We use the Python library $\mathrm{igraph}$ and the built-in implementation of $\mathrm{fastgreedy}$ modularity optimization algorithm described in~\cite{Clauset2004}, which also implements some improvements proposed by~\cite{Wakita2007}.\\

\textbf{Spectral clustering.} Spectral clustering was first used in the context of modularity maximization by~\cite{Newman2006a,Newman2006b} and has become one of the most popular modern clustering algorithms, being simple to implement and very efficient to solve using standard linear algebra software. In our implementation of this method we use two matrices that simultaneously capture the network structure and flow pattern, the modularity matrix and the weighted Laplacian matrix. They can be both calculated from the graph $G=(V,E)$ with edge weights equal the absolute power flows $\{|f_{ij}|\}_{(i,j)\in \calE}$ as follows:
\begin{itemize}
    \item the \textit{modularity matrix} $B$, whose $(i,j)$ entry is $B_{i,j}= |f_{ij}|-\frac {F_{i} F_{j}}{2 M}$, and
    \item the \textit{weighted Laplacian matrix} $L$, whose entries are $L_{i,j}= -|f_{ij}|$ if $i\neq j$ and $L_{i,i}=-\sum_{j \neq i} L_{i,j}$.
\end{itemize} 
In both cases we choose to work with their normalized counterparts, namely
$$B_n := W^{-1/2} B W^{-1/2} \qquad \text{ and } \qquad L_n := W^{-1/2} L W^{-1/2},$$
where $W=\mathrm{diag}(F_1,\dots,F_n)$, since, especially in graphs of large size or with very heterogeneous weights, it has been argued that the spectral clustering method is more effective and computationally more stable when using the normalized version of these matrices, see~\cite{Bolla2011,vonLuxburg2007}.

The spectral clustering performed on the normalized Laplacian matrix $L_n$ approximates the optimal solution of the NP-hard problem known as \textit{Normalized Cut (NCut)}. Working with the normalized modularity matrix $B_n$ means that the spectral clustering method approximates the partition that maximizes a renormalized version $Q_n$ of the network modularity, namely
\[
	Q_n(\calP) := \frac {1}{2 M} \sum_{r=1}^{|\calP|} \frac{1}{\sum_{k \in \calV_r} |F_{k}|} \sum \limits _{i,j \in \calV_r}  \left ( |f_{ij}| - \frac {F_{i} F_{j}}{2 M} \right ).
\]
%\alec{Shall we formulate the OBI problem directly in terms of the normalized modularity?}
If we fix the target number $b$ of clusters the optimal normalized modularity clustering is equal to the normalized cut clustering, in the sense that $\arg\max_\calP Q_n(\calP)= \arg\min_\calP \mathrm{NCut}(\calP)$. This follows from the identity
\[
	Q_n(\calP) = \frac{b-1}{2M} - \frac{1}{2M} \mathrm{NCut}(\calP),
\]
proved in~\cite{Bolla2011,YuDing2010} under the assumption that the target number $b$ of clusters is fixed. This means that the spectral clustering method performed on either matrix $B_n$ and $L_n$ solve approximately the same optimization problem. However, having different eigensystems, they often yield to slightly different results. For this reason, we consider both of these two variants of the spectral clustering approximation method in the following subsection and label them as \textit{Spectral $L_n$} and \textit{Spectral $B_n$}.

We remark that the authors in~\cite{Bialek2014} also adopt the normalized-Laplacian-based spectral clustering to power systems, proposing several choices for the edge weights, including the one we adopted in this paper, i.e., the absolute value of power flows. In the same paper, some heuristics are outlined to decide the optimal number of clusters in which to partition the network, but these leverage the eigensystem structure of the Laplacian matrix, rather than being informed by a specific target number of clusters $b$ like in our method.

% As proved by~\cite{YuDing2010,Bolla2011}, for a fixed number $b$ of clusters, the following identity holds
% \[
% 	Q_n(\calP)= \frac{b-1}{2M} - \frac{1}{2M} \mathrm{NCut}(\calP).
% \]
% Hence, the normalized modularity clustering is equivalent to NCut introduced earlier in~\eqref{eq:ncut}, in the sense that $\arg\max_\calP Q_n(\calP)= \arg\min_\calP \mathrm{NCut}(\calP)$. 
% %and, for this reason, we will refer to this second variant of the spectral method as $\mathrm{NCut}$.
% The generalization to $k$-way clustering is immediate and can be implemented in a similar way as already done in the literature when the clustering is based on the graph Laplacian matrix $L$~\alec{REFS HERE}. 

% The spectral clustering approaches leverage an alternative matrix formulation of the network modularity, which we briefly illustrate in the case of a bipartition $\calP=\{\calV,\calV^c\}$. In this case the weighted network modularity rewrites as
% %\begin{equation}
% %	Q(\calV)= \frac {1}{2 M} \sum \limits _{i,j \in V} \left ( w_{ij}-\frac {w_{i} w_{j}}{2 M} \right )(s_i s_j  +1) = \frac {1}{2 M} \sum \limits _{i,j \in V} \left ( w_{ij}-\frac {w_{i} w_{j}}{2 M} \right )s_i s_j,
% %\end{equation}
% $$
% 	Q(\calP)= \frac {1}{2 M} \bm{s}^T B \bm{s}, 
% $$
% where $\bm{s} = \bm{s}(\calP) \in \{-1,+1\}^n$ is the vector encoding the partition $\calP$, and $B \in \R^{n \times n}$ is the so-called \textit{modularity matrix}, whose $(i,j)$-th element is $B_{i,j}= |f_{ij}|-\frac {F_{i} F_{j}}{2 M}$. 
% %The matrix $B$ has an eigenvector $\mathbf{1}=(1,\dots,1)$ with eigenvalue $0$ and its spectrum is in fact intimately related with that of the weighted graph Laplacian (for more details see~\cite{Jiang2015,Newman2013}).

% The main idea behind spectral clustering is to approximate the exact solution of the network modularity maximization problem $\arg\max_{\calP} Q(\calP)$ by studying the spectrum of the modularity matrix $B$, more precisely by finding the solution of the following (relaxed) problem
% \begin{equation}
% \label{eq:spectralclustering}
% 	\arg\max_{\bm{s} \in \R^n, \bm{s}^T \bm{1}=0} \frac {1}{2 M} \bm{s}^T B \bm{s}.
% \end{equation}
%\alec{Alternative matrix formulation...useful particularly in spectral optimization algorithms, This function has the same form as the Hamiltonian of an Ising spin glass, a connection that has been exploited to create simple computer algorithms, for instance using simulated annealing, to maximize the modularity. The general form of the modularity for arbitrary numbers of communities is equivalent to a Potts spin glass and similar algorithms can be developed for this case also}
%We illustrate the basic idea of spectral clustering in the special case where we want to find the maximum modularity bipartition $\calV=\{\calV_1,\calV_2\}$ of a given graph $G$. The modularity can be rewritten as
%\begin{equation}
%\label{eq:Qspectral}
%	Q(\calV)= \frac {1}{2 M} \sum \limits _{i,j \in V} \left ( w_{ij}-\frac {w_{i} w_{j}}{2 M} \right )(s_i s_j  +1) = \frac {1}{2 M} \sum \limits _{i,j \in V} \left ( w_{ij}-\frac {w_{i} w_{j}}{2 M} \right )s_i s_j,
%\end{equation}
%where $\bm{s} = \bm{s}(\calV) \in \{-1,+1\}^n$ is the vector encoding the partition $\calV$, namely for $i=1,\dots,n$
%\[
%	s_i=
%	\begin{cases}
%	+1 & \text{ if } i \in \calV_1,\\
%	-1 & \text{ if } i \in \calV_2.\\
%	\end{cases}
%\]
%The expression in~\eqref{eq:Qspectral} can be further rewritten as
%\begin{equation}
%\label{eq:spectralclustering}
%	Q(\calV)= \frac {1}{2 M} \bm{s}^T B \bm{s}, 
%\end{equation}
%where $B$ is the so-called \textit{modularity matrix} of the weighted graph $G$, whose $(i,j)$-th element is $B_{i,j}= w_{ij}-\frac {w_{i} w_{j}}{2 M}$. The matrix $B$ has an eigenvector $\mathbf{1}=(1,\dots,1)$ with eigenvalue $0$ and its spectrum is in fact intimately related with that of the weighted graph Laplacian (for more details see~\cite{Jiang2015,Newman2013}). Spectral clustering is a way to find the solution of the problem
%\[
%	\argmax_{\bm{s} \in \{-1,+1\}^n} \frac {1}{2 M} \bm{s}^T B \bm{s}
%\]
%by solving its relaxed version, namely
%\[
%	\argmax_{\bm{s} \in \R^n, \bm{s}^T \bm{1}=0} \frac {1}{2 M} \bm{s}^T B \bm{s}
%\]

%Let $\b_1 \geq \dots \geq \b_n$ be the eigenvalues of $B$ and $\bf{u}_1,\dots,\bf{u}_n$ the corresponding eigenvectors. Rewriting the vector $s$ in this basis as $s = \sum_{i=1}^n a_i \bf{u}_i$, the objective function of the problem rewrites as
%\[
%	\frac {1}{2 M} \bm{s}^T B \bm{s} = \frac {1}{2 M} \sum_{i=1}^n a_i^2 \b_i,
%\]
%suggesting that in order to maximize the network modularity $Q(\calV)$, we should choose $\bm{s}$ proportionally to the leading eigenvector $\bm{u}_1$ (assuming that $\b_1 >0$) as proposed by~\cite{Newman2006b}. 

%\alec{Keep the following digression on the spectral clustering using Laplacian?}\\
%Spectral clustering has also been explored to approximated similar min-cut problems (e.g., RatioCut and NCut on weighted graphs) using the graph Laplacian matrix $L$ instead of $B$, see the review by~\cite{vonLuxburg2007}. In the same paper, there is an interesting discussion regarding the usage of normalized versus unnormalized version of the graph Laplacian matrix, arguing in favor of the first, which is also the only one proved to be statistically consistent~\cite{vonLuxburg2008}.

%Spectral clustering is a way to solve the relaxed versions of these problems, normalized for $\textrm{NCut}$~\cite{vonLuxburg2007}.
%
%Spectral method works for both cut minimization and modularity maximization, they just apply to different matrices.
%
%\ale{Overview spectral approximations for RatioCut and NCut on weighted graphs + comparision/discussion normalized vs. unnormalized ~\cite{vonLuxburg2007}}
%
%\ale{Explain why we keep the dangling/trivial bridges for modularity-maximization purposes.} Modularity maximization will not yield trivial clustering, that's one of the reason we chose it
%
%\alec{It's adaptive to changing power injections, modulo restarting from the full network}



%\ale{Usually $k$ is decided looking at the spectrum of the Laplacian and/or on local maxima of the modularity, we have a different approach}}

%\ale{Conditions under which the largest eigenvalue of $B$ is zero~\cite{Bolla2011}, namely ``A connected graph has the largest eigenvalue of the modularity matrix equal to zero if and only if it is a complete multipartite graph''}
%}

%\[
%	Q(\mathcal{V},p)={\frac {1}{2m(p)}} \sum_{r=1}^k \sum \limits _{i,j \in V_r} \left ( w_{ij}(p)-\frac {w_{i}(p)w_{j}(p)}{2m(p)} \right ),
%\]
%where $w_{ij}(p)=|f_{ij}(p)|$ is the absolute power flow on the line $(i,j) \in E$, $w_{i}(p)=\sum_{j} w_{ij}(p)=\sum_{j} |f_{ij}(p)|$ and $m(p) = \frac{1}{2} \sum_{i,j} w_{ij}(p)=\frac{1}{2} \sum_{i,j} |f_{ij}(p)|$.

%The modularity of a network partition measures the fraction of total edge weight within communities versus what one might expect if edges were placed randomly according to some null model. Modularity gives one definition of the ``quality'' of a partition, and maximizing modularity is supposed to yield a reasonable partitioning of a network into disjoint communities.
%
%Community detection is related to graph partitioning, which has been applied to problems in numerous areas [74,81,95]. In graph partitioning, a network is divided into disjoint sets of nodes. Graph partitioning usually requires the number of clusters to be specified to avoid trivial solutions, whereas modularity optimization does not require one to specify the number of clusters [76]. This is a desirable feature for applications such as social and biological networks.
%
%In [45], we interpret modularity optimization (using the Newman-Girvan null model [71, 73]) from a novel perspective. Inspired by the connection between graph cuts and the total variation (TV) of a graph partition, we reformulate the problem of modularity optimization as a minimization of an energy functional that consists of a graph cut (i.e., TV) term and an L2 balance term

%\subsection*{Random material Pt.1}
%\zok{Potts interpretation~\cite{Reichardt2006}

%Recall that, under the DC approximation, the line flows $f \in \R^m$ are fully determined by the power injections in the nodes $p \in \R^n$ via the linear relationship $f = f(p) = BC^T L^+ p$. The edge weights~\eqref{eq:powerweights} and thus the network modularity can both then be seen as functions of the power injections $p \in \R^n$ and, in multiple instances, it will be convenient to make this dependence explicit by writing $w_{ij}(p)=|f_{ij}(p)|$ and $Q(\mathcal{V},p)$, respectively.

%\ale{Normalized Laplacian matrix: why is it better?}

%\textbf{Other stuff}
%\ale{Current-Flow Betweenness Centrality -- it's similar to the node weights in our system\\ Mildly related, edge-betweenness it's used by Girvan and Newman divisive algorithm}

%We denote by $\calV^*$ the partition of the network $G$ that maximizes the network modularity, i.e.,
%\begin{equation}
%\label{eq:mod}
%	\calV^* = \arg\max_{\calV \in \Pi(G)} Q(\calV) = \arg\max_{\calV \in \Pi(G)}  \frac {1}{2 M} \sum_{r=1}^{|\calV|} \sum \limits _{i,j \in \calV_r} \left ( |f_{ij}|-\frac {|f_{i}| |f_{j}|}{2 M} \right ).
%\end{equation}
%In most cases, we are interested in finding the optimal partition when the number of clusters is fixed or bounded and thus we further require $\calV \in \Pi_k(G)$ or $\calV \in \Pi_{\leq k}(G)$, respectively.

%Of particular interest for us will be the scenario where we search for a bipartition of the network that is $\calV=\{C,C^c\}$ with $C \subseteq V$, in which the problem~\eqref{eq:mod} rewrites as
%\begin{equation}
%\label{eq:mod2}
%	\arg\max_{\calV \in \Pi_2(G)} Q(\calV) = \arg\max_{C \subseteq V}  \frac {1}{2 M} \left ( \sum \limits _{i,j \in C} \left ( |f_{ij}|-\frac {|f_{i}| |f_{j}|}{2 M} \right ) + \sum \limits _{i,j \in C^c} \left ( |f_{ij}|-\frac {|f_{i}| |f_{j}|}{2 M} \right ) \right ).
%\end{equation}

\subsubsection{Performance comparison}

We compare the performance of the three aforementioned clustering methods (FastGreedy, Spectral $L_n$ and Spectral $B_n$) to optimally partition some standard IEEE test cases available in the pglib-opf library~\cite{pglibopf,pglibopf_git}. We consider four networks of various sizes, ranging from small (39 nodes) to large (2737 nodes). 

We first consider the quality of the network partitions returned by three methods by looking exclusively at graph-related quantities. In the following tables, we report for different target number $b$ of clusters the normalized modularity score $Q_n$ (the higher the better) of the partition returned by each algorithm, as well as the sizes of the $b$ clusters and the fraction of edges that are cross-edges between them. We further report the number of cross-edges to be switched off to obtained a bridge-block decomposition with the identified clusters as bridge-blocks. Recall that, as we argued in Section~\ref{sub:mod}, it is highly desirable to have a small number of cross-edges between the identified clusters, since it dramatically reduces the feasible sets of switching actions for the OBS problem.

%\alec{Need to introduce (separately?) Tables 2,4,6,8 and talk about recursive splitting -- do it here or at the end of the section when we talk about the recursive structure?}
\begin{table}[!ht]
\centering
\begin{tabular}{c|C{1.1cm}|r|C{0.8cm}|C{1.7cm}|C{2cm}|C{3.8cm}}
\toprule
Clustering method & runtime (sec) & $b$ & $Q_n$ & fraction of cross-edges & \#lines to be switched off & resulting partition of the largest bridge-block\\
\hline \hline
Spectral $L_n$  &   0.0192 &  2 &   0.379 &               0.0869 &                    3 &                   [10, 18] \\
Spectral $B_n$ &   0.0186 &  2 &    0.406 &               0.0652 &                    2 &                   [11, 17] \\
FastGreedy  &  0.0016 &  2 &    0.406 &               0.0652 &                    2 &                   [11, 17] \\
\hline
Spectral $L_n$  &   0.0247&  3 &   0.486 &                0.152 &                    5 &                 [9, 9, 10] \\
Spectral $B_n$ &    0.0210 &  3 &   0.501 &                0.130 &                    4 &                 [8, 9, 11] \\
FastGreedy  &  0.0018 &  3 &   0.524 &                0.109 &                    3 &                [7, 10, 11] \\
\hline
Spectral $L_n$  &   0.0306 &  4 &   0.513 &                0.173 &                    5 &               [4, 7, 8, 9] \\
Spectral $B_n$ &   0.0291 &  4 &   0.527 &                0.196 &                    5 &               [4, 7, 8, 9] \\
FastGreedy  &  0.0027 &  4 &   0.535 &                0.152 &                    4 &              [4, 7, 7, 10] \\
\end{tabular}
\caption{39 EPRI}
\end{table}

\begin{table}[!ht]
\centering
\begin{tabular}{c|C{1.1cm}|r|C{0.8cm}|C{1.7cm}|C{2cm}|C{3.8cm}}
Clustering method & runtime (sec) & $b$ & $Q_n$ & fraction of cross-edges & \#lines to be switched off & resulting partition of largest bridge-block\\
\hline \hline
Spectral $L_n$  &    0.0255 &  2 &   0.220 &               0.032 &                    5 &                   [28, 81] \\
Spectral $B_n$ &   0.0294 &  2 &   0.390 &               0.032 &                    5 &                   [40, 69] \\
FastGreedy  &  0.0032 &  2 &   0.427 &               0.075 &                   13 &                   [50, 59] \\
\hline
Spectral $L_n$  &    0.0338 &  3 &   0.490 &               0.053 &                    8 &               [27, 33, 49] \\
Spectral $B_n$ &   0.0341 &  3 &   0.518 &               0.059 &                    9 &               [29, 38, 42] \\
FastGreedy  &  0.0061 &  3 &   0.527 &                0.102 &                   17 &               [16, 34, 59] \\
\hline
Spectral $L_n$  &  0.0366 &  4 &    0.498 &               0.075 &                   11 &            [9, 19, 33, 48] \\
Spectral $B_n$ &  0.0477 &  4 &   0.540 &                0.102 &                   16 &           [18, 21, 29, 41] \\
FastGreedy  &   0.0381 &  4 &   0.620 &                0.140 &                   23 &           [16, 27, 32, 34] \\
\end{tabular}
\caption{IEEE 118}
\end{table}

\begin{table}[!ht]
\centering
\begin{tabular}{c|C{1.1cm}|r|C{0.8cm}|C{1.7cm}|C{2cm}|C{3.8cm}}
Clustering method & runtime (sec) & $b$ & $Q_n$ & fraction of cross-edges & \#lines to be switched off & resulting partition of largest bridge-block\\
\hline \hline
Spectral $L_n$  &   0.912 &  2 & 0 &             0.0008 &                    1 &                   [1, 917] \\
Spectral $B_n$ &  0.844 &  2 &     0.483 &               0.0107 &                   26 &                 [391, 527] \\
FastGreedy  &  0.443 &  2 &      0.489&               0.0130 &                   32 &                 [415, 503] \\
\hline
Spectral $L_n$  &   7.536 &  3 &   0.610 &               0.0217 &                   51 &            [168, 356, 394] \\
Spectral $B_n$ &   1.201 &  3 &   0.648 &               0.0194 &                   46 &            [273, 308, 337] \\
FastGreedy  &  0.461 &  3 &   0.617 &                0.0198 &                   48 &            [205, 298, 415] \\
\hline
Spectral $L_n$  &  8.167 &  4 &     0.709 &               0.0221 &                   52 &       [187, 189, 222, 320] \\
Spectral $B_n$ &  5.693 &  4 &   0.709 &               0.0205 &                   48 &       [157, 204, 261, 296] \\
FastGreedy  &  1.028 &  4 &   0.724 &               0.0217 &                   52 &       [153, 205, 262, 298] \\
\end{tabular}
\caption{1888rte}
\end{table}

\begin{table}[!ht]
\centering
\begin{tabular}{c|C{1.1cm}|r|C{0.8cm}|C{1.7cm}|C{2cm}|C{3.8cm}}
Clustering method & runtime (sec) & $b$ & $Q_n$ & fraction of cross-edges & \#lines to be removed & resulting partition of largest bridge-block\\
\hline \hline
Spectral $L_n$  &   3.949 &  2 &   0.375 &              0.0076 &                   24 &                [674, 1436] \\
Spectral $B_n$ &    2.702 &  2 &    0.379 &               0.0058 &                   18 &                [690, 1420] \\
FastGreedy  &  0.606 &  2 &   0.461 &               0.0489 &                  159 &               [1000, 1110] \\
\hline
Spectral $L_n$  &   4.394 &  3 &   0.640 &               0.0150 &                   47 &            [659, 698, 753] \\
Spectral $B_n$ &   2.837 &  3 &   0.640 &               0.0159 &                   50 &            [667, 702, 741] \\
FastGreedy  &  0.987 &  3 &   0.632 &               0.0516 &                  167 &           [410, 590, 1110] \\
% \hline
% Spectral $L_n$	\\
% Spectral $B_n$	\\
% FastGreedy	
\end{tabular}
\caption{Polish 2737sop}
\end{table}
\FloatBarrier

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size &  \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.466 & \{14,25\} & 3 & 0.065 \\
% FastGreedy & 2 & 0.466 & \{14,25\} & 3 & 0.065 \\
% \hline
% Spectral & 3 & 0.580 & \{5,13,21\} & 5 & 0.1086\\
% FastGreedy & 3 & 0.646 & \{12,13,14\} & 5 & 0.1086\\
% \hline
% Spectral & 4 & 0.646 & \{3,7,11,18\} & 6 & 0.1304\\
% FastGreedy & 4 & 0.691 & \{6,8,12,13\} & 7 & 0.1521\\
% \hline 
% Spectral & 5 & 0.695 & \{3,4,7,12,13\} & 8 & 0.1739\\
% FastGreedy & 5 & 0.723 & \{5,6,7,8,13\} & 8 & 0.1739\\
% \end{tabular}
% \caption{IEEE 39}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size & \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.451 & \{37,81\} & 5 & 0.0267\\
% FastGreedy & 2 & 0.390 & \{33,85\} & 7 & 0.0376\\
% \hline 
% Spectral & 3 & 0.524 & \{12,37,69\} & 10 & 0.0538\\
% FastGreedy & 3 & 0.584 & \{27,33,58\} & 13 & 0.0699\\
% \hline 
% Spectral & 4 & 0.618 & \{12,16,30,60\} & 15 & 0.0806\\
% FastGreedy & 4 & 0.694 & \{15,27,33,43\} & 17 & 0.0914\\
% \hline 
% Spectral & 5 & 0.700 & \{12,16,21,32,37\} & 19 &  0.1022\\
% FastGreedy & 5 & 0.740 & \{15,21,22,27,33\} & 19 & 0.1022\\
% \end{tabular}
% \caption{IEEE 118}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size &  \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.475 & \{90,110\} & 8 &  0.0327\\
% FastGreedy & 2 & 0.471 & \{95,105\} & 11 & 0.0449\\
% \hline 
% Spectral & 3 & 0.559 & \{19,80,101\} & 12 & 0.0490 \\
% FastGreedy & 3 & 0.623 & \{46,59,95\} & 15 & 0.0612\\
% \hline 
% Spectral & 4 & 0.602 & \{23,52,56,69\} & 19 & 0.0776\\
% FastGreedy & 4 & 0.703 & \{35,46,59,60\} & 19 & 0.0776\\
% \hline 
% Spectral & 5 & 0.694 & \{23,29,48,48,52\} & 20 & 0.0816\\
% FastGreedy & 5 & 0.731 & \{26,33,35,46,60\} & 20 & 0.0816\\
% \end{tabular}
% \caption{IEEE 200}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size &  \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.481 & \{79,221\} & 3 & 0.0073\\
% FastGreedy & 2 & 0.491 & \{107,193\} & 11 & 0.0268\\
% \hline
% Spectral & 3 & 0.613 & \{35,79,186\} & 7 & 0.0170\\
% FastGreedy & 3 & 0.612 & \{76,107,117\} & 16 & 0.0389\\
% \hline
% Spectral & 4 & 0.648 & \{11,65,78,146\} & 14 & 0.0341\\
% FastGreedy & 4 & 0.716 & \{36,71,76,117\} & 22 &  0.0535\\
% \hline
% Spectral & 5 & 0.694 & \{11,17,69,72,131\} & 20 & 0.0487 \\
% FastGreedy & 5 & 0.759 & \{22,36,49,76,117\} & 28 & 0.0681\\
% \end{tabular}
% \caption{IEEE 300}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size &  \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.492 & \{646,708\} & 23 & 0.0116\\
% FastGreedy & 2 & 0.435 & \{505,849\} & 17 & 0.0085\\
% \hline
% Spectral & 3 & 0.641 & \{255,527,572\} & 29 & 0.0146\\
% FastGreedy & 3 & 0.649 & \{301,505,548\} & 35 & 0.0176\\
% \hline
% \textbf{Spectral} & 4 & 0.718 & \{253,281,390,430\} & 42 & 0.0211\\
% FastGreedy & 4 & 0.715 & \{239,301,309,505\} & 39 & 0.0196\\
% \hline
% Spectral & 5 & 0.685 & \{3,128,171,517,535\} & 33 & 0.0166\\
% FastGreedy & 5 & 0.757 & \{168,239,301,309,337\} & 58 & 0.0291\\
% \end{tabular}
% \caption{IEEE 1354pegase}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ & $Q$ & Clusters size &  \# cross-edges & \# cross-edges/$|E|$ \\ 
% \hline \hline
% Spectral & 2 & 0.403 & \{1010,1726\} & 30 & 0.0092\\
% FastGreedy & 2 & 0.462 & \{1270,1466\} & 84 & 0.0257\\
% \hline
% \textbf{Spectral} & 3 & 0.620 & \{677,933,1126\} & 52& 0.0159\\
% FastGreedy & 3 & 0.636 & \{601,865,1270\} & 128 & 0.0392\\
% \hline
% Spectral & 4 & 0.657 & \{434,557,667,1078\} & 70 & 0.0214\\
% FastGreedy & 4 & 0.710 & \{472,601,798,865\} & 129 & 0.0395\\
% \hline
% \textbf{Spectral} & 5 & 0.664 & \{128,403,478,667,1060\} & 77 &0.0236 \\
% FastGreedy & 5 & 0.760 & \{417,448,472,601,798\} & 161 & 0.0493\\
% \end{tabular}
% \caption{IEEE 2736sp, Polish network}
% \end{table}

In the vast majority of the considered cases, the two spectral clustering methods yield partitions with smaller values of the normalized modularity $Q_n$ with respect to the FastGreedy method, which, however, consistently returns partitions with a larger number of cross-edges than the other two methods. In our experiments, the FastGreedy method is considerably (2x-10x times) faster than the two spectral clustering methods. 

FastGreedy has the advantage that all the partitions for various $b$ are calculated jointly because the algorithm is nested in that each partition of size $b$ is obtained from the corresponding one of size $b-1$ by optimally dividing one of the clusters into two. This recursive nature of the FastGreedy method makes it faster, but at times it means that partitions with unbalanced clusters sizes could be returned. On the other hand, the two spectral clustering methods almost always identify partitions with clusters of balanced size.

In the cases considered above, all methods always yield partitions with exactly $b$ connected clusters. It is possible that the actual number of identified \textit{connected} clusters could be strictly larger than $b$ because some of them induce network subgraphs that are disconnected, violating our assumption (A1). This occurs very rarely as the OBI objective function severely penalizes such partitions, but even so it would not be an issue as it would lead to a finer bridge-block decomposition. 

% \begin{figure}
% \includegraphics[scale=0.4]{case2736sp_nice.png}
% \caption{The four candidate clusters of the 2736sp network found by the spectral clustering method}
% \end{figure}
% \FloatBarrier

\subsection{Performance of one-shot and recursive algorithms}
\label{sub:switchingnum}

% \subsubsection{Results for one-shot algorithm}
We first illustrate the numerical results for the one-shot algorithm, i.e., Algorithm~\ref{alg:oneshotrefinement}, for various test networks. 
More specifically, for each network we solve the OBS problem~\eqref{eq:optswitch_basic} three times, using the (possibly different) optimal partition $\calP$ into $b$ clusters returned by each of the three different clustering algorithms (cf.~Subsection~\ref{sub:modnum}). 
Recall that there is a one-to-one correspondence between the feasible subsets of cross-edges $\calE \subset E_c(\calP)$ and the spanning trees of the reduced multi-graph $G_\calP$. This means that the one-shot algorithm cannot be solve exactly already for partitions into $b \geq 5$ clusters, since the spanning trees of the reduced multi-graph grow exponentially with $b$. However, if we consider a small number of target clusters, say $b\leq 4$, we can still solve the OBS exactly by considering all possible spanning tree of $G_\calP$.

As pre-processing step, for each of the considered networks we first run a DC-OPF to obtain the power flow configuration and calculate the initial network congestion level $\gamma(\emptyset)$  (which is possibly equal to $1$ if one or more line limits are active for the OPF solution). We then run Algorithm~\ref{alg:oneshotrefinement} with $b=4$ using the three different clustering methods discussed in the previous section. Table~\ref{tab:one-shot_results} below reports for each network both the initial congestion level $\gamma(\emptyset)$ and the results of the one-shot algorithm ran with $b=4$ as target number of clusters. More specifically, for each network and each clustering algorithm, we report
\begin{itemize}
    \item the runtime,
    \item the number of spanning trees of $G_\calP$ considered,
    \item the optimal post-switching network congestion level $\gamma(\calE^*)$,
    \item the number of lines that to be switched off for the optimal set of switching actions $\calE^*$ and which fraction they represent on the total number of network lines.
\end{itemize}

\begin{table}[!ht]
    \centering
    \begin{tabular}{p{1.85cm}|p{2.1cm}|p{1.15cm}|p{1.6cm}|p{1cm}|p{1.85cm}|p{1.8cm}|p{1.8cm}}
network & partition method &  runtime (sec) & \# spanning trees &  $\gamma(\calE^*)$ & \# congested lines & \# of lines switched off & $\%$ of lines switched off\\
\hline \hline
\multirow{4}{*}{case39\_epri} 
& \multicolumn{2}{l}{initial network configuration} & - & 1.000 & 2 & - & -\\
\cline{2-8}
& Spectral $L_n$  &  0.238 &             10 &      0.960 &                0 &              3 &            6.52 \\
& Spectral $B_n$ &   0.270 &             10 &      0.960 &                0 &              3 &            6.52 \\
& \textbf{FastGreedy}  &  0.245 &             12 &  \textbf{0.833} &                \textbf{0} &              3 &            6.52 \\
\hline
\hline
\multirow{4}{*}{case57\_ieee} 
& \multicolumn{2}{l}{initial network configuration} & - & 0.938 & 0 & - & -\\ 
\cline{2-8}
& Spectral $L_n$  &   6.210 &            220 &   1.050 &                2 &             13 &            16.25 \\
& Spectral $B_n$ &   5.454 &            216 &   1.078 &                2 &             12 &            15.00 \\
& \textbf{FastGreedy}  &  6.829 &            256 &  \textbf{0.921} &                \textbf{0} &             14 &            17.50 \\
\hline
\hline
\multirow{4}{*}{case73\_ieee}
& \multicolumn{2}{l}{initial network configuration} & - & 0.632 & 0 & - & -\\
\cline{2-8}
& Spectral $L_n$  &   1.330 &             49 &   1.171 &                1 &              8 &           6.66 \\
& Spectral $B_n$ &   2.010 &             71 &   1.171 &                3 &             10 &           10.83 \\
& \textbf{FastGreedy}  &  0.970 &             31 &  \textbf{0.723} &                \textbf{0} &              6 &           5.00 \\
\hline
\hline
\multirow{4}{*}{case118\_ieee} 
& \multicolumn{2}{l}{initial network configuration} & - & 1.000 & 2 & - & - \\
\cline{2-8}
& \textbf{Spectral} $L_n$ &  1.912 &             80 &    \textbf{1.004} &                \textbf{2} &             10 &           5.38 \\
& Spectral $B_n$ &   2.259 &             80 &  1.016 &                3 &             10 &           5.38 \\
& FastGreedy  &  7.958 &            264 &  2.248 &                8 &             18 &           9.68 \\
\hline
\hline
\multirow{4}{*}{case179\_goc} 
& \multicolumn{2}{l}{initial network configuration} & - & 1.000 & 4 & - & -\\
\cline{2-8}
& Spectral $L_n$  &  1.699 &             54 &  1.243 &                7 &              7 &           2.66 \\
& Spectral $B_n$ &  10.358 &            312 &  1.035 &                2 &             13 &           4.94 \\
& \textbf{FastGreedy}  &  2.103 &             69 &  \textbf{1.000} &                \textbf{1} &              9 &            3.42 \\
\hline
\hline
\multirow{4}{*}{case200\_activ} 
& \multicolumn{2}{l}{initial network configuration} & - & 0.708 & 0 & - & -\\
\cline{2-8}
& Spectral $L_n$  &  6.541 &            196 &   0.591 &                0 &             15 &           6.12 \\
& Spectral $B_n$ &  9.146 &            312 &   0.591 &                0 &             16 &           6.53 \\
& \textbf{FastGreedy}  &  6.863 &            208 &   \textbf{0.591} &                \textbf{0} &             12 &           4.90 \\
\hline
\hline
\multirow{4}{*}{case300\_ieee} 
& \multicolumn{2}{l}{initial network configuration} & - & 1.000 & 11 & - & -\\
\cline{2-8}
& Spectral $L_n$  &  3.610 &            120 &  1.220 &                7 &             12 &           2.92 \\
& \textbf{Spectral} $B_n$ &  14.275 &            468 &  \textbf{1.058} &                \textbf{5} &             14 &           3.41 \\
& FastGreedy  &  37.212 &           1112 &  1.161 &                6 &             24 &           5.84 \\
\hline
\hline
    \end{tabular}
    \caption{Results obtained by the one-shot algorithm with $b=4$ target clusters using three different methods for the candidate bridge-blocks identification. We highlight in bold the best method and the resulting post-switching congestion $\gamma(\calE^*)$ for each network.}
    \label{tab:one-shot_results}
\end{table}
\FloatBarrier
From Table~\ref{tab:one-shot_results} we deduce that the resulting post-switching network congestion level varies a lot depending on the test network and partition method. In particular, in a few instances the maximum congestion is strictly bigger than $1$, but when considering all three methods, there is always at least one solution that does not increase the congestion significantly. Furthermore, in many instances the post-switching network congestion level even decreases with respect to the initial configuration and so does the number of congested lines. 

We did not run the one-shot algorithm on larger networks, as it would have required a substantially (exponentially) larger amount of time. This is not a surprise, in view of the discussion in Section~\ref{sub:pra} regarding the feasible region of the OBS problem. Indeed, the runtime of Algorithm~\ref{alg:oneshotrefinement} does not depend on the network size per-se, but rather on the the number of spanning trees of the reduced graph $G_\calP$ corresponding to the optimal partition $\calP$ identified by each of the three methods. This makes the runtime of the one-shot algorithm rather unpredictable, discouraging its usage in real time.

% \subsubsection{Results for recursive algorithm and comparison with the one-shot algorithms}

Let us now focus on the performance of the recursive algorithm, i.e.~Algorithm~\ref{alg:recursiverefinement}. In Table~\ref{tab:recursive_results} below, we report the results for the same test networks considered in Table~\ref{tab:one-shot_results} s well as a few more networks of larger size. Indeed, the running time of the recursive algorithm depends solely on the number of spanning trees that needs to be considered in the OBS problem. By design, for the recursive algorithm this number is in most cases very small even for large networks, as we can deduce from the second last column of Table~\ref{tab:recursive_results}. Indeed for the recursive algorithm the number of considered spanning trees is equal to the number of cross-edges of the selected bipartition, which is in turn equal to one plus the number of lines switched off.

For each test network, we run the recursive algorithm with $i_\mathrm{max}=3$, reporting the runtime of each of these three iterations. This choice for $i_\mathrm{max}$ allows us to make a fair comparison with the one-shot algorithm with a target of $b=4$ clusters, since we expect the same number of resulting bridge-blocks (modulo ``spontaneous'' splits in smaller bridge-blocks).

% We now focus on the implementation of the OBS problem~\eqref{eq:optswitch_basic}. %, whose feasible set are all the subsets of cross-edges $\calE \subset E_c(\calP)$ whose removal make the reduced graph $(G^\calE)_\calP$ a tree.
% As we remarked earlier, there is a one-to-one correspondence between feasible subsets $\calE$ of cross-edges and spanning trees of the reduced multi-graph $G_\calP$. We can solve the OBS exactly with brute-force for small partitions $\calP$ of $G$ (consisting of, say, less than $5$ clusters) by listing all possible spanning tree of $G_\calP$. \alec{this technical detailed should be moved later} We adopt this approach for three of the IEEE test networks considered in the previous subsection of very different sizes. 

% For each network we use the one-shot bridge-block decomposition refinement (as formulated in Algorithm~\ref{alg:oneshotrefinement}) for various target number of blocks $b=2,3,4$ and using both the two \alec{three?} clustering methods described in the previous subsection. For each of these scenarios we find the optimal set of switching actions $\calE^*$ and report the post-switching network congestion level $\gamma(\calE^*)$ and the average line congestion $\bar{\gamma}(\calE^*) = (|E\setminus\calE^*|)^{-1} \sum_{e \in E\setminus \calE^*} |f^{\calE^*_e}|/C_e$, which are to be compared with those of the original network, $\gamma(\emptyset)$ and $\bar{\gamma}(\emptyset)$ respectively.
% \begin{table}[!ht]
% \centering
% % \begin{tabular}{c|c|c|c|c|c}
% % Method & $b$ &  $Q$ & \# cross-edges removed & $\gamma(\calE^*)$ & $\bar{\gamma}(\calE^*)$\\ 
% % \hline \hline
% % Spectral & 2 & 0.466 & 2 & $=$ & 0.3795 \\
% % FastGreedy & 2 & 0.466 & 2 & $=$ & 0.3795\\
% % \hline
% % Spectral & 3 & 0.580 & 3 & $=$ & 0.3788\\
% % FastGreedy & 3 & 0.646 & 3 & $=$ & 0.3779\\
% % \hline
% % Spectral & 4 & 0.646 & 3 & $=$ & 0.3781 \\
% % FastGreedy & 4 & 0.691 & 4 & $=$ & 0.3765\\
% % \end{tabular}
% \begin{tabular}{c|c|c|p{1cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{2.5cm}}
% step &     runtime & max cong &  avg cong & \# cong lines & cross-edges & spanning trees & \# removed lines & fraction removed lines & largest bridge block size &                                        block sizes \\
% \hline \hline
% 0 &  0.0026 &        1 &  0.3712 &                2 &           0 &              0 &              0 &                    - &       0 &              [28] \\
% 1 &    0.1122 &        1 &  0.3884 &                1 &           3 &              3 &              2 &              0.0434 &      28 &  [10, 9, 5] \\
% 2 &   0.0902 &  1.11299 &  0.3937 &                4 &           2 &              2 &              1 &              0.0217 &      10 &  [9, 5, 4, 4] \\
% 3 &   0.0936 &  1.11299 &  0.4035 &                5 &           2 &              2 &              1 &              0.0217 &       9 &  [5, 4, 4, 3] \\
% \end{tabular}
% \caption{IEEE 39. Spectral $L_n$}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|p{1cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{2.5cm}}

% step &     runtime & max cong &  avg cong & \# cong lines & cross-edges & spanning trees & \# removed lines & fraction removed lines & largest bridge block size &                                        block sizes \\
% \hline \hline
% 0 &  0.0026 &        1 &  0.3712 &                2 &           0 &              0 &              0 &                    - &       0 &              [28] \\
% 1 &    0.1022 &        1 &  0.3884 &                1 &           3 &              3 &              2 &              0.0434 &      28 &  [10, 9, 5,] \\
% 2 &   0.0870 &  1.14307 &  0.4037 &                2 &           2 &              2 &              1 &              0.0217 &      10 &  [9, 5, 4, 4] \\
% 3 &    0.0954 &  1.14307 &  0.4116 &                2 &           2 &              2 &              1 &              0.0217 &       9 &  [5, 4, 4, 3] \\
% \end{tabular}
% \caption{IEEE 39. Spectral $B_n$}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|p{1cm}|p{1cm}|p{0.8cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{2.5cm}}
% step &     runtime & max cong &  avg cong & \# cong lines & cross-edges & spanning trees & \# removed lines & fraction removed lines & largest bridge block size &                                        block sizes \\
% \hline \hline
% 0 &  0.0030 &        1 &  0.3712 &                2 &           0 &              0 &              0 &                    - &       0 &              [28] \\
% 1 &    0.0953 &        1 &  0.3938 &                1 &           3 &              3 &              2 &              0.0434 &      28 &  [10, 9, 5] \\
% 2 &   0.0656 &        1 &  0.4058 &                1 &           2 &              2 &              1 &              0.0217 &      10 &  [9, 5, 4, 4] \\
% 3 &   0.0730 &        1 &  0.4152 &                1 &           2 &              2 &              1 &              0.0217 &       9 &  [5, 4, 4, 3] \\
% \end{tabular}
% \caption{IEEE 39. Fastgreedy}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ &  $Q$ & \# cross-edges removed & $\gamma(\calE^*) $ & $\bar{\gamma}(\calE^*)$\\ 
% \hline \hline
% Spectral & 2 & 0.475 & 7 & $=$ & 0.1179 \\
% FastGreedy & 2 & 0.471 & 10 & $=$ & 0.1158\\
% \hline 
% Spectral & 3 & 0.559 & 10 & $=$ & 0.1150\\
% FastGreedy & 3 & 0.623 & 13 & $=$  & 0.1153\\
% \hline 
% Spectral & 4 & 0.602 & 16 & $=$ & 0.1206 \\
% FastGreedy & 4 & 0.703 & 16 & $=$ & 0.1153 \\
% \end{tabular}
% \caption{IEEE 200. Original congestion: $\gamma(\emptyset) =0.7075$ and $\bar{\gamma}(\emptyset)=0.1167$}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method & $b$ &  $Q$ & \# cross-edges removed & $\gamma(\calE^*) $ & $\bar{\gamma}(\calE^*)$\\ 
% \hline \hline
% Spectral & 2 & 0.403 & 29 & 0.9929 & 0.1429\\
% FastGreedy & 2 & 0.462 & 83 & 1.2719 & 0.1471\\
% \hline
% \textbf{Spectral} & 3 & 0.620 & 50 & 0.9172 & 0.1429\\
% FastGreedy & 3 & 0.636 & 126 & 1.2719 & 0.1481 \\
% \hline
% Spectral & 4 & 0.657 & 67 & 0.9172 & 0.1431\\
% FastGreedy & 4 & 0.710 & 126 & 0.9812 & 0.1506\\
% \end{tabular}
% \caption{IEEE 2736sp. Original congestion: $\gamma(\emptyset) =0.9767$ and $\bar{\gamma}(\emptyset)=0.1423$}
% \end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{p{1.9cm}|p{3.2cm}|p{1.25cm}|p{2cm}|p{1.85cm}|p{1.8cm}|p{1.8cm}}
network & iteration &  runtime (sec) &  $\gamma(\calE^*)$ & \# congested lines & \# of lines switched off & $\%$ of lines switched off\\
\hline \hline
\multirow{5}{*}{case39\_epri} 
& initial configuration & - &  $\gamma(\emptyset) =1.000$ & 2 & - & -\\
\cline{2-7}
& 1 &   0.091 &                0.794 &                0 &              2 &                4.35 \\
& 2 &   0.069 &                0.833 &                0 &              1 &                2.17 \\
& 3 &  0.082 &                0.833 &                0 &              1 &                2.17 \\
\cline{2-7}
& final &  0.242 &  \textbf{0.833} & \textbf{0} & \textbf{4} & \textbf{8.70} \\
\hline
\hline
\multirow{4}{*}{case57\_ieee} 
& initial configuration & - &  $\gamma(\emptyset) =0.938$ & 0 & - & -\\ 
\cline{2-7}
& 1 &   0.371 &                1.038 &                2 &             10 &                     12.5 \\
& 2 &   0.142 &                1.038 &                2 &              3 &                     3.75 \\
& 3 &  0.085 &                 1.038 &                2 &              1 &                     1.25 \\
\cline{2-7}
& final &  0.598 &   \textbf{1.038} &  \textbf{2} & \textbf{14} & \textbf{17.5} \\
\hline
\hline
\multirow{4}{*}{case73\_ieee}
& initial configuration & - &  $\gamma(\emptyset) = 0.632$ & 0 & - & -\\
\cline{2-7}
& 1 &  0.076 &                0.778 &                0 &              1 &                 0.83 \\
& 2 &   0.099 &                0.772 &                0 &              2 &                  1.67 \\
& 3 &   0.156 &                0.694 &                0 &              4 &                  3.33 \\
\cline{2-7}
& final &  0.242 &   \textbf{0.694} & \textbf{7} & \textbf{6} &  \textbf{5.83} \\
\hline
\hline
\multirow{4}{*}{case118\_ieee} 
& initial configuration & - &  $\gamma(\emptyset) = 1.000$ & 2 & - & - \\
\cline{2-7}
& 1 &   0.278 &                1.011 &                2 &              5 &                  2.69 \\
& 2 &  0.168 &                1.045 &                2 &              4 &                  2.15 \\
& 3 &  0.135 &                1.045 &                2 &              3 &                   1.61 \\
\cline{2-7}
& final &  0.581 &  \textbf{1.045} & \textbf{2} &  \textbf{12} & \textbf{6.45} \\
\hline
\hline
\multirow{4}{*}{case179\_goc} 
& initial configuration & - &  $\gamma(\emptyset) =1.000$ & 4 & - & -\\
\cline{2-7}
& 1 &   0.148 &                1.382 &                5 &              3 &                  1.14 \\
& 2 &   0.154 &                1.382 &                5 &              2 &                 0.76 \\
& 3 &   0.251 &                1.382 &                5 &              6 &                  2.28 \\
\cline{2-7}
& final &  0.553 &  \textbf{1.382} & \textbf{5} & \textbf{11} & \textbf{4.18} \\
\hline
\hline
\multirow{4}{*}{case200\_activ} 
& initial configuration & - &  $\gamma(\emptyset) =0.708$ & 0 & - & -\\
\cline{2-7}
& 1 &   0.221 &                 0.591 &                0 &              5 &                  2.04 \\
& 2 &   0.281 &                 0.591 &                0 &              8 &                  3.26 \\
& 3 &   0.141 &                0.605 &                0 &              3 &                  1.22 \\
\cline{2-7}
& final &  0.643 &  \textbf{0.605} &  \textbf{0} & \textbf{16} & \textbf{6.52} \\
\hline
\hline
\multirow{4}{*}{case300\_ieee} 
& initial configuration & - &  $\gamma(\emptyset) =1.000$ & 11 & - & -\\
\cline{2-7}
& 1 &  0.509 &               1.161 &                5 &             12 &                  2.91 \\
& 2 &  0.223 &               1.161 &                5 &              3 &                 0.73 \\
& 3 &  0.386 &               1.197 &                7 &              8 &                  1.95\\
\cline{2-7}
& final & 1.118 &   \textbf{1.197} & \textbf{7} & \textbf{23} & \textbf{5.59} \\
\hline
\hline
\multirow{4}{*}{case1888\_rte} 
& initial configuration & - &  $\gamma(\emptyset) =1.000$ & 14 & - & -\\
\cline{2-7}
& 1 &     4.567 &              0.869 &                0 &             48 &                  1.89 \\
& 2 &    1.994 &               0.869 &                0 &              9 &                 0.36 \\
& 3 &    2.694 &               0.869 &                0 &             24 &                 0.95 \\
\cline{2-7}
& final &  9.225 &  \textbf{0.869} & \textbf{0} & \textbf{81} & \textbf{3.20} \\
\hline
\hline
\multirow{4}{*}{case2735\_sop} 
& initial configuration & - &  $\gamma(\emptyset) =1.000$ & 1 & - & -\\
\cline{2-7}
& 1 &   12.57 &              0.964 &                0 &            116 &                  3.54 \\
& 2 &   1.317 &              0.964 &                0 &             19 &                  0.58 \\
& 3 &   2.145 &              2.637 &               13 &             33 &                  1.00\\
\cline{2-7}
& final &  16.032 &  \textbf{2.637} & \textbf{13} & \textbf{168} & \textbf{5.12} \\
\hline
\hline
    \end{tabular}
    \caption{Results obtained by the recursive algorithm stopped after $3$ iterations using the FastGreedy method for the candidate bridge-blocks identification.}
    \label{tab:recursive_results}
\end{table}
\FloatBarrier

% Our numerical experiments illustrate that in all the considered IEEE test networks it is always possible to refine the bridge-block decomposition to have $b=2,3,4$ bridge-blocks without increasing the maximum congestion level and, in a few cases, the congestion can even be reduced.

% Looking in particular at the Polish network, the spectral clustering method seems more effective than the FastGreedy method in identifying partitions that, given as input to the OBS problem, yield a refined network with lower congestion level. This could be a consequence of the fact that the spectral clustering method seems to identify partition with fewer cross-edges, which in turn means that a smaller number of switching actions has to be taken.

% It is worth noticing that all these power networks have a lot of spare capacity, as it is evident from the histograms below \alec{add histograms} and the average congestion levels $\bar{\gamma}$ reported above. This fact corroborates the intuition that network operators may indeed have a lot of ``room'' to make operational decisions and, in particular, to temporarily switch off lines. The only exception in this regard is the Polish network, which at least in the 2003 summer peak scenario considered here, has a single transmission line with congestion $0.9767$ which severely limits the possible switching actions. In particular, the FastGreedy method does not yield any valid set of switching actions for $b=2$ and $b=3$, because even the best one result in a congestion larger than one on that line.

%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 0.00077 & 0.4483 & \{13,26\} & 3 \\
%\hline 
%NMod Spectral & 0.00088 & 0.4888 & \{19,20\} & 3 \\
%\hline 
%FastGreedy & 0.00104 & 0.4640 & \{14,25\} & 3 \\ 
%\end{tabular}
%\caption{IEEE 39 statistics for finding two communities}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 0.25928 & 0.6619 & \{6,7,12,14\} & 7 \\
%\hline 
%NMod Spectral & 0.26961 & 0.6766 & \{5,8,12,14\} & 6 \\
%\hline 
%FastGreedy & 0.00119 & 0.6903 & \{6,8,12,13\} & 7 \\
%\end{tabular}
%\caption{IEEE 39 statistics for finding $4$ communities recursive spectral vs fastgreedy}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 0.00475 & 0.2697 & \{10,108\} & 8 \\
%\hline 
%NMod Spectral &  0.00619 & 0.4498 & \{58,60\} & 12 \\
%\hline 
%FastGreedy & 0.00287 & 0.4783 & \{52,66\} & 14 \\
%
%\end{tabular}
%\caption{IEEE 118 statistics for finding two communities}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 1.39983 & 0.4505 & \{5,5,22,86\} & 29 \\
%\hline 
%NMod Spectral & 1.38727 & 0.6791 & \{24,29,29,36\} & 20 \\
%\hline 
%FastGreedy & 0.00251 & 0.7031 & \{15,29,37,37\} & 23 \\
%\end{tabular}
%\caption{IEEE 118 statistics for finding $4$ communities recursive spectral vs fastgreedy}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 0.02734 & 0.2875 & \{33,267\} & 23 \\
%\hline 
%NMod Spectral &  0.02948 & 0.4785 & \{82,218\} & 5 \\
%\hline 
%FastGreedy & 0.00650 & 0.4911 & \{107,193\} & 11 \\
%\end{tabular}
%\caption{IEEE 300 statistics for finding two communities}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 5.220 & 0.4619 & \{9,22,24,245\} & 43 \\
%\hline 
%NMod Spectral & 5.452 & 0.6866 & \{43,44,50,174\} & 14 \\
%\hline 
%FastGreedy & 0.007 & 0.7165 & \{36,71,76,117\} & 22 \\
%\end{tabular}
%\caption{IEEE 300 statistics for finding $4$ communities recursive spectral vs fastgreedy}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 4.6788 & 0.1961 & \{65,2671\} & 87 \\
%\hline 
%NMod Spectral &  4.7021 & 0.4449 & \{1167,1569\} & 38 \\
%\hline 
%FastGreedy & 0.2199 & 0.4614 & \{1267,1469\} & 101 \\
%\end{tabular}
%\caption{IEEE 2736wp statistics for finding two communities}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{c|c|c|c|c}
%Method & Time (sec) & $Q$ & Regions size & cross-edges \\ 
%\hline \hline
%Mod Spectral & 28.143 & 0.2231 & \{28,28,37,2643\} & 141 \\
%\hline
%NMod Spectral & 25.998 & 0.6862 & \{354,748,813,821\} & 121 \\
%\hline 
%FastGreedy & 0.20800 & 0.7063 & \{472,584,795,885\} & 180 \\
%\end{tabular}
%\caption{IEEE 2736wp statistics for finding $4$ communities recursive spectral vs fastgreedy}
%\end{table}

%\begin{table}[!ht]
%\centering
%\begin{tabular}{p{3cm}|c|p{2cm}|p{1.5cm}|c|p{1.5cm}|p{1.5cm}|p{1.5cm}}
%Method & \# bridges & Non-cong.-increasing bridges & Best bridge & Max cong. & Mean cong. & Bridge cong. & Bridge cong. increase\\ 
%\hline \hline
%Original & - & -& -& 0.75921 & 0.38262 & - \\
%\hline 
%After switching -- Spectral dir & 3& 2& (25,26) & 0.75921 & 0.39544 & 0.44147 & +78.5\%\\
%\hline 
%After switching -- FastGreedy dir & 3& 3& (3,18) & 0.75921 & 0.39608 & 0.03447& -26.4\%\\ 
%\hline 
%After switching -- Spectral rec & 3& 2& (25,26) & 0.75921 & 0.39544 & 0.44147 & +78.5\%\\
%\hline 
%After switching -- FastGreedy rec & 3& 3& (3,18) & 0.75921 & 0.39608 & 0.03447& -26.4\%\\ 
%\end{tabular}
%\caption{IEEE 39 congestion statistics after switching (2 communities)}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{p{3cm}|c|p{2cm}|p{1.5cm}|c|p{1.5cm}|p{1.5cm}|p{1.5cm}}
%Method & \# bridges & Non-cong.-increasing bridges & Best bridge & Max cong. & Mean cong. & Bridge cong. & Bridge cong. increase\\ 
%\hline \hline
%Original & - & -& -& 0.75921 & 0.38262 & - \\
%\hline 
%After switching -- NMod Spectral & 3& 2& (25,26) & 0.75921 & 0.39544 & 0.44147 & +78.5\%\\
%\hline 
%After switching -- FastGreedy & 3& 3& (3,18) & 0.75921 & 0.39608 & 0.03447& -26.4\%\\ 
%\end{tabular}
%\caption{IEEE 39 congestion statistics after switching (2 communities)}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{p{3cm}|c|p{2cm}|p{1.5cm}|c|p{1.5cm}|p{1.5cm}|p{1.5cm}}
%Method & \# bridges & Non-cong.-increasing bridges & Best bridge & Max cong. & Mean cong. & Bridge cong. & Bridge cong. increase\\ 
%\hline \hline
%Original & - & -& -& 0.707022 & 0.117357 & - \\
%\hline 
%After switching -- NMod Spectral & 9& 3 & (150,194) & 0.70702 & 0.12983& 0.00157 & -99.4\% \\
%\hline 
%After switching -- FastGreedy & 11& 11 & (22,158) & 0.70702 & 0.12305 & 0.01413 & -22.7\%\\
%\hline 
%After switching -- FastGreedy & 11& 11 & (45,187) & 0.70702 & 0.12170 & 0.05338 & -44.4\%\\
%\end{tabular}
%\caption{IEEE 200 congestion statistics after switching (2 communities)}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{p{3cm}|c|p{1.9cm}|p{1.5cm}|c|p{1.5cm}|p{1.5cm}|p{1.5cm}}
%Method & \# bridges & Best bridges & Max cong. & Mean cong. & Bridge cong. & Bridge cong. increase\\ 
%\hline \hline
%Original & - & -& 0.75921 & 0.38262 & - & -\\
%\hline 
%After switching -- Recursive NMod Spectral & 3&  (3,4), (17,27), (25,26) & 0.75921 & 0.40548 & (0.23925, 0.56320, 0.08182)& (+151.8\%, +1102.7\%, -2\%)\\
%\hline 
%After switching -- FastGreedy & 3& (3,4), (3,18), (16,21) & 0.75921 & 0.41299 & (0.03447, 0.19360, 0.06659) & (-52.4\%, -64.9\% -20.3\%)\\ 
%\end{tabular}
%\caption{IEEE 39 congestion statistics after switching (4 communities)}
%\end{table}
%
%\begin{table}[!ht]
%\centering
%\begin{tabular}{p{3cm}|c|p{1.9cm}|p{1.5cm}|c|p{1.5cm}|p{1.5cm}|p{1.5cm}}
%Method & \# bridges & Best bridges & Max cong. & Mean cong. & Bridge cong. & Bridge cong. increase\\ 
%\hline \hline
%Original & - & -& 0.70702 & 0.11736 & - & -\\
%\hline 
%After switching -- Recursive NMod Spectral & 3&  (194,150), (102,45), (159,39) & 0.70702 & 0.13294 & (0.00270, 0.03166, 0.00257)& (-99.0\%, -27.9\%, -93.5\%)\\
%\hline 
%After switching -- FastGreedy & 3 & (45,187), (95,58), (128,33) & 0.70702 & 0.14239 & (0.07527, 0.44213, 0.0183) & (-21.6\%, +8776\%, -84.5\%)\\
%\hline 
%After switching -- FastGreedy & 3 & (81,178), (14,149), (128,133) & 0.70702 & 0.12373 & (0.07426, 0.44823, 0.13699) & (-20.5\%, +137.3\%, +16.4\%)\\ 
%\end{tabular}
%\caption{IEEE 200 congestion statistics after switching (4 communities) - 23/45 non-congestion increasing possible bridge combinations for NMod, 176/176 non-congestion increasing possible bridge combination for FG}
%\end{table}

By comparing Tables~\ref{tab:one-shot_results} and~\ref{tab:recursive_results} it is clear that among the two algorithms, the one-shot algorithm is the one with slightly better performance, as it yields lower network congestion level for almost all the test networks considered. %\lguo{If we only compare Table 7 and the one-shot algorithm with FastGreedy, looks like recursive is actually either very close or much better (in 118 case)?}. 
On the other hand, the recursive algorithm still yields good results (even when using only the FastGreedy method for the first subproblem), but it is orders of magnitude faster.

% \alec{How to better quantify the computational costs and thus the tradeoff? Currently #scenarios = #spanning tree of the multigraph $G_\calP$ to be considered}
% \alec{Both for Tables 6 and 7 we need to quantify the benefits in terms of bridge-block refinement. How to do this?} \adam{I'm not sure adding anything is needed...maybe just a sentence or two reminding of the benefits?}

% \alec{Comparison of ONE SHOT vs. RECURSIVE Add explanation for the next three tables to compare $b=4$ done with brute force (all possible spanning trees of the reduced graph) vs.~$b=4$ done with recursive partitions. The last column report how many scenarios (=spanning trees) are checked in each of the two cases to show the huge speed-up obtained by using the recursive method.}
% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method &  $Q$ & cross-edges & $\gamma(\calE^*) $ & $\bar{\gamma}(\calE^*)$ & \# scenarios\\ 
% \hline \hline
% Spectral $b=4$ 			& 0.646 & 6 	& 0.7667 	 	& 0.3781 &\\
% FastGreedy $b=4$ 		& 0.691 & 7		& 0.7667 		& 0.3765 &\\
% \hline 	
% Spectral recursive 		& 0.713 & 7 	& 0.75 			& 0.3827 &\\
% FastGreedy recursive	& 0.697 & 7 	& 0.7667 		& 0.3760 &\\
% \end{tabular}
% \caption{IEEE 39 with $b=4$ target clusters. Original congestion: $\gamma(\emptyset) =0.7667$ and $\bar{\gamma}(\emptyset)=0.3834$}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method &  $Q$ & cross-edges & $\gamma(\calE^*) $ & $\bar{\gamma}(\calE^*)$ & \# scenarios\\ 
% \hline \hline
% Spectral $b=4$ 			& 0.602 & 19	&	 0.7075    & 0.1171 &\\
% FastGreedy $b=4$ 		& 0.703 & 19 &  0.7075		& 0.1164 &\\
% \hline
% Spectral recursive		& 0.600 & 16 & 0.7074 &	0.1228 &\\
% FastGreedy recursive 	& 0.721 & 19 & 0.7075 & 0.1170 &\\
% \end{tabular}
% \caption{IEEE 200 with $b=4$ target clusters. Original congestion: $\gamma(\emptyset) =0.7075$ and $\bar{\gamma}(\emptyset)=0.1167$}
% \end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c}
% Method &  $Q$ & cross-edges & $\gamma(\calE^*) $ & $\bar{\gamma}(\calE^*)$ & \# scenarios\\ 
% \hline \hline
% Spectral $b=4$ 			& 0.657 & 70 	&  	0.9172 & 0.1431 &\\
% FastGreedy $b=4$ 		& 0.710 & 129	&  	0.9812 & 0.1506 &\\
% \hline
% Spectral recursive 		& 0.653 & 70 	&  0.9508 &	0.1465 &\\
% FastGreedy recursive	& 0.710 & 140 	&  0.9967 &	0.1554 &\\
% \end{tabular}
% \caption{IEEE 2736sp with $b=4$ target clusters. Original congestion: $\gamma(\emptyset) =0.9767$ and $\bar{\gamma}(\emptyset)=0.1423$}
% \end{table}

% \begin{figure}
% \includegraphics[scale=0.45]{case2736sp_nice_pruned.png}
% \caption{The 2736sp network after the optimal switching actions}
% \end{figure}

% \begin{figure}
% \includegraphics[scale=0.45]{case2736sp_nice_tree.png}
% \caption{The 2736sp network after the optimal switching actions and with the nodes rearranged to highlight the bridge-block decomposition}
% \end{figure}
% \FloatBarrier

% \subsection{Counterexample loop flows \& monotonicity \& increased modularity}
% \label{subcounterexample}
% One may expect that the network congestion level is monotone increasing along the bridge-block decomposition refinement process, namely $\gamma^*_{n+1} \geq \gamma^*_{n}$. The following 4-node power network is a counterexample that proves that this is not necessarily the case and that is instrumental to illustrate some further counter-intuitive properties of the network congestion level.

% \alec{Is this counterexample still relevant? We have examples of network congestion level decreasing after switching actions for IEEE networks, which are probably more convincing?}

% \ale{Put 4-node network here\\

% 4-node network example $p=(-0.1, 1, -0.5, -0.4)$, unit capacities, unit susceptances, before $f=(0.4,-0.6,-0.1,0.3)$ after $f=(0.5,-0.5, \times ,0.4)$\\

% 4-node network example $p=(-0.4, 1, -0.5, -0.1)$, unit capacities, susceptances $\beta=(1, 0.5, 1, 0.5)$, before $f=(0.55, -0.45, 0.05, 0.15)$, cross-edges flows $(0.05, 0.15)$ (LOOP!), after $f=(0.5,-0.5,0.1)$\\

% Further comments to make: (1) $\gamma^*$ is monotone increasing if and only if the partition is the optimal one and (2) The network modularity maximization problem always yields an optimal partition $\calP^*$ for which there are no loop flows across different clusters.
% }


==> arxiv submission/optimization.tex <==
\section{Improving network reliability by bridge-block decomposition refinement}
\label{sec:optimization}
In this section we outline a new method to refine the bridge-block decomposition of a given power network by means of \textit{line switching actions}. 
Even though we usually think of transmission lines as static assets, network operators have the ability to remotely control circuit breakers that open and close them, effectively removing them from service and thus modifying the network topology. This procedure, that goes under the name of \textit{transmission line switching}, is a mature power system technology that is already commonly used by network operators. 
A large body of literature has been devoted to the optimization problems that stem from this network flexibility, see our discussion about Optimal Transmission Switching (OTS) in Section~\ref{sub:literature}.
% Optimal Transmission Switching (OTS) has been studied either (i) as a corrective mechanism in case of voltage violations and line overloads~\cite{khanabadi2012optimal,korad2013robust,li2016real,li2019enhanced} or (ii) as a way to further decrease energy dispatching costs and/or reduce line losses while maintaining reliability standards~\cite{fisher2008optimal,hedman2008optimal,hedman2009optimal,ruiz2012tractable,soroush2013accuracies,kocuk2017new}. \alec{Can this be removed in view of the related literature subsection?} \adam{yes} 
% Furthermore, several automated protection schemes (put in place as set of prescribed rules by network operators) often prescribe disconnecting/reconnecting lines, but these schemes are activated under specific contingencies rather than in normal conditions and do not involve any optimization.

In this paper we want to propose a new way to improve the network reliability leveraging the flexibility offered by these transmission line switches. Our strategy is inspired by Lemma~\ref{lem:finer}, which suggests that switching off a subset of the currently active lines is a way to refine the bridge-block decomposition of a network. In Figs.~\ref{fig:influencegraph_pre} and~\ref{fig:influencegraph_post} we briefly illustrated how a significant bridge-block decomposition refinement is possible for the IEEE 118-bus network by switching off only three lines.
Such switching actions can be taken both proactively, as semi-permanent network design decision, but also as temporary response to a contingency or an unusual load/generation profile. As summarized by our results in Section~\ref{sec:localization}, a finer bridge-block decomposition greatly improves the network robustness against failure propagation, since it automatically avoids long-distance propagation of line failures. More specifically, an immediate consequence of Proposition~\ref{prop:glodf_non_cut} is that any non-cut set line outage does not propagate outside the bridge-bridge block(s) to which the disconnected lines belong. 

Our approach is particularly promising in view of the fact that most power grids have a trivial bridge-block decomposition, making a global propagation of line failures very likely in these networks. Indeed, all the considered IEEE test networks have a single massive bridge-block and possibly a few additional blocks consisting of a single vertex, see Fig.~\ref{fig:influencegraph_pre}, Table~\ref{tab:networkstatistics} in Section~\ref{sec:numerics}, and Fig.~\ref{fig:oneshotalgorithm}(a). 

The crucial step is thus, given a power network $G$, identifying a subset of lines $\calE \subset E$ to be temporarily removed from service by means of switching actions, so that the newly obtained network $G^\calE$ has a ``good'' bridge-block decomposition $\calBB(G^\calE)$ while still remaining connected. In this section, we formulate an optimization problem to find the best subset of lines to switch off that would guarantee a desired network bridge-block decomposition without creating congestion in the remaining lines.
However, any line switching action causes a power flow redistribution on the remaining lines (exactly like line outages do) and may cause overloads. It is then crucial to carefully assess the impact of each set of switching actions on the network flows and avoid creating any congested line. A brute-force search to find such best switching actions and recalculate the line flows for each instance is infeasible, since there are exponentially many such subsets of lines $\calE \subset E$ to consider.
%Optimal transmission switching for economic benefit in a market context was investigated by O'Neill et al. [14]. Fisher et al. [15] and Hedman et al. [16] present and analyze the optimal transmission switching problem on the IEEE 118-bus test case and showed that co-optimizing the generation and the network topology can result in substantial savings. Transmission switching is not by definition incompatible with reliable network operations. Hedman et al. [17] demonstrated that transmission switching can be beneficial even while ensuring an N-1 reliable network.

% The switching actions we are interested in are only those that take lines temporarily offline, as only these make the network block partition finer. Switching off lines, however, induces a power flow redistribution on the remaining lines and may cause overloads. We thus formulate an optimization problem to find the best subset of lines to switch off that would guarantee a desired network block decomposition without creating congestion in the remaining lines.

Aiming to reduce the number of possible subsets of lines to consider, our method takes a different approach and ``works backwards''. Indeed, we first identify a ``good'' network partition $\calP$ whose clusters we want to become its bridge-blocks and then, using these clusters, we choose which of the cross-edges between them to remove so that $\calP$ actually becomes the network bridge-block decomposition. We thus propose an algorithm that consists of two steps, each one tackling one of these two sub-problems. 
%\adam{weak statement, need to say why it is computationally hard (e.g.~number of constraints) and why it becomes easier by breaking it into subproblems)}
This section is structured as follows:
\begin{itemize}
    \item In Subsection~\ref{sub:mod} we introduce the \textit{Optimal Bridge-Block Identification} (OBI) problem, which aims at identifying a good network partition based on the current network flow configuration, 
    \item In Subsection~\ref{sub:obs} we tackle the second sub-problem by formulating the \textit{Optimal Bridge Selection} (OBS) problem, which identifies the best subset of lines to be switched off that refines the network bridge-block decomposition and simultaneously minimizes the network congestion level, 
    \item In Subsection~\ref{sub:pra} we discuss some practical considerations regarding the algorithm implementation and present a faster recursive variant.
\end{itemize}

%In this section we introduce graph structures based on the spectral views introduced in the previous section that are instrumental to formalizing the impact of the network topology and balancing scheme on power flow redistribution. More precisely, we introduce the notion of the \textit{network tree partition}, which leverages cut edges, and the \textit{block decomposition}, an even finer graph partition obtained using cut vertices. Furthermore, we show how these network substructures are pivotal to understand how failure propagates in power networks. As a consequence, the concept of tree partition is at the core of the network reliability optimization procedure that we present later in Section~\ref{sec:optimization}. We illustrate the power of the tools introduced in this section through applications to \ale{XXX} which are described in more detail in Section~\ref{sec:applications}.

%, as summarized in Algorithm \ref{alg:tree_partition}:
%\begin{algorithm}[!h]
%\SetAlgoLined
%\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%\Input{ The graph $G=(V,E)$}
%\BlankLine
%\DontPrintSemicolon
%Compute the set of cut edges $\calE_b$ of $G=(V,E)$ using Tarjan's algorithm~(see~\cite{tarjan1974note});\\
%Remove edges in $\calE_b$ from $E$ and obtain a new graph $G'=(V, E \bs\calE_b)$;\\
%Breadth-first search on $G'$ to compute its connected components $\calP:=\set{\calV_1, \calV_2, \ldots, \calV_k}$;\\
%\KwRet{$\calP$}.
%\caption{Irreducible Tree Partition Finding Algorithm}\label{alg:tree_partition}
%\end{algorithm}
%\FloatBarrier

%To summarize, we have shown that each graph $\calG$ has a unique irreducible tree partition, which can be computed in linear time. Thus, to simplify the terminology, whenever we say the tree partition of $\calG$ in the sequel, we always refer to its irreducible partition.

%\subsubsection{Cells: Minimal Boundaries of Failure Propagation}
%Before stating our technical results, we first need to introduce the concept of \emph{cells}. 

%A vertex $v \in V$ is a \textit{cut vertex} if removing it (and edges through it) disconnects the graph. A \textit{block} of a graph is a maximal connected subgraph with no cut vertex or, equivalently, a maximal biconnected component. The blocks of a graph $G$ are attached to each other at shared vertices, which are precisely the cut vertices of $G$. The edge set $E$ of any connected graph decomposes into a tree of blocks called the \textit{block-cut tree} or \textit{block decomposition} of the graph. Given the tree partition of a graph, both the endpoints of every bridge are cut vertices, which readily implies that the block decomposition is finer than the tree partition (more specifically, the partition of the edge set $E$ induced by it). The block decomposition of a graph always exists and can be found in linear time as proved by~\cite{tarjan1985efficient}.


\subsection{Identifying candidate bridge-blocks using network modularity}
\label{sub:mod}
The bridge-block decomposition refinement should ideally require a minimum number of line switching actions. For this reason, it is thus crucial to leverage the structure of the existing network as much as possible when identifying the candidate bridge-blocks. In this subsection we describe in detail how we tackle this first sub-problem using the notion of network modularity.

Consider a power network $G=(V,E,\bm{b})$ with a fixed power injection configuration $\pp$. Aiming to find a network partition $\calP = \{\calV_1,\dots,\calV_{|\calP|}\}$ into clusters with the most suitable properties to become bridge-blocks via line switching, we introduce the following \textit{Optimal Bridge-Blocks Identification (OBI)} problem:
\begin{equation}
\label{eq:maxmodprob}
\max_{\calP \in \Pi(G)} \frac {1}{2 M} \sum_{r=1}^{|\calP|} \sum \limits _{i,j \in \calV_r} \left ( |f_{ij}|-\frac {F_{i} F_{j}}{2 M} \right ),  \qquad \textrm{(OBI)}
\end{equation}
where $\ff=(f_{ij})_{(i,j)\in E}$ is the current power flow pattern determined by the injections $\pp$ as prescribed by~\eqref{eq:flowsdc_model}, $F_{i} :=\sum_{j \in V} |f_{ij}|$ is the sum of absolute line flow incident to vertex $i$ and $M := \frac{1}{2} \sum_{i \in V} F_i = \frac{1}{2} \sum_{i,j \in V} |f_{ij}|$ is the total absolute line flows over the network.
When we restrict the subset of feasible partitions to $\Pi_{k}(G)$, we refer to problem~\eqref{eq:maxmodprob} as the OBI-$k$ problem. 

Having in mind the optimal line switching that we intend to perform in the second step of our algorithm, it is important to remember that each line that we decide to switch off will cause a power flow redistribution on the remaining lines. Aiming to prevent any of these lines to become congested, it is thus crucial to identify in this first step a ``good'' partition into clusters such that (i) a smaller number of switching actions to create the desired bridge-block decomposition and that (ii) the power flow redistribution ensuing the switching actions has a minimal impact on the rest of the network and does not create congestion.

The OBI problem~\eqref{eq:maxmodprob} is formulated precisely to find a partition with these features. Indeed, its objective function indirectly favors partitions that have:
\begin{itemize}
    \item[(F1)] very few (and/or low-weight) cross-edges between clusters;
    %they have very few cross-edges between them;
    \item[(F2)] clusters are balanced in terms of total net power and with very modest power flows from/towards the neighboring clusters.
    %they are balanced in terms of total net power and with very modest power flows from/towards the neighboring clusters.
\end{itemize}
These features follows from the fact that the objective function of~\eqref{eq:maxmodprob} is a power-flow-weighted version of the \textit{network modularity} introduced by~\cite{Newman2004b,Newman2004}. Network modularity is a key notion that has been introduced to tackle a classical problem in complex networks theory, namely unveiling the underlying community structure in a given network. Informally, the proposed optimal block identification problem is a community detection problem on a transmission network topology while using in a crucial way its electrical properties. The network modularity $Q(\calP)$ associated with a partition $\calP$ is a scalar between $-1/2$ and $1$~\cite{Brandes2008} that quantifies the quality of such a partition: a large value indicates a stronger ``community structure'', in the sense that there are more (and in the weighted case high-weight) edges within each cluster in $\calP$ than across them.

% \begin{equation}
% \label{eq:powerweights}
% 	w_{ij}=\begin{cases}
% 	|f_{ij}| & \text{ if } (i,j) \in E,\\
% 	0 & \text{ otherwise.}
% 	\end{cases}
% \end{equation}
%In the next subsections we explain in detail the idea behind this optimization problems and how it relates to the network modularity literature, as well as discuss its implementation.
%\subsubsection{Network modularity}
%Let $G=(V,E,w)$ be an undirected simple graph with $n=|V|$ nodes, $m=|E|$ edges and non-negative edge weights $\{w_{ij}\}_{i,j \in V}$, with the convention that absent edges have weight equal to zero. 
%As remarked earlier, here $G$ denotes a general graph with arbitrary edge weights and not necessarily a power network, which is a directed graph with the line susceptances as the edge weights.
%For $k\in \{1,\dots,n\}$, let $\mathcal{V} = \{V_1,\dots,V_k\}$ be a $k$-partition of the vertex set, i.e., a collection of nonempty subsets $V_i \subseteq V$ to which we will refer as \textit{regions} such that $V_i \cap V_j = \emptyset$ for $i\neq j$ and $\bigcup_{i=1}^k V_i = V$. Given a partition, we refer to an edge as a \textit{cross-edge} if its two endpoints belong to different regions and \textit{internal edge} otherwise. A partition $\mathcal{V}$ of the vertex set $V$ automatically induces a partition of the edge set $E$ into cross-edges and internal edges, whose collections will be denoted as $E_c(\mathcal{V})$ and $E_i(\mathcal{V})$, respectively.
%\begin{equation}
%\label{eq:defmod}
%	Q(\calP) :={\frac {1}{2 M}} \sum_{r=1}^{|\calP|} \sum \limits _{i,j \in \calV_r} \left ( w_{ij}-\frac {w_{i}w_{j}}{2 M} \right ),
%\end{equation}
%where $w_{i}=\sum_{j \in V} w_{ij}$ is the sum of the weights of the edges attached to node $i$ (sometimes referred to as the \textit{strength of node} $i$) and $M = \frac{1}{2} \sum_{i \in V} w_i = \frac{1}{2} \sum_{i,j \in V} w_{ij}$ is the sum of all edge weights.
%\begin{itemize}
%	\item $w_{ij}$ is the weight of edge $(i,j) \in E$;
%	\item $w_{i}=\sum_{j \in V} w_{ij}$ is the sum of the weights of the edges attached to node $i$;
%	\item $M = \frac{1}{2} \sum_{i \in V} w_i = \frac{1}{2} \sum_{i,j \in V} w_{ij}$ is the sum of all of the edge weights in the graph.
%\end{itemize}
%The network modularity takes value between \alec{...} and is a common way to define the quality of a partition $\calP$, namely a large value indicates a stronger ``community structure'', in the sense that there are more and/or stronger links within each cluster in $\calP$ than across them.
%
%Let us understand better the notion of network modularity by considering the simplest choice of weights, that is the case of a unweighted network $G=(V,E)$, where $w_{i,j}=\mathds{1}_{\{(i,j)\in E\}} \in \{0,1\}$. Consequently, the strength of node $i$ is equal to its degree, namely $w_i=d_i$, and $2M=2 |E|$ is equal to the total node degree sum. The modularity of a partition $\{\calV_1,\dots,\calV_k\}$ of such a graph measures the fraction of total internal edges within each cluster against the same quantity in a network with the same number $n$ of nodes and the same node degrees, but where the edges are placed randomly. Indeed, the term $\frac {d_i d_j}{2 M}$ should be interpreted as the likelihood of finding edge $(i,j)$ in a random graph conditioned on having the node degree sequence $d_1,\dots, d_n$. In other words, a graph with a high network modularity is a graph where the connectivity within each cluster is larger than the one expected in a random network with the same node properties. 
%
%The modularity of a partition $\{\calV_1,\dots,\calV_k\}$ of such a graph measures the fraction of total internal edges within each cluster against the same quantity in a network with the same number $n$ of nodes and the same node degrees, but where the edges are placed randomly. Indeed, the term $\frac {d_i d_j}{2 M}$ should be interpreted as the likelihood of finding edge $(i,j)$ in a random graph conditioned on having the node degree sequence $d_1,\dots, d_n$. In other words, a graph with a high network modularity is a graph where the connectivity within each cluster is larger than the one expected in a random network with the same node properties. 
%
% More specifically, the network modularity of a partition $\{\calV_1,\dots,\calV_k\}$ measures the weight of each internal edge $w_{ij}$ within each cluster against the expected weight $\frac {w_{i}w_{j}}{2 M}$ for that edge in a complete graph whose random edge weights are sampled proportionally to the node weights $w_1, \dots, w_n$ of their endpoints. A graph with a high network modularity is a graph where the (weighted) connectivity within each cluster is larger than the one expected in a random network with the same node properties. 

%We formulated the optimization problem~\eqref{eq:maxmodprob} taking as the objective function the network modularity~\eqref{eq:defmod} with weights equal to absolute power flows, namely 
%\begin{equation}
%\label{eq:powerweights}
%	w_{ij}=\begin{cases}
%	|f_{ij}| & \text{ if } (i,j) \in E,\\
%	0 & \text{ otherwise.}
%	\end{cases}
%\end{equation}
%and the strength of node $i$ is correspondingly equal to $F_{i}=\sum_{j \in V} |f_{ij}|$, that is the sum of the absolute value of the line flows arriving or leaving from node $i$.
% \adam{Can we make the rest of this subsection more structured? First explain the approach, then why, do not mix the two.}\\
Broadly speaking, a partition that yields a high network modularity is one where the connectivity within each cluster is larger than the one expected in a random network with the same nodal properties. More specifically, the modularity of a network partition measures the total weight of the internal edges within each cluster against the same quantity in a network with the same number of nodes and nodal properties, but in which the edges are placed randomly. Indeed, the term $\frac {F_i F_j}{2 M}$ should be interpreted as the likelihood of finding edge $(i,j)$ in a random graph conditioned on having the node generalized degree sequence $F_1,\dots, F_n$.

For the OBI problem we take as the objective function the network modularity where each edge weight is equal to absolute power flow on the corresponding line. In view of the definition of network modularity, the optimal partitions for the OBI problem are those with few lines between clusters and modest power flowing on them. We also remark that using the absolute power flows as weights in the OBI problem implicitly makes the resulting bridge-block decomposition adaptive to the possibly changing power injection and flow patterns. Such a feature would not be present if we used an unweighted network modularity as objective function or if we used other static network quantities, e.g. the line susceptances $\{\b_\ell\}_{\ell \in E}$, as weights. 

The notion of network modularity has been extended to deal with negative edge weights in~\cite{Gomez2009}: in this extension the high-modularity partitions tend to assign the two nodes at the endpoints of an edge with a negative weight to different clusters. In power networks, however, the flow signs are just an artifact of the (arbitrary) directions chosen for the network edges -- in fact, one could always choose edge directions so that all the flows are positive. Our goal to identify the network partitions with modest flows across different clusters \textit{regardless of their directions} makes the \textit{absolute values} of the flows the sensible choice for the edge weights.

% With this choice of edge weights, a high modularity partition of the network will have very few lines with modest flows connecting different clusters. As mentioned earlier, this is highly desirable, since fewer switching actions will be necessary to create a block decomposition and the impact on the remaining lines after the power flow redistribution will be minor, lowering the chance of congestion.

%This means that (i) it is unlikely to yield clusters that are trivial (consisting of only a few nodes) or very heterogeneous (with very uneven sizes) and that (ii)

%\subsubsection{Practical considerations: approximating optimal modularity}
%\adam{This subsection seems more like a remark currently, unless there is more to say}
\subsubsection{Related classical clustering problems}
One might argue that a simpler approach for bridge-block identification could have been solving a weighted \textit{minimum $k$-cut problem}
\begin{equation}
\label{eq:mincut}
	\arg\min_{\calP \in \Pi(G)} \sum_{r=1}^{|\calP|} \mathrm{Cut}(\calV_r),
\end{equation}
where $\mathrm{Cut}(\calV_r) := \sum_{i \in \calV_r, \, j \in \calV_r^c} |f_{ij}|$. This combinatorial optimization problem can be solved efficiently, especially in the case $k=2$, as illustrated in~\cite{StoerWagner1997}. However, such a min-cut solution would often not be a satisfactory partition for the power systems application at hand. Indeed, in many instances the min-cut solution separates one or very few vertices from the rest of the network and such trivial partitions will yield a rather unbalanced bridge-block decomposition with limited failure localization potential. On the contrary, it is very unlikely that the OBI problem yields trivial partitions. Indeed, using the weighted network modularity~\eqref{eq:maxmodprob} as objective function favors partitions with ``balanced clusters'', which in our setting means with small total net power $\sum_{i \in \calV_r} p_i$, $r=1,\dots,|\calP|$. This feature of high modularity partition has been proved rigorously: as shown by~\cite{Reichardt2006} and~\cite{Bertozzi2018}, for a fixed number $k$ of clusters the OBI problem~\eqref{eq:maxmodprob}
%\[
%	\arg\max_{\calV \in \Pi_k(G)} \frac {1}{2 M} \sum_{r=1}^{k} \sum \limits _{i,j \in \calV_r} \left ( w_{ij}-\frac {w_{i} w_{j}}{2 M} \right )
%\]
has the same solution of the following \textit{balanced-cut problem}
\begin{equation}
\label{eq:balancedcut}
	\arg\min_{\calP \in \Pi_k(G)} \sum_{r=1}^k \left ( \mathrm{Cut}(\calV_r) + \frac {\mathrm{Vol}(\calV_r)^2}{2 M} \right ),
\end{equation}
where we used the classical notion of \textit{volume} of a cluster, which in our context is equal to $\mathrm{Vol}(\calV_r)= \sum_{i \in \calV_r} F_i$. This equivalence suggests that an optimal partition that maximizes modularity favors sparsely interconnected clusters with balanced volumes. This is particularly evident in the case of $k=2$ target clusters, in which~\eqref{eq:balancedcut} is equivalent to
\begin{equation}
\label{eq:modvol}
	\arg\min_{\calV \subset V} \left ( \mathrm{Cut}(\calV) + \frac {\mathrm{Vol}(\calV) \mathrm{Vol}(\calV^c)}{2 M} \right ).
\end{equation}
The second term $\mathrm{Vol}(\calV) \mathrm{Vol}(\calV^c)$ is maximal when $\mathrm{Vol}(\calV)= \mathrm{Vol}(\calV^c)=M$ and thus favors network partition with two clusters of roughly equal volume. In contrast, the first term favors a partition of the graph in which few edges with small weights are removed. This is reminiscent of the NCut problem introduced in~\cite{ShiMalik2000}, in which the objective is to minimize the ratio
\begin{equation}
\label{eq:ncut}
	\textrm{NCut}(\calP)= \frac{\mathrm{Cut}(\calV,\calV^c)}{\mathrm{Vol}(\calV)} +  \frac{\mathrm{Cut}(\calV,\calV^c)}{\mathrm{Vol}(\calV^c)} %\frac{\mathrm{Cut}(\calV,\calV^c)(\mathrm{Vol}(\calV) + \mathrm{Vol}(\calV^c))}{\mathrm{Vol}(\calV) \mathrm{Vol}(\calV^c)}
	\propto \frac{\mathrm{Cut}(\calV,\calV^c)}{\mathrm{Vol}(\calV) \mathrm{Vol}(\calV^c)}
\end{equation}
over all possible bipartitions $\calP=\{\calV,\calV^c\}$.
%The larger $\gamma$, the more the incentive to smaller communities.
%Furthermore, our method can be applied directly to any power system topology without the need of any pre-processing, as often done in the literature (for instance by removing leaf nodes). 
Whenever a cluster-balancing condition is introduced in the objective function either in the form of~\eqref{eq:balancedcut}, \eqref{eq:modvol} or~\eqref{eq:ncut} the min-cut problem become NP-hard, see~\cite{WagnerWagner1993} for details on NCut and~\cite{Brandes2006} for details on network modularity. Efficient algorithms are thus necessary to find good locally optimal network partitions with reasonable computational costs. Numerous methods have been proposed in the literature, for a review see~\cite{Fortunato2010,Fortunato2016,Porter2009,Chen2014}. These include greedy algorithms~\cite{Blondel2008,Clauset2004,Newman2004a,Wakita2007}, extrenal optimization~\cite{Boettcher2002,Duch2005}, simulated annealing~\cite{Guimera2005,Massen2005,Medus2005}, spectral methods %(which use eigenvectors of a modularity matrix)
~\cite{White2005,Newman2006a,Richardson2009}, sampling techniques~\cite{Sales-Pardo2007} and mathematical programming~\cite{Agarwal2008}.
%\zok{The locally greedy algorithm named ``Louvain Method'' introduced by~\cite{Blondel2008} is arguably the most popular computational heuristic; it is a very fast algorithm, and it also yields high modularity value~\cite{Lancichinetti2009}. Finally, it provides a hierarchy, induced by the successive aggregation steps
%of the algorithm, but this is not a full hierarchy, however, as there are typically a few aggregation steps. 
%This is a bottom-up algorithm: initially every vertex belongs to a separate community, and vertices are moved between communities iteratively in a way that maximizes the vertices' local contribution to the overall modularity score. When a consensus is reached (i.e. no single move would increase the modularity score), every community in the original graph is shrank to a single vertex (while keeping the total weight of the adjacent edges) and the process continues on the next level. The algorithm stops when it is not possible to increase the modularity any more after shrinking the communities to vertices. This algorithm is said to run almost in linear time on sparse graphs.}
%\alec{\cite{ShiMalik2000,Weiss1999,Ruan2008,Ruan2007,White2005} spectral methods but not for modularity?}
%\alec{The KCUT algorithm~\cite{Ruan2007} is intermediate between a recursive spectral bipartitioning algorithm~\cite{ShiMalik2000} that recursively divides each subnetwork into two and a $K$-way partitioning algorithm that directly divides a network into $K$ subnetworks~\cite{White2005}. The KCUT algorithm is recursive in essence. However, instead of searching for the best bipartitioning at each step, the algorithm attempts to divide a subnetwork into $2,3,\dots,l$ subnetworks using a $K$-way spectral graph partitioning algorithm, where $l$ is a small integer. These partitions are compared, and the one with the highest $Q$ is selected. The algorithm is then applied recursively to each subnetwork, until the $Q$ value of the network cannot be improved.}
In the present work we focus on two of these state-of-the-art algorithms, namely the ``fastgreedy'' method of~\cite{Clauset2004} and the spectral clustering method~\cite{Newman2006a,Newman2006b}, which we briefly review later in Section~\ref{sec:numerics}. These two methods are particularly suitable for our purposes because they allow for recursive partitioning. In the next section we use this feature in a crucial way, by devising an algorithmic procedure that progressively refines the block decomposition by splitting existing blocks in smaller ones, thus allowing to take switching actions in a sequential fashion.

\subsubsection{Intentional controlled islanding}

In this subsection, we briefly give an overview of another failure mitigation strategy that has some similarities with the candidate bridge-blocks identification described earlier in this section.
%\alec{High-level idea: there exists similar approaches for optimal islanding, our method can be used to identify potential islands}

In the midst of a cascading failure, it is sometimes recommended to avoid catastrophic wide area blackouts by means of \textit{intentional controlled islanding} (ICI)~\cite{Zhao2003,you2004}. In other words, by means of line switching actions, they temporarily partition the network into islands to prevent the cascading failure from propagating further and/or creating very imbalanced grid sections. Moreover, such an intentional islanding can enhance faster restoration of the full grid later and avoid transient stability issues during reconnection~\cite{you2003self,you2004}. 

The network operator ideally would want each of these islands to have:
\begin{itemize}
\item a net power as close as possible to zero, in the sense that power supply and demand should be almost equal, so that only minimal load shedding or generators adjustment are needed;
\item enough capacity to safely sustain the power flows within the island.
\end{itemize}
A lot of research has been devoted to the problem of finding a network partition with such properties, using either efficient search algorithms~\cite{Sun2003,Zhao2003}, mixed integer programming~\cite{Fan2012,Pahwa2013}, graph theory~\cite{Soltan2017}, or spectral clustering techniques~\cite{Esmaeilian2017,Bialek2014}. Similar methods have also been used in~\cite{Liu2009,Vittal2003,Vittal1998} to group together synchronized generators in case of frequency disturbance events. 

These island design principles are clearly very much aligned with those we outlined for bridge-blocks, see (F1) and (F2) in the previous section. In view of this similarity, we expect an optimal islands design based on weighted network modularity to be very effective, but a detailed exploration of this other application is out of the scope of the present paper.

Dynamically creating a bridge-block decomposition is proposed in~\cite{Bialek2021}  as a less drastic emergency measure in alternative to controlled islanding. The authors also classical spectral $k$-way clustering techniques to identify the optimal clusters to be transformed into bridge-blocks.
% \ale{\textbf{Possibly expand the literature overview and include some of these references?}

% Flexible constrained spectral clustering~\cite{WangDavidson2010} and applications to islanding~\cite{Ding2013}

% Controlled islanding~\cite{Kirschen2017,Kirschen2019,you2004}  

% Slow coherency-based islanding (two steps (i) classify generators and (ii) best cutset of transmission lines via exhaustive search~\cite{you2004}  \ale{NOT SCALABLE TO LARGE SYSTEM!}

% OBDD method for parallel restoration and sectionalizing of subsystems~\cite{WangVittal2011}

% blackout restoration using spectral clustering $w_{ij}=x_{ij}^{-1}$ + additional black start constraints ~\cite{QuirosTortos2014}. It's an alternative to the OBDD method

% minimizing load-generation imbalance is NP-hard~\cite{you2004} 

% Two-Step (first generators, then all the other nodes) Spectral Clustering Controlled Islanding Algorithm~\cite{Ding2013} \ale{NO GUARANTEES}

% two-steps algorithm: minimal cutsets for islanding (no edge weights) + minimum imbalance ~\cite{WangVittal2004} with WECC 129 example

% Swing equation with no damping \cite{Kirschen2019} two-step (selecting generators first, then solving min power-flow disruption on cutting edges)

% \cite{LiLiu2010} developed a hierarchical clustering method that takes into account the active and reactive power mismatch between areas. one edge weight obtained combining the one for active power and the one for reactive power.

% \cite{XuVittal2010} real power flow as edge weight + cutset determination after slow-coherency grouping
% }

% \ale{partitioning based on influence matrix = LODF matrix + Infomap for clustering~\cite{Panciatici2018}}

%In the next subsection we explore which network features and substructures are the most crucial to understand how failures can propagate and unravel their interplay with balancing schemes.

% ICI papers~\cite{Babaei2019,Babaei2021,Ding2013,Ding2017,Ding2018,FernandezPorras2018,Noebels2019,Pahwa2013,QuirosTortos2014,Tyuryukanov2017,Tyuryukanov2018,Tyuryukanov2019,Trodden2013,Teymouri2019,Tyuryukanov2020,Znidi2019,Vittal1998,Vittal2003,XuVittal2010,Sun2003,LiLiu2010,Kirschen2019}

\subsection{Building the bridge-block decomposition via optimal switching actions}
\label{sub:obs}

% \begin{figure}[!h]
% \centering
% \subfloat[The network $G$ with the partition $\calP$]{\includegraphics[width=0.45\textwidth]{tree_partition_newlabels1.png}}
% \subfloat[The corresponding multigraph $G_\calP$]{\includegraphics[width=0.45\textwidth]{tree_partition_newlabels2.png}}

% \caption{Example of reduced graph $G_\calP$.}\label{fig:tree_partition}
% \end{figure}

% A partition $\calP=\set{\calV_1,\calV_2,\cdots,\calV_k}$ of $G$ is said to be a \textit{tree partition} if the reduced graph $G_\calP$ is a tree. Every graph has always a tree partition, namely the trivial one $\calP=\set{V}$. In general, the tree partition of a graph $G$ is not unique (more specifically whenever $G$ has at least one cut edge). However, if we require the tree partition to be as ``fine'' as possible, such a partition is unique. More concretely, we can define a partial order $\succeq$ over the set of all tree partitions of a given graph (which is nonempty as it always contains the trivial partition $\calP_0$) as follows: For two tree partitions $\calP^1=\set{\calV_1^1,\calV_2^1,\cdots,\calV_{k_1}^1}$ and $\calP^2=\set{\calV_1^2,\calV_2^2,\cdots,\calV_{k_2}^2}$, we say $\calP^1$ is \emph{finer} than $\calP^2$, denoted as $\calP^1\succeq \calP^2$, if each subset in $\calP^1$ is contained in some subset in $\calP^2$. More precisely, $\calP^1\succeq \calP^2$ if for every $i=1,2,\ldots, k_1$, there exists some $j(i)\in \set{1,2,\ldots, k_2}$ such that $\calV_i^1\subset \calV_{j(i)}^2$. We illustrate two different tree partition for the same network in Fig.~\ref{fig:partition_order}).

% \begin{figure}[!h]
% \centering
% \includegraphics[width=.4\textwidth]{partition_order_newlabels.png}
% \caption{An illustration of the partial order $\succeq$ over tree partitions, in which $\calP^1=\set{\calV_1^1, \calV_2^1, \calV_3^1, \calV_4^1}$ is finer than $\calP^2=\set{\calV_1^2, \calV_2^2}$.}\label{fig:partition_order}
% \end{figure}

%\ale{[Adam: take more ownership throught this section. These are ``our'' results that we are surveying here for the OR audience!]}\\
% \alec{Check whether some of this material is still needed}\\
% \ale{\textbf{Remark:}  In the rest of the paper we will tacitly make this assumption, since any partition that does not satisfy this property can always be transformed into one that does (by adding individually all the connected components of each cluster to the partition). If two blocks are connected in $G_\calP$ by a single edge, then such an edge is a bridge of the original graph $G$.}
% A tree partition $\calP$ is said to be \textit{irreducible} if it is maximal with respect to the partial order $\succeq$. The irreducible tree partition of a graph $G$ is unique if $G$ is connected~\cite[Proposition 5]{Guo2018}, and, in this case, we denote it by $\calT(G)$. 

% \begin{prop}[Irreducible tree partition characterization]
% The irreducible tree partition $\calT(G)$ of a connected graph $G$ consists of the bridge-blocks and the reduced graph $G_{\calT(G)}$ associated to such partition is the bridge-block tree.
% \end{prop}
% In view of this result, it is clear that the problem of computing the irreducible tree partition reduces to finding all bridges of $G$. The algorithm introduced by~\cite{tarjan1974note} can thus be adapted to compute the irreducible tree partition of $G$ in $O(n+m)$ time.
% }

In the previous subsection we formulated the OBI problem, which for a given power network identifies a partition with desirable features that we want to transform into the ``backbone'' of the network bridge-block decomposition. In this subsection we focus on the second sub-problem, namely how to, given such a partition $\calP$, reconfigure the network topology so that the resulting network (i) has a bridge-block decomposition at least as fine as $\calP$ and (ii) has minimum line congestion. 

The feasibility and effectiveness of such a network reconfiguration crucially depends on the ``quality'' of the chosen partition $\calP$. Nonetheless, all the results of this section do not rely on any specific features of $\calP$ and they are valid for a general partition of $G$. The only additional assumption that we tacitly make in the rest of the section is the following:
\begin{itemize}
    \item[(A1)] for every cluster $\calV \in \calP$, the subgraph of $G$ induced by $\calV$ is connected.
\end{itemize}
Note that this is not really a stringent assumption: indeed, for any partition $\calP$ that does not satisfy it, we can always consider the finer partition $\calP'$ in which all the connected components of all its subgraphs are considered as separate clusters. Assumption (A1) is useful as it links the connectedness of the network with that of its reduced graph, as illustrated by the following lemma. 

\begin{lem}[Connectedness of the reduced graph] \label{lem:connected}
If $G$ is a connected graph, then the reduced graph $G_\calP$ is connected for any partition $\calP$. The converse is true only when the partition $\calP$ satisfies (A1). %is such that each of subgraphs induced by its clusters is connected.
\end{lem}
%Clearly, if $G$ is connected, so is any reduced graph $G_\calP$. The converse is true only when the partition $\calP$ is such that each of sugraphs induced by its clusters is connected. 

To any partition $\calP$ is associated a subset $E_c(\calP) \subset E$ of cross-edges, i.e., the edges whose endpoints belong to different clusters of $\calP$ (cf.~Subsection~\ref{sub:basic}). Given a partition $\calP$ of $G$, we are interested in finding a subset $\calE \subset E_c(\calP)$ of cross-edges that, if removed, yield a network $G^\calE$ whose bridge-block decomposition is at least as fine as $\calP$, i.e.,
\begin{equation}
\label{eq:BBGE}
    \calBB(G^\calE) \succeq \calP.
\end{equation}
Each of these subsets of cross-edges corresponds to a different set of transmission lines that we could temporarily disconnect by means of switching actions, which yields a transmission network topology with the desired bridge-block decomposition.
The next proposition shows that the condition~\eqref{eq:BBGE} is equivalent to requiring that the reduced graph induced by the partition $\calP$ on the post-switching network $G^\calE$ is a tree.
\begin{prop}[Reduced graph characterization]
\label{prop:treecharacterization}
Let $\calP$ be a vertex partition of a connected graph $G$. Then, $\calBB(G) \succeq \calP$ if and only if the reduced graph $G_\calP$ is a tree.
\end{prop}
\begin{proof}
Assume by contradiction that $G_\calP$ is not a tree and thus there exists a non-trivial cycle in $G_\calP$. Since we assume all the clusters of $\calP$ induce connected subgraphs, there exists also a non-trivial cycle $c$ in $G$ that includes vertices from at least two different clusters of $\calP$. Recall that by definition of bridge-block decomposition $\calP_{\mathrm{circuit}}(G) = \calBB(G)$ (cf. Subsection~\ref{sub:basic}), all the vertices on the cycle $c$ must belong to the same bridge-block, say $B \in  \calBB(G)$. But then $\calBB(G)$ cannot be finer than $\calP$ since the bridge block $B$ is not contained in any cluster in $\calP$, since it has vertices from at least two different clusters of $\calP$ and thus $B \not\subseteq V$ for every $V \in \calP$.

The reverse implication can be proved along the same lines, assuming by contradiction that $\calBB(G^\calE) \not\succeq \calP$ and leveraging again the connection between the circuits in $G$ and those in the reduced graph $G_\calP$.
\end{proof}

In view of Proposition~\ref{prop:treecharacterization}, we can assume that $G_\calP$ is not a tree, otherwise is suffices to take $\calE = \emptyset$ and the target condition~\eqref{eq:BBGE} is automatically satisfied. When the reduced graph $G_\calP$ is a not a tree (possibly with/because of multiple edges), there are many valid subsets of cross-edges $\calE \subset E_c(\calP)$ that satisfy the target property~\eqref{eq:BBGE}. Indeed, there exists a suitable subset of cross-edges for each spanning forest of the reduced graph $G_\calP$. Aiming to have the least impact possible on the network and, in particular, avoiding its disconnection, we exclude all the subsets $\calE \subset E_c(\calP)$ that are cut sets for the graph $G$ and thus we can focus on the spanning trees of the reduced graph $G_\calP$.

Among all these possible choices for the set $\calE$, we want to pick the one that has the least impact on the surviving network in terms of line congestion. We define as \textit{congestion} on a transmission line $\ell \in E$ the ratio between the absolute power flow on that line and its (thermal) capacity $C_\ell$, i.e., $|f_\ell|/C_\ell \geq 0$.

Assuming the power injections $\pp$ do not change, after the removal of the lines in any such subset $\calE \subset E_c(\calP)$, the power redistributes on the remaining $|E \setminus \calE|$ lines as described in Subsection~\ref{sub:noncut}, yielding a new vector of new power flows $\ff^\calE$. We define the \textit{network congestion level} $\gamma(\calE)$ as the maximum line congestion in the surviving graph $G^\calE$, i.e.,
\begin{equation}
\label{eq:congestionlevel}
	\gamma(\calE):=\max_{\ell \in E\setminus \calE} |f^\calE_\ell| / C_\ell.
\end{equation}
With a minor abuse of notation, we use $\gamma(\emptyset)$ to denote to the network congestion level of the original network where no lines have been removed yet, i.e., $\calE = \emptyset$. Power networks must be operated so that each line flow is strictly below the capacity of the corresponding line, meaning that the network congestion level should not be larger than one.
%Recall that $\calT(G^\calE)$ denotes the (unique) irreducible tree partition of the surviving network $G^\calE$.

The problem of finding the best set $\calE$ of switching actions that yields a network $G^\calE$ with minimum network congestion and bridge-block decomposition as fine as $\calP$ can be formalized as the following \textit{Optimal Bridge Selection} (OBS) problem:
\begin{subequations}\label{eq:optswitch}
\begin{align}
	 \min_{\calE \subset E_c(\calP)} \quad & \gamma(\calE) \qquad \qquad \qquad \textrm{(OBS)} \label{eq:optswitch_basic}\\
	 \textrm{ s.t. } \quad &(G^\calE)_\calP \text{ is a tree}. \label{eq:optswitch_constraint2}
\end{align}
\end{subequations}

The constraint~\eqref{eq:optswitch_constraint2}, by requiring the reduced graph $(G^\calE)_\calP$ of the post-switching network $G^\calE$ to be a tree (and not a forest), implicitly guarantees that $(G^\calE)_\calP$ is connected and therefore so is $G^\calE$ by virtue of Lemma~\ref{lem:connected}. In other words, for any feasible set $\calE$ for~\eqref{eq:optswitch} the resulting post-switching network $G^\calE$ is still connected.

In view of Proposition~\ref{prop:treecharacterization}, constraint~\eqref{eq:optswitch_constraint2} ensures that the bridge-block decomposition of the surviving network $G^\calE$ is at least as fine as $\calP$, but it can possible be finer. This happens when the removal of the cross-edges in $\calE$ accidentally creates additional bridges in $G^\calE$ that the original network did not have. By construction these new bridges were not cross-edges and thus must have been \textit{inside} one or more clusters of $\calP$. This means that the switching actions $\calE$ involuntarily split each of these clusters into two or more smaller bridge-blocks, and thus the resulting bridge-block decomposition $\calBB(G^\calE)$ is finer than $\calP$. This happens also in the example that we illustrate in the next subsection, see Fig.~\ref{fig:oneshotalgorithm}.
%Consider a subset $\calE \subset E_c(\calP)$ that satisfies constraint~\eqref{eq:optswitch_constraint2}. By construction, the cross-edges in $\calB_\calE := E_c(\calP) \setminus \calE$, automatically become bridges for $G^{\calE}$.
%For this reason, we consider a weight parameter $\alpha>0$ and augment the objective function of the optimization problem~\eqref{eq:optswitch} so that the optimal solution is the one with the minimal congestion on the newly created bridges, namely
%\begin{subequations}\label{eq:optswitch_augmented}
%\begin{align}
%	\min_{\calE \subset E_c(\calP)} \quad & \gamma(\calE) + \alpha \sum_{\ell \in \calB_\calE} |f^\calE_\ell| / C_\ell \label{eq:optswitch_aug}\\
%	% &  \calT(G^\calE) \succeq \calP, \label{eq:optswitch_aug_constraint1}\\
%	\textrm{ s.t. } \quad &(G^\calE)_\calP \text{ is a tree}. \label{eq:optswitch_aug_constraint2}
%\end{align}
%\end{subequations}
%Note that adding $\sum_{\ell \in \calB_\calE} f_\ell^{\calE}$
%and set $f^*:= f^{\calE^*}$ and $\gamma^*:= \|\gamma(\calE^*)\|_\infty$.
If $G_\calP$ is not a tree, the OBS problem~\eqref{eq:optswitch} has always at least one feasible nontrivial solution $\calE \neq \emptyset$ for any target partition $\calP$. Indeed, $G_\calP$ has at least one spanning tree as long as it is connected, property guaranteed by assumption (A1) and by Lemma~\ref{lem:connected}.

It could be the case that even for the optimal set $\calE^*$ of switching actions, at least one line gets congested, i.e.,
$$\gamma(\calE) \geq 1, \quad \text{ for every feasible subset } \calE.$$
This is a rare occurrence and, in fact, an optimal solution $\calE^*$ with congestion level $\gamma(\calE^*) < 1$ exists in most cases (see Section~\ref{sec:numerics} for our numerical results for IEEE test networks), especially if the original network was not heavily congested, i.e., $\gamma (\emptyset) \not\approx 1$. Furthermore, as we illustrate in the same section, it is often the case that the network congestion level \textit{decreases} after taking the optimal switching actions, i.e.,
\[
	\gamma(\calE^*) < \gamma (\emptyset).
\]
A possible explanation for this counter-intuitive fact is the presence of loop-flows involving edges in two or more clusters, which are then removed by the switching actions, hence possibly reducing the congestion on the newly created bridges or inside the clusters. %\alec{Steven remarks that maybe loop flows are not the only culprits?}

Since the optimal solution of the combinatorial OBS problem~\eqref{eq:optswitch} may not be unique, in which case we heuristically select the one that minimizes the total number of congested lines in the post-switching network. %congestion on the newly created bridges, i.e., $\sum_{\ell \in \calB_\calE} |f^\calE_\ell| / C_\ell$, where $\calB_\calE := E_c(\calP) \setminus \calE$. 
%\subsection{Practical considerations: recursive splitting and a stopping rule}

Lastly, we remark that an optimization problem similar to OBS is proposed in~\cite{Bialek2021} to refine the bridge-block decomposition as emergency measure. In their formulation, however, the objective is to minimize the total weight of the spanning tree $(G^\calE)_\calP$ of the reduced graph rather than minimizing the congestion in the post-switching network.

\subsection{Full algorithm and its recursive variant}
\label{sub:pra}
We now present in full our proposed algorithm by combining the two steps described in the previous subsections. Furthermore, we discuss some practical considerations regarding the implementation of the OBS problem. In particular, we show how the computational complexity of~\eqref{eq:optswitch} can be dramatically reduced by adopting a strategy where the bridge-block decomposition is progressively made finer by recursively splitting the existing bridge-blocks in smaller ones.
%This recursive approach has many advantages:
%\begin{itemize}
%\item it makes
%\end{itemize}

%Note that for each feasible subset $\calE$ of edges for the optimization problem~\eqref{eq:optswitch_augmented}, the cross-edges in $E_c(\calV)$ which are not removed automatically becomes bridges for the reduced graph $(G^\calE)_\calV$ and we denote their collection by $\calB_\calE := E_c(\calV) \setminus \calE$. By construction the bridges in $\calB_\calE$ form a spanning tree of the reduced graph $G_\calV$. Therefore, any admissible subset $\calE$ for the optimization problem~\eqref{eq:optswitch} is in one-to-one correspondence with a spanning tree of the reduced graph $G_\calV$.

By combining the OBI and OBS problems described in the previous subsections we obtain the following procedure to refine the bridge-block decomposition of a given power network $G$ with power injections $\pp$. This algorithm also requires in input the target number of bridge-blocks $b \in \mathbb{N}$.

\begin{algorithm}[!ht]
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{The power network $G=(V,E,\bm{b})$, the set of power injections $\pp$, the target number of bridge-blocks $b$}
\BlankLine
\DontPrintSemicolon
Calculate the current line flows $\ff$ on the network $G$ induced by the injections $\pp$;\\%and the current congestion level $\gamma_0=\gamma(\emptyset)$;\\
Calculate the current bridge-block decomposition $\calBB(G)$;\\
Consider in isolation the largest bridge-block in size of the current bridge-block decomposition, say $\calV \in \calBB(G_i)$;\\
Solve a OBI-$b$ problem for $\calV$ in isolation to find its optimal $b$-partition $\calP^*$;\\
Solve the OBS problem~\eqref{eq:optswitch} for $\calV$ in isolation with target $b$-partition $\calP^*$, obtaining an optimal subset $\calE^*_i$;\\
Calculate the new congestion level $\gamma^*=\gamma(\calE^*)$;\\
Calculate the new set of active lines to be $E' := E \setminus \calE^*_{i}$, set $G'=(V,E',\bm{b}')$, and calculate its bridge-block decomposition $\calBB(G')$;\\
\Output{$G'$, $\calBB(G')$, $\gamma^*$}
\caption{One-shot bridge-block decomposition refinement}\label{alg:oneshotrefinement}
\end{algorithm}
Fig.~\ref{fig:oneshotalgorithm} illustrates the steps of Algorithm~\ref{alg:oneshotrefinement} with $b=4$ when used to refine the bridge-block decomposition of the IEEE 73-bus network.

\begin{figure}[!ht]
    \centering
    \vspace{-0.3cm}
    \subfloat[The graph $G$ corresponding to IEEE 73 network with its bridge-block decomposition $\calBB(G)$ consisting of three bridge-blocks, two of which are trivial.]{\makebox[1.2\width]{\includegraphics[scale=0.39]{ieee73_1_original.png}}}
    \hspace{2cm}
    \subfloat[The bridge-block tree of $G$, i.e., the reduced graph $G_{\calBB(G)}$ corresponding to the bridge-block decomposition of the network in (a)]{\makebox[1.2\width]{\includegraphics[scale=0.39]{ieee73_1_bbd.png}}}
    \vspace{-0.3cm}\\
    \subfloat[The biggest bridge-block of the network in (a) is split into $b=4$ clusters by solving an OBI-$4$ problem, obtaining a finer partition $\calP^*$. The cross-edges of $\calP^*$ inside the original bridge-block are highlighted in red.]{\makebox[1.2\width]{\includegraphics[scale=0.39]{oneshot_ieee73_1_clustering.png}}}
    \hspace{2cm}
    \subfloat[The reduced graph $G_{\calP^*}$ corresponding to the optimal partition $\calP^*$ in (c), with the set $E_c(\calP^*)$ of its cross-edges highlighted in red. Each feasible set of switching actions corresponds to a spanning tree of $G_{\calP^*}$.]{\makebox[1.2\width]{\includegraphics[scale=0.39]{oneshot_ieee73_1_reducedgraph.png}}}
    \vspace{-0.3cm}\\
    \subfloat[The network $G'$ obtained after switching off the optimal subset $\calE^*$ consisting of $6$ cross-edges. The vertex colors display its bridge-block decomposition $\calBB(G')$, which is finer than the original one $\calBB(G)$.]{\makebox[1.2\width]{\includegraphics[scale=0.39]{oneshot_ieee73_2_original.png}}}
    \hspace{2cm}
    \subfloat[The bridge-block tree of $G'$, i.e., the reduced graph $G'_{\calBB(G')}$ corresponding to the new bridge-block decomposition $\calBB(G')$ of the post-switching network $G'$ in (e).]{\makebox[1.2\width]{\includegraphics[scale=0.39]{oneshot_ieee73_2_bbd.png}}}
    \caption{One-shot algorithm at work. Even if the goal was to split the biggest bridge-block into $b=4$ smaller ones, the algorithm returned a finer bridge-block decomposition consisting of $11$ bridge-blocks.}
    \label{fig:oneshotalgorithm}
\end{figure}
\FloatBarrier

Solving the one-shot bridge-block decomposition refinement presents several issues. Firstly, it is hard to determine a priori a reasonable target number $b$ of bridge-blocks, which is required as input of the algorithm: a small value would only yield a minor refinement of the network bridge-block decomposition, while a large one might yield only network with congested lines, i.e., $\gamma^* >1$.
Secondly, solving the OBS at the step 3 might be computationally very expensive. As mentioned earlier, the feasible sets $\calE \subset E_c(\calP)$ for the OBS problem~\eqref{eq:optswitch} are in one-to-one correspondence with the spanning trees of the reduced multi-graph $G_\calP$, which has at least $b$ nodes. 

Unfortunately, the OBS problem is not a minimum spanning tree problem, since the network congestion level appears in the objective function. For every spanning tree $T$ of $G_\calP$, we need to recalculate the power flows $\ff^\calE$ on the network $G^\calE$ obtained from the original one by removing the cross-edges that do not belong to that spanning tree, i.e., $\calE=E_c(\calP) \setminus T$. In view of this fact, the bottleneck of the above algorithm is precisely finding all such spanning trees of $G_\calP$. The time required to generate all spanning trees of a graph $G$ can be expressed as $O(g(b,|E_c(\calP)|) + \tau(G_\calP) h(b,|E_c(\calP)|)$ where $g,h$ are functions that are specific to the algorithm under consideration (see~\cite{Chakraborty2019} for a detailed overview), but it is largely dominated by $\tau(G_\calP)$, the number of spanning trees of $G_\calP$, that increases exponentially in the graph size $b$. 
%$\tau (G)$ can be computed in polynomial time for any graph using Kirchhoff’s matrix tree theorem).

This latter issue disappears if the selected target partition $\calP$ consists of only two clusters, say $\calV_1$ and $\calV_2$, as the reduced multi-graph $G_\calP$ has a number of spanning trees at most linear in the number of edges of the original network $G$. Indeed, in this case any spanning tree for $G_\calP$ consists of a single cross-edge in $E_c(\calP)$. Therefore, selecting a subset $\calE \subset E_c(\calP)$ of cross-edges between $\calV_1$ and $\calV_2$ feasible for the OBS problem is equivalent to choosing the unique cross-edge $e \in E_c(\calP)$ to keep, which become the unique bridge of the reduced graph $(G^\calE)_\calP$. Thus the number of feasible sets $\calE$ for the OBS problem is precisely equal to that of the cross-edges, and, trivially, $|E_c(\calP)| \leq |E|$.
Restricting ourselves to bi-partitions $\calP \in \Pi_2(G)$, the OBS problem~\eqref{eq:optswitch} becomes
\begin{equation}
	\min_{e \in E_c(\calP)} \gamma(E_c(\calP) \bs \{e\}) .
\label{eq:optswitch_tworegions}
\end{equation}
where the constraint~\eqref{eq:optswitch_constraint2} disappears because $(G^\calE)_\calP$ is always trivially a tree in this case. This optimization problem is much simpler and faster to solve than the original one: instead of optimizing over a complex combinatorial object, namely the family of spanning trees of the reduced graph $G_\calP$, the feasible set is just the collection of cross-edges $E_c(\calP)$.

This fact suggests the idea that it may be computationally more efficient to refine the bridge-block decomposition progressively, splitting the current largest bridge-block into two smaller bridge-blocks in a recursive fashion. We thus propose a second algorithm that leverages this idea. 
Besides drastically simplifying the structure of the OBS problem to be solved, this recursive approach embeds a natural stopping rule for the bridge-block decomposition refinement. As we hinted at already, it is impossible to estimate a priori how much the bridge-block decomposition of a power network can be refined without creating congestion on any line. In this respect, a procedure that increases the number of blocks by one at each step while monitoring the network congestion level can help find the best trade-off between the number of bridge-blocks and network congestion level. We introduce the following stopping rule. We keep refining the bridge-block decomposition splitting the largest bridge-block in a recursive fashion as long as:
\begin{itemize}
    \item[(i)] the current maximum number of splits is less than a predefined threshold $i_\mathrm{max} \in \N$, and
    \item[(ii)] the obtained network congestion level $\gamma^*$ is not larger than a threshold $\delta \in (0,1]$ describing the maximum tolerable congestion that the network operator can set.
\end{itemize}
%\alec{Mention here that the modularity problem can use the new flows (hence be more accurate) and using simpler spectral methods?}
The high-level structure of the proposed recursive procedure is shown in Algorithm~\ref{alg:recursiverefinement}.

\begin{algorithm}[!ht]
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{A power network $G=(V,E,\bm{b})$, a maximum number of iterations $i_\mathrm{max}$, and a congestion threshold $\delta$}
\BlankLine
\DontPrintSemicolon
Set $i=0$;\\
Set $E_0=E$ and $G_0=(V,E_0)$;\\
Calculate the line flows $\ff_0$ and the current network congestion level $\gamma_0^*:=\gamma(\emptyset)$;\\
\While{$\gamma^*_{i} < \delta$ \textbf{\textup{and}} $i < i_\mathrm{max}$}{
Calculate the current bridge-block decomposition $\calBB(G_i)$;\\
Consider in isolation the largest bridge-block in size of the current bridge-block decomposition, say $\calV \in \calBB(G_i)$;\\
Solve a OBI-2 problem for $\calV$ in isolation to find its optimal bipartition $\calP^*_i$;\\
Solve the simplified OBS problem~\eqref{eq:optswitch_tworegions} for $\calV$ in isolation with target bipartition $\calP^*_i$, obtaining an optimal subset $\calE^*_i \subset E_c(\calP^*_i)$ and the new network congestion level $\gamma^*_i=\gamma(\calE^*_i)$;\\
Calculate the new set of active lines to be $E_{i+1} := E_{i} \setminus \calE^*_{i}$ and set $G_{i+1}=(V,E_{i+1})$;\\
Increase $i$ by $1$;\\
}
\Output{$i$, $G_i$, $\calBB(G_i)$, $\gamma^*_i$}
\caption{Recursive bridge-block decomposition refinement}\label{alg:recursiverefinement}
\end{algorithm}
Note that in Step 6 we select the current largest bridge-block to be further split, so that all the bridge-blocks progressively become smaller, indirectly ensuring that, when the algorithm stops, the sizes of the resulting bridge-blocks are similar. However, we could tweak the algorithm to select either (i) the bridge-block with the lowest congestion level (inside which is probably safer to switch off lines without creating overloads) or (ii) the one with the highest potential to be clustered in terms of modularity score. Both these approaches, however, could possibly lead to ineffective bridge-block decompositions, where there are still very large bridge-blocks and several small (trivial) ones.

The OPS problem needs to be solved several times in this recursive variant (and not only once as prescribed in the one-shot variant, Algorithm~\ref{alg:oneshotrefinement}), which means that Algorithm~\ref{alg:recursiverefinement} requires possibly many more power flows calculations. However, a remarkable feature of the recursive approach is that all these power flow redistribution calculations can be done ``locally'' (i.e., inside the bridge-block that is being split) and thus become progressively faster as the size of the largest bridge-block decreases. More specifically, let $\calV$ be the bridge-block selected to be further split in Step 6 of Algorithm~\ref{alg:recursiverefinement}. By virtue of Proposition~\ref{prop:glodf_non_cut}, any switching action (which is effectively equivalent to line failure in this context) inside the bridge-block $\calV$ does not affect the line flows in any other bridge-block $\calV' \neq \calV$ of the current bridge-block decomposition. Therefore, only the line flows inside $\calV_i$ needs to be recalculated and this can be done by solving the DC power flow equations~\eqref{eq:flowsdc_model} only for the subgraph induced by $\calV$ and the corresponding local power injections. The only caveat is that we need to adjust the net power at all the nodes of $\calV$ that are endpoints of bridges to account for the outgoing flow. 

Adopting this recursive splitting strategy, the bridge-blocks become smaller at every iteration, which in turn means that fewer flows (and congestion levels) need to be recalculated at each step when solving the OBS problem~\eqref{eq:optswitch_tworegions}, making it increasingly faster to solve.

The recursive structure also makes Step 10 of Algorithm~\ref{alg:recursiverefinement} faster: the bridge-block decomposition does not have to be recomputed globally, since all the bridge-blocks but the one considered in this iteration will be unchanged and we only need to identify the new bridge-blocks created locally. We remark that this step cannot be skipped as the optimal set of switch action may accidentally split the considered bridge-block into more than two bridge-blocks.

Figs.~\ref{fig:recursivealgorithm_1} and~\ref{fig:recursivealgorithm_2} visualize the various steps that  Algorithm~\ref{alg:recursiverefinement} takes when set with $i_\mathrm{max}=2$ and applied to the same network considered in Fig.~\ref{fig:oneshotalgorithm}, namely the IEEE 73-bus network. It is clear that the OBS problem is essentially trivial for the recursive algorithm in both steps, see~Figs.~\ref{fig:recursivealgorithm_1}(d) and~\ref{fig:recursivealgorithm_2}(b), while it was more involved for the one-shot algorithm, cf.~Fig.~\ref{fig:oneshotalgorithm}(d).

\begin{figure}[!ht]
    \centering
    \vspace{-0.5cm}
    \subfloat[The graph $G_0$ corresponding to IEEE 73 network with its bridge-block decomposition $\calBB(G_0)$ consisting of three bridge-blocks, two of which are trivial.]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_1_original.png}}}
    \hspace{1cm}
    \subfloat[The bridge-block tree of $G_0$, i.e., the reduced graph $(G_0)_{\calBB(G_0)}$ corresponding to the bridge-block decomposition of the network in (a)]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_1_bbd.png}}}
    \vspace{-0.2cm}\\
    \subfloat[The biggest bridge-block of the network in (a) is split into 2 clusters by solving a simplified OBI-$2$ problem, obtaining a finer partition $\calP^*_0$. The cross-edges of $\calP^*_0$ inside the original bridge-block are highlighted in red.]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_1_clustering.png}}}
    \hspace{1cm}
    \subfloat[The reduced graph $G_{\calP^*_0}$ corresponding to the optimal partition $\calP^*_0$ in (c), with the set $E_c(\calP^*_0)$ of its cross-edges highlighted in red. The spanning trees of $G_{\calP^*_0}$ (and thus the feasible switching actions) to consider do not grow exponentially with the size of $G_{\calP^*_0}$, being in one-to-one correspondence with $E_c(\calP^*_0)$.]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_1_reducedgraph.png}}}
    \vspace{-0.2cm}\\
    \subfloat[The network $G_1$ obtained after switching off the cross-edges in $\calE^*_0$. The vertex colors display its bridge-block decomposition $\calBB(G_1)$, which is finer than the original one $\calBB(G_0)$.]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_2_original.png}}}
    \hspace{1cm}
    \subfloat[The bridge-block tree of $G_1$, i.e., the reduced graph $(G_1)_{\calBB(G_1)}$ corresponding to the new bridge-block decomposition of the post-switching network $G_1$ in (e).]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_2_bbd.png}}}
    \caption{Recursive algorithm at work -- first iteration $i=1$}
    \label{fig:recursivealgorithm_1}
\end{figure}
\FloatBarrier
\begin{figure}[!h]
    \centering   
    \subfloat[The biggest bridge-block of the network $G_1$ in Fig.~\ref{fig:recursivealgorithm_1}(e) is split into 2 clusters by solving a simplified OBI-$2$ problem, obtaining a finer partition $\calP^*_1$. The cross-edges of $\calP^*_1$ inside the original bridge-block are highlighted in red.]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_2_clustering.png}}}
    \hspace{1cm}
    \subfloat[The reduced graph $(G_1)_{\calBB(G_1)}$ corresponding to the bridge-block decomposition of the network in (a)]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_2_reducedgraph.png}}}
    \\
    \subfloat[The network $G_2$ obtained after switching off the cross-edges in $\calE^*_1$. The vertex colors display its bridge-block decomposition $\calBB(G_2)$, which is finer than the previous one $\calBB(G_1)$]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_3_original.png}}}
    \hspace{1cm}
    \subfloat[The bridge-block tree of $G_2$, i.e., the reduced graph $(G_2)_{\calBB(G_2)}$ corresponding to the new bridge-block decomposition of the post-switching network $G_2$ in (c).]{\makebox[1.25\width]{\includegraphics[scale=0.39]{ieee73_3_bbd.png}}}
    \caption{Recursive algorithm at work -- second iteration $i=2$}
    \label{fig:recursivealgorithm_2}
\end{figure}
\FloatBarrier
%\lguo{I think as the the iteration continues, the number of problems to solve also increases? The total amount of calculation should still go down though, because the complexity of solving a linear system is somewhere between $O(n^2)$ and $O(n^3)$, so the impact of having smaller problems dominate the impact of having more problems. Not sure if we want to rephrase a bit.}. \alec{The number of subproblems to solve does not explode due to the recursion. If we want $k$ regions, then we will solve exactly $k$ subproblems. Or am I overlooking something?}
%
%\alec{comment about and forward-reference counterexamples in Subsection~\ref{subcounterexample} in the numerical subsection about monotonicity and loop flows}
%
% \alec{Shrink and merge with earlier subsection}
Both the one-shot and the recursive algorithms focus on the scenario where the power injections are fixed. However, in practical settings the network operator could \textit{jointly} reconfigure the network topology by means of switching actions \textit{and} adjust (some of) the power injections, either by shedding load or by adjusting generator levels. In this scenario, the OBS problem could potentially find a solution with an even lower network congestion level, but analyzing this joint optimization problem or proposing heuristics leveraging this additional injection flexibility is beyond the scope of this paper. 

We remark that one such possible strategy, in the spirit of~\cite{Liang2021}, is aiming for local power adjustments and only change the power injections at the endpoints of each line that is being switched off by an amount exactly equal to its original flow on that line. This strategy would guarantee that the power flows on the entire surviving network will be unchanged and no congestion will be created. However, there might not be enough flexibility in terms of injection adjustment in each pair of endpoints. Alternatively, one can solve a global OPF problem for the whole network after the switching actions, hence ensuring that no line will be overloaded. Even better results could be obtained when considering the line switching and power injection adjustment jointly in the same optimization problem. 
%\alec{We probably need to argue here why we don't consider this latter strategy in this paper?} \adam{I think we can potentially remove all of this or at least minimize it...}
%
% \lguo{Now I think of it, adjusting the injections at removed bridges is a great idea! Essentially it guarantees flows on the surviving bridges do not change and thus all flow changes only happen within each partition block. Regardless, I feel we should highlight this point when formulating OBS? My current reading at OBS is that we only allow power redistribution but not adjustment.} \alec{This is not something we considered yet, but it could be a possible extension. How to decide what is the best injection adjustment? Should we essentially solve a local bridge-block OPF?}
% \lguo{I believe the ``optimal'' way for adjustment is to use the UC trick. But I meant something different here: I was proposing we adjust the injections at the removed bridge endpoints (by exactly the original flows), since the resulting power flows would be identical to that before bridge removals. This seems to be a nice property and may be helpful for further steps of the algorithm. One downside though, is that such adjustments may not always be feasible if these endpoints have a tight injection bound.}
%\chen{I'm a bit confused... Do the removed bridges and surviving bridges refer to the lines we switch off and the remaining lines as bridges? I think no matter how we adjust the injections (unless change the injections to be the same as the flow over switched lines), the flow change is likely to happen in both blocks. Am I missing anything here...?}
%
% \lguo{A couple of random ideas:
% \begin{itemize}
%     %\item  In contrast to the size, how about some other metrics for selecting the next block to divide further:
%     %\begin{enumerate}
%     %    \item Volume, that is, the sum of weights inside the block; \alec{wouldn't this criteria also pick the bridge-block which is hardest to refine/partition further?}
%     %    \item Congestion level within block, that is, we only further divide blocks whose current congestion level is low enough; \alec{Interesting, but how would you prevent this to just fragment a small bridge-block into many possibly trivial mini bridge-blocks while keeping the biggest (and say most congested) bridge-block untouched?}
%     %    \item Modularity; that is we only further divide a block if it shows potential of community structure. \alec{There isn't any proved strong relationship between a higher modularity score and the benefits for a finer BBD. At the same time, the congestion stopping criterion usually kicks in way sooner than the optimal number of clusters is reached (in terms of modularity score).}
%     %\end{enumerate}
%     %I doubt any of these would lead to noticeable impact for three iterations, but maybe it is good to comment on some of these? \alec{Yes, definitely} Conceptually, I think these fit better with the rest of our framework than size. \alec{But size still relates to the number of zeros in the (G)LODF matrix, right?} \lguo{I now agree these ideas probably won't work out... Let's not worry about them then!}
%     %\item At each iteration, are there multiple solutions leading to the same best congestion level? If so, which one did we pick? Not sure if we can do anything with this choice. \alec{In case of ties, we pick the one with the least number of line at full capacity} \lguo{Makes sense!}
%     \item Right now the partitions returned by recursive can be quite different from one-shot, since each step may impact the best bipartition for next iteration. What would happen in recursive if we use the same partition as one-shot, but recursively and greedily find the lines to switch off? This should retain the efficiency benefit of recursive, but may potentially bring its performance closer to one-shot in cases one-shot indeed performs better. \alec{Intriguing idea, but how to greedily choosing pairs of candidate bridge-blocks and removing lines while guaranteeing to still obtained a tree at the end? Doesn't seem a trivial task to me. Say, if you have identified four clusters with the one-shot algo, your reduced graph now is a (almost) complete graph with several multiedges, where to start pruning edges? Cf. Figure 3(d).}\lguo{I was thinking about not focusing on the pairs of blocks, but instead consider the set of all edges between these blocks. We then recursively remove the edge with ``minimal'' impact in proper sense, with the constraint that the resulting graph is still connected. Alternatively, maybe we can just choose the pairs randomly? My (likely problematic) belief is that how the blocks are formed might have a larger impact than how we select the edges to remove...} \alec{Your guess is indeed correct, the clustering plays the biggest role, which is also confirmed by the more extensive numerics that my master students is currently running.}
%     \item This idea is probably pushing too much: How about we do the UC trick here too, and solve an OPF within each new block to balance out the injections (in addition to adjusting the endpoints of removed lines). I suspect this would potentially give us much better numbers in terms of the final congestion. \alec{Probably won't fit in this paper, but, Chen, here's an idea for our next paper! :) On a more serious note, the UC trick here means you add the zero-balance constraints to the OPF and if needed you gradually relax them?} \lguo{Pretty much yeah!}
% \end{itemize}}

==> arxiv submission/redistribution.tex <==
\section{Distribution factors and power flow redistribution}
\label{sec:distfactor}
In this section we introduce two families of sensitivity factors of power networks, also known as \textit{distribution factors}. The first class is that of \textit{power transfer distribution factors} (PTDF), which describe how changes in power injections impact line flows. The second type of factors are the so-called \textit{generalized line outage distribution factors} (GLODF), which capture how line removal/outages impact power flows on the surviving lines. As illustrated in the previous section, if the power injections or the network topology change, one can always recompute the new line flows by solving the power flow equations~\eqref{eq:flowsdc_model}. The distribution factors are based on the DC approximation for power flows and provide fast estimates of the new line flows without solving again the AC power flow equations. For this reason, they have been widely used for security and contingency analysis when power flow solutions are computationally expensive, see~\cite[Chapter 7]{Wood2013}. %Usually only lines that might encounter congestion are monitored. The number of such lines is typically small even in a large network, and therefore such analysis is much simpler than solving for a power flow solution. For automatic contingency selection distribution factors can be used to quickly identify contingencies that will most stress a network. These contingencies are then selected for more detailed examination.

In this paper, we use distribution factors to analyze structural properties of power flow solutions and to design failure localization and mitigation mechanisms to reduce the risk of large-scale blackouts from cascading failures. In this section we unveil the deep connection between the distribution factors and specific substructures of the power network topology, complementing~\cite{Ronellenfitsch2017,Strake2019}. We henceforth assume the power network to be connected. The rest of the section is structured as follows. We first focus on the impact of power injection changes on line flows in Subsection~\ref{sub:PTDF}, introducing the PTDF factors and matrix and showing how they can be calculated in terms of spectral quantities. We then illustrate the effect of network topology changes on power flows. In our analysis we distinguish two very different cases. In Subsection~\ref{sub:noncut} we look at the scenario in which the set of outaged/removed lines does not disconnect the power network, obtaining the close-form expression for the GLODFs. In Subsection~\ref{sub:cut} we consider the more involved case in which the outaged lines disconnect the power network into multiple islands and show how the impact of topology change can be clearly distinguished from that of the balancing rule that needs to be invoked to rebalance the power in each of these newly created islands.

\subsection{Power transfer distribution factors (PTDF)}
\label{sub:PTDF}
The goal of this subsection is to analyze the effect of power injections change on line flows. We will use $\tilde{\cdot}$ to denote variables after such a change (possibly a contingency, but not exclusively).

Consider two nodes $s,t \in V$ (not necessarily adjacent) and a scalar $\delta_{\hi\hj}$ describing an injection change, which can be either positive or negative. Suppose the injection at node $\hi$ is increased from $p_{\hi}$ to $\tilde p_{\hi} := p_{\hi }+ \delta_{\hi\hj}$ and that at node $\hj$ is reduced from $p_{\hj}$ to $\tilde p_{\hj} := p_{\hj} - \delta_{\hi\hj}$, while all other injections remain unchanged $\tilde p_i = p_i$, $i \neq \hi, \hj$, so that
\[
	\tilde{\pp} =  \pp + \delta_{\hi \hj} (\mathbf{e}_{\hi} - \mathbf{e}_{\hj})
\]
remains balanced, i.e., $\sum_{i\in V} \tilde p_i = \sum_{i\in V} p_i = 0$. Note that this is an equivalent condition a power injection for being balanced since we assumed that $G$ is connected and thus $\mathrm{ker}(L)=\bm{1}$ (cf.~Proposition~\ref{ch:lm; eq:Laplacian-properties}).
%In general we will use $\tilde{\cdot}$ to denote variables after a contingency, e.g., injections are changed from $\pp$ to $\tilde \pp$, a power flow is changed from $f_\ell$ to $\tilde f_\ell$ on line $\ell=(i,j)$.

The \textit{power transfer distribution factor} (PTDF) $D_{\ell, \hi\hj}$, also called the \textit{generation shift distribution factor}, is defined to be the resulting change $\Delta f_{\ell} := \tilde f_{\ell} - f_{\ell}$ in the line flow on line $\ell$ normalized by $\delta_{\hi\hj}$:
\[
	D_{\ell, \hi\hj} := \frac{\Delta f_{\ell}}{\delta_{\hi\hj}} =  \frac{\tilde f_{\ell} - f_\ell }{\delta_{\hi\hj}}.
\]
For convenience $D_{\ell,\hi\hj}$ is defined to be $0$ if $i=j$ or $\hi = \hj$. The next proposition shows how this factor can be computed from the pseudo-inverse $L^\dag$ of the graph Laplacian matrix $L$ or, alternatively, in terms of the spanning forests of $G$. 
\begin{prop}[PTDF $D_{\ell,\hi \hj}$]
\label{ch:lm; prop:PTDF.1}
Given a connected power network $G = (V, E, \bm{b})$, the following identities hold for every line $\ell = (i, j)\in E$ and any pair of nodes $\hi, \hj \in V$:
%\begin{itemize}
%\item[(i)] $D_{\ell, \hi\hj} \ \ = \ \ b_{\ell} \left( L^\dag_{i\hi} +  L^\dag_{j\hj} -  L^\dag_{i\hj} -  L^\dag_{j\hi} \right)$;
%
%\item[(ii)] $ \displaystyle D_{\ell, \hi \hj} = b_{\ell} \frac{\sum_{\calE\in T(i\hi, j\hj)}\, \beta(\calE) \ - \ \sum_{\calE\in T(i\hj, j\hi)}\, \beta(\calE)}{\sum_{\calE\in T}\, \beta(\calE)}$.
%\end{itemize}
\begin{equation}
\label{eq:Dlst}
    D_{\ell, \hi\hj} \ = \ b_{\ell} \left( L^\dag_{i\hi} +  L^\dag_{j\hj} -  L^\dag_{i\hj} -  L^\dag_{j\hi} \right) \ = \ b_{\ell} \ \frac{\sum_{\calE\in T(\{i,\hi\}, \{j,\hj\})}\, \beta(\calE) \ - \ \sum_{\calE\in T(\{i,\hj\}, \{j,\hi\})}\, \beta(\calE)}{\sum_{\calE\in T}\, \beta(\calE)}.
\end{equation}
\end{prop}
Recall that $T(\{i,\hi\}, \{j,\hj\})$ has been defined in Section~\ref{sec:spectral} as the collection of spanning forests of $G$ consisting of exactly two disjoint trees, one containing nodes $i$ and $\hi$ and the other one containing nodes $j$ and $\hj$ (the definition of $T(\{i,\hj\}, \{j,\hi\})$) is analogous).
The proof easily follows combining~\cite[Theorem 4]{TPS1} and the properties of the pseudo-inverse $L^\dag$ derived in~\cite{Guo2017}.
Besides the precise spectral relation with pseudo-inverse of the graph Laplacian, the previous proposition shows that the PTDFs depend \textit{only on the topology and line susceptances} and are thus independent of the injections $\pp$. We remark that the insensitivity of the PTDFs to injections is, however, specific to the DC power flow approximation, which yields a linear relation between power injections and line flows.

As noted above, $D_{\ell,\hi \hj}$ is the change in power flow on line $\ell$ when a unit of power is injected at node $\hi$ and withdrawn at node $\hj$ where nodes $\hi$ and $\hj$ need not be adjacent.  When they are adjacent, i.e., $\hat \ell := (\hi, \hj)$ is a line in $E$, then the PTDFs define a $m\times m$ matrix $D := ( D_{\ell\hat \ell}, \, \ell, \hat \ell\in E)$, to which we refer as the \textit{PTDF matrix}. %We write $D_{\ell\hat \ell}$ in place of $D_{\ell, \hat \ell}$ when there is no danger of confusion.
The following proposition summarizes some properties of the PTDF matrix that already appeared without proof in~\cite[Corollary 5]{TPS1}. A detailed proof is thus provided in the Appendix.
\begin{prop}[PTDF matrix]
\label{ch:lm; prop:PTDF.2}
If $G = (V, E, \bm{b})$ is a connected power network, then the following properties hold for the PTDF matrix $D= ( D_{\ell\hat \ell}, \, \ell, \hat \ell\in E)$:
\begin{itemize}
\item[(i)] $D \ = \  B C^T  L^\dag  C$.

\item[(ii)] For every line $\ell \in E$ the corresponding diagonal entry of the PTDF matrix $D$ is given by
	\[
	D_{\ell \ell} = 1 \ - \ \frac{ \sum_{\calE\in T\!\setminus\! \{\ell\}} \beta(\calE) } { \sum_{\calE\in T} \beta(\calE) }.
	\]
	Hence, in particular, $0<D_{\ell\ell} \leq 1$.
\item[(iii)] For every line $\ell = (i,j) \in E$ the corresponding diagonal entry of the PTDF matrix $D$ is given by
	\[
	D_{\ell \ell} = b_{\ell} \left( L^\dag_{ii} +  L^\dag_{jj} -  2 L^\dag_{ij} \right) = b_{\ell} R_{ij}.
	\]
\end{itemize}
\end{prop}
Identity (ii) reveals that the more ways to connect every node without going through $\ell = (i,j)$, the smaller $D_{\ell\ell}$ is, i.e., the smaller it is the impact on the power flow on line $\ell$ when a unit of power is injected and withdrawn at nodes $i$ and $j$ respectively.

Recall that $T\!\setminus\! \{\ell\}$ is the collection of all spanning trees of $G$ consisting of edges in $E\!\setminus\! \{\ell\}$. Using~\eqref{eq:effr} and the fact that if $\ell$ is a bridge, then $T\!\setminus\! \{\ell\} = \emptyset$, we immediately obtain the following spectral characterization for the bridges of the network.
\newpage
\begin{cor}[Spectral characterization of network bridges]
\label{ch:lm; corollary:PTDF.3}
If $G = (V, E, \bm{b})$ is a connected power network, the following three statements are equivalent:
\begin{itemize}
\item Line $\ell$ is a bridge;
\item $D_{\ell\ell} = 1$;
\item $R_{ij} = L^\dag_{ii} +  L^\dag_{jj} -  2 L^\dag_{ij} = b_{\ell}^{-1}$.
\end{itemize}
\end{cor}
The proof immediately follows from the statements (ii) and (iii) of Proposition~\ref{ch:lm; prop:PTDF.2} noticing that line $\ell$ is a bridge if and only if it belongs to \textit{any} spanning tree of the power network $G$, or equivalently $T\!\setminus\! \{\ell\}=\emptyset$. %Combining~\cite[Corollary 5]{TPS1} with~\cite[Lemma 1]{Soltan2017b}.

Lastly, we present a sufficient condition for having zero PTDF in purely topological terms. Its proof is given in the Appendix and relies on the representation of the PTDF in terms of spanning forests given in~\eqref{eq:Dlst}.
\begin{thm}[Simple Cycle Criterion for PTDF]
\label{thm:zeroPTDF}
If there is no simple cycle in a power network $G = (V, E, \bm{b})$ that contains both lines $\ell$ and $\hat \ell$, then $D_{\ell \hat \ell} = 0$.
\end{thm}

\subsection{GLODF for non-cut set}
\label{sub:noncut}
%\chen{We use $\calE$ for both line failures and elements of spanning forests ($\calE \in T$). We may change one of them?} \alec{I think there is no confusion, also because a spanning forest is a subset of edges for us. Can you pinpoint to the exact place which you think is confusing, Chen?}
Consider a connected power network $G=(V,E, \bm{b})$ with balanced injections $\pp$. When a subset of lines $\calE \subset E$ trips or is removed from service, the network topology changes and, as a consequence, the power flow redistributes on the \textit{surviving network} $G^\calE :=(V,E \setminus \calE)$ as prescribed by power flow physics.%, possibly causing overloads in some of the other lines, not necessarily adjacent to the removed ones in $\calE$. 
To fully understand the power flow redistribution and unveil the impact of network topology on the flow changes, we distinguish two scenarios, depending on whether $\calE$ is a cut set or not for the power network $G$, and analyzed them separately. 

Even if the disconnection of the subset of lines $\calE \subset E$ can be deliberate, for instance due to maintenance or network optimization (as it will be the case in the Section~\ref{sec:optimization}), in most cases it is due to a \textit{contingency}, e.g., a line or node (bus) failure. For this reason and for conciseness, we present the next family of distribution factors using the standard power system terminology, referring to the lines in $\calE$ as \textit{outaged lines} and distinguishing between \textit{pre-contingency} and \textit{post-contingency line flows}.

Let $\calE\subsetneq E$ be any non-cut set of $k:=|\calE|$ lines that are simultaneously removed from the power network. The resulting surviving network $G^\calE=(V,E\setminus \calE)$ is still connected. Assuming that the injections $\pp$ remain unchanged (and thus balanced), the new power flows can be calculated directly from~\eqref{eq:flowsdc_model} after having updated the matrices $B$, $C$, and $L$ to reflect the structure of the surviving network $G^{\calE}=(V,E\setminus \calE)$. We now review this calculations in more detail and show how it leads to the notion of \textit{generalized line outage distribution factors (GLODFs}. These factors quantify the impact of the removal of each line in $\calE$ to each of the survival lines and are thus essential for any power network contingency analysis.

We first introduce some auxiliary notation. Let $\ff_\calE$ be the vector of the pre-contingency power flows on the outaged lines in $\calE$ and let $\ff_{-\calE}$ and $\tilde \ff_{-\calE}$ be the pre and post-contingency power flows respectively on the surviving lines in $-\calE := E\!\setminus\! \calE$. 
%We are particularly interested in characterizing how the flows change after removing the subset $\calE$ of lines assuming that injections $\pp$ remain unchanged.
Partition the susceptance matrix $B$ and the incident matrix $ C$ into submatrices corresponding to surviving lines in $-\calE$ and outaged lines in $\calE$:
\begin{equation}
	B \ =: \ \textup{diag} (B_{-\calE}, \, B_{\calE}), \qquad  C \ =: \ [ C_{-\calE} \ \  C_{\calE}].
\label{ch:cf; subsec:LODF; eq:BCpartitions.1}
\end{equation}
Assuming that the injections $\pp$ remain unchanged, we can calculate the post-contingency network flows by solving the DC power flow equations~\eqref{eq:flowsdc_model}
$
	\tilde \ff_{-\calE} \ = \ B_{-\calE}  C_{-\calE}^T  L_{-\calE}^\dag  \pp,
$
expressed in terms of the Laplacian matrix $ L_{-\calE} :=  C_{-\calE} B_{-\calE}  C_{-\calE}^T$ of the surviving network. 

The main result of this section shows that for a non-cut set $\calE \subsetneq E$ the post-contingency flow net changes $\Delta \ff_{-\calE} := \tilde \ff_{-\calE} - \ff_{-\calE}$ depend linearly on the pre-contingency power flows $\ff_\calE$ on the outaged lines. Their sensitivity to $\ff_\calE$ defines a $|E \bs \calE| \times |\calE|$ matrix $K^\calE := (K^\calE_{\ell\hat \ell}, \ell\in E\setminus\! \calE, \hat \ell \in \calE)$, called the \textit{Generalized Line Outage Distribution Factor} (GLODF) matrix, through
\[
	\Delta \ff_{-\calE} = K^\calE \, \ff_\calE,
\]
i.e., $\Delta f_\ell = \tilde f_\ell - f_\ell \ = \ \sum_{\hat \ell\in \calE}\, K^\calE_{\ell\hat \ell} f_{\hat \ell}$, for any $\ell\in E\setminus\! \calE$. Like the PTDFs, also the GLODFs depend solely on the network topology and susceptances, as illustrated by the next theorem, which shows how the GLODF matrix $K^{\calE}$ can be calculated using spectral quantities.

To state this result, we first need some additional notation. Partition the PTDF matrix $D$ into submatrices corresponding to non-outaged lines in $-\calE$ and outaged lines in $\calE$, possibly after permutations of rows and columns. Since $D \ = \  B C^T  L^\dag  C$ from Proposition \ref{ch:lm; prop:PTDF.2}(i), these different blocks of $D$ can be written explicitly in terms of the submatrices of $B$ and $C$ introduced in~\eqref{ch:cf; subsec:LODF; eq:BCpartitions.1}:
\begin{equation}
	D = \begin{bmatrix} D_{-\calE, -\calE} & D_{-\calE\calE} \\ D_{\calE, -\calE} & D_{\calE\calE} \end{bmatrix} = 
	\begin{bmatrix} 
	B_{-\calE} C_{-\calE}^T  L^\dag  C_{-\calE} & B_{-\calE} C_{-\calE}^T  L^\dag  C_{\calE} \\ 
	B_{\calE} C_{\calE}^T  L^\dag  C_{-\calE} & B_{\calE} C_{\calE}^T  L^\dag  C_{\calE} \\
	\end{bmatrix}.
	\label{ch:cf; subset:glodf; eq:decomposeD.1}
\end{equation}
%These explicit expressions will prove useful later in the study of the GLODF $K^\calE$ and failure localization. The next result generalizes the property $1 - D_{\hat \ell\hat \ell}>0$ in Proposition \ref{ch:lm; prop:PTDF.2} from the case of a non-bridge $\hat \ell$ outage to the case of a non-cut set outage.
%\begin{lemma} \label{ch:lm; lemma:invertibleM}
%The matrix $I - D_{\calE\calE} \ = \ I - B_{\calE}  C_{\calE}^T  L^\dag  C_\calE$ is invertible provided that $\calE$ is a non-cut set.
%\end{lemma}

We now express the GLODF matrix $K^\calE$ explicitly in terms of the PTDF submatrices introduced in~\eqref{ch:cf; subset:glodf; eq:decomposeD.1}.
%and then to the submatrix $K_{-\calE\calE} := \left( K_{\ell\hat \ell},\, \ell\in -\calE, \, \hat \ell\in \calE \right)$ of the LODF matrix $K$ in Table \ref{ch:cf; subsec:lodf; table:notations} using \eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}.

\begin{thm} [GLODF $K^\calE$ for non-cut set outage]
\label{ch:cf; thm:LODF.3}
Let $\calE\subsetneq E$ be a non-cut set outage for the power network $G=(V,E, \bm{b})$. %of lines that trip simultaneously so that the surviving graph $(V, E\!\setminus\! \calE)$ remains connected. 
Then, the matrix $I - D_{\calE\calE} \ = \ I - B_{\calE}  C_{\calE}^T  L^\dag  C_\calE$ is invertible and the net line flow changes $\Delta \ff_{-\calE}$ are given by
\begin{equation}
	\Delta \ff_{-\calE} = K^\calE \, \ff_\calE,
\label{ch:cf; subsec:lodf; eq:defKlF}
\end{equation}
where the GLODF matrix can be calculated as
\begin{equation}
	K^\calE  =  D_{-\calE\calE}\, \left( I - D_{\calE\calE} \right)^{-1} = B_{-\calE}  C_{-\calE}^T  L^\dag  C_\calE \left( I - B_{\calE}  C_{\calE}^T  L^\dag  C_\calE \right)^{-1}.
\label{ch:cf; eq:GLODF.1}
\end{equation}%
\end{thm}
The proof is immediate using~\cite[Theorem 7]{TPS1}, after reformulating the results appearing there in terms of the inverse of reduced Laplacian matrix $A$ using the pseudo-inverse $L^\dag$ using the identities proved in~\cite{Guo2017}. 

This formula of $K^\calE$ is derived by considering the pre-contingency network with changes $\Delta \pp$ in power injections that are judiciously chosen to emulate the effect of simultaneous line outages in $E$. The reference \cite{AlsacStottTinney1983} seems to be the first to introduce the use of matrix inversion lemma to study the impact of network changes on line currents in power systems. This method is also used in \cite{StottAlsacAlvarado1985} to derive the GLODF for ranking contingencies in security analysis. The GLODF has also been derived earlier, e.g., in \cite{EnnsQuadaSackett1982}, and re-derived recently in \cite{GulerGrossLiu2007, GulerGross2007}, without the simplification of the matrix inversion lemma.

%We now extend the results on LODF from a non-bridge outage to a non-cut set outage. 

%We pause to clarify notations; see Table \ref{ch:cf; subsec:lodf; table:notations}.
%\begin{table*}[htbp]
%\centering
%\begin{tabular}{ || l | l ||}
%	\hline\hline
%	\textbf{GLODF} & \textbf{Non-cut set outage} \\
%	\hline
%	$K^\calE_{\ell\hat \ell}$	& Sensitivity (a scalar) of power flow on a surviving line $\ell \in -\calE$ due to the outage of  \\
%	&  line $\hat \ell\in \calE$ when a non-cut set $\calE$ of lines are outaged \emph{simultaneously}(see \eqref{ch:cf; subsec:lodf; eq:defKlF}).  \\
%	\hline
%	$K^\calE_{L\hat L}$ & $|L|\times |\hat L|$ matrix whose $(\ell, \hat \ell)$-th entry is $K^\calE_{\ell\hat \ell}$, with $L\subseteq -\calE$ and $\hat L \subseteq \calE$. \\
%	\hline
%	$K^\calE := K^\calE_{-\calE\calE}$ 	& $(m-k) \times k$ matrix in \eqref{ch:cf; subsec:lodf; eq:defKlF} whose $(\ell, \hat \ell)$-th entry is $K^\calE_{\ell\hat \ell}$ for $\ell\in -\calE$, $\ell\in \calE$. \\
%	\hline \hline 
%	\textbf{LODF}		& \textbf{Non-bridge outage} \\
%	\hline
%	$K_{\ell\hat \ell} := K^{\hat \ell}_{\ell\hat \ell}$  &  The $\ell$-th entry of the column vector $K^{\hat \ell}$.  \\
%	\hline
%	$K^{\hat \ell} := K^{\hat \ell}_{-\hat \ell, \ell}$ & A size $m-1$ column vector $K^{\hat \ell} = K^\calE_{-\calE\calE}$ when $\calE = \{\hat \ell\}$.  It is the $\hat \ell$-th column of  \\
%	& $K$ in \eqref{ch:cf; subsec:lodf; eq:KDpartitions.1} without the diagonal entry $K_{\hat \ell\hat \ell}$.\\
%	\hline
%	$K_{-\calE\calE}$ 	& $(m-k) \times k$ submatrix of $K$ in \eqref{ch:cf; subsec:lodf; eq:KDpartitions.1} whose $(\ell, \hat \ell)$-th 	entry is $K_{\ell\hat \ell}$ for $\ell\in -\calE$, $\ell\in \calE$. \\
%	\hline\hline
%\end{tabular}
%\caption{GLODF $K^\calE$ and LODF $K^{\hat \ell}$ notations. %Note that the $(\ell, \hat \ell)$-th entry of $K^F$ is$K^F_{\ell\hat \ell}$ whereas that of $K_{-FF}$ is $K_{\ell\hat \ell}$. In general $K^F \neq K_{-FF}$ (see \eqref{ch:cf; eq:GLODF.1c} below for their relationship).
%}
%\label{ch:cf; subsec:lodf; table:notations}
%\end{table*}
%Despite notational similarities and the same size $(M-m)\times m$, the GLODF $K^F$ when a non-cut set $F$ of lines are outaged simultaneously are different from the LODF $K_{-FF}$ when each non-bridge line $\hat \ell\in F$ is outaged separately (their relation is clarified in \eqref{ch:cf; eq:GLODF.1c} below).
%The matrix $K^F$ specifies the post-contingency flow changes on lines $\ell\in -F$ when all lines in $F$ trip \emph{simultaneously} whereas the $\hat \ell$-th column of $K_{-FF}$ specifies the post-contingency flow changes on lines $\ell \in -F$ when a \emph{single} line $\hat \ell\in F$ trips.
%When $F = \{\hat \ell\}$, \eqref{ch:cf; subsec:lodf; eq:defKlF} reduces to \eqref{ch:cf; subsec:lodf; eq:defKlhatl.1b} and $K^F$ reduces to $K^{\hat \ell}$.    % , the $\hat \ell$-th column of $K_{-FF}$.

\subsubsection{Non-bridge outages}
\label{sub:lodfnonbridge}
We now briefly consider the special case in which the subset $\calE$ of outaged lines is still a non-cut set, but consists of a single line, i.e., $\calE = \{ \hat \ell\}$. Since the singleton $\{\hat \ell\}$ is a cut set if and only if $\hat \ell$ is a bridge, we are thus focusing on \textit{non-bridge line outages}.

The GLODF matrix $K^\calE$ introduced earlier rewrites now as a vector $(K_{\ell\hat \ell}, \ell \in E\setminus\! \{\hat \ell\})$, where, since there is no ambiguity, we suppressed the superscript ${\{\hat \ell\}}$ for compactness. We recover in this way the so-called \textit{line outage distribution factor} (LODF) $K_{\ell\hat \ell}$, which is formally defined to be the change $\Delta f_\ell := \tilde f_\ell - f_\ell$ in power flow on surviving line $\ell \neq \hat \ell$ when a \textit{single non-bridge} line $\hat \ell$ trips, normalized by the pre-contingency line flow $f_{\hat \ell}$:
\[
	K_{\ell\hat \ell}  :=  \frac{\Delta f_\ell}{f_{\hat \ell}}, \qquad \ell \neq \hat \ell \in E, \ \text{for non-bridge line }\hat \ell
\]
assuming that the injections $ \pp$ remain unchanged, cf.~\cite{Wood2013} and \cite{Guo2017}. The LODFs for non-bridge outages inherit all the properties of GLODFs for non-cut sets and, in particular, they are also independent of $\pp$. The next proposition reformulates the results in Theorem~\ref{ch:cf; thm:LODF.3} in the case of a single non-bridge failure, and relates the LODF to the weighted spanning forests of pre-contingency network; see~\cite[Theorem 6]{TPS1} for the proof of this latter fact.
%
\begin{prop}[LODF $K_{\ell \hat \ell}$ for non-bridge outage]
\label{ch:lm; thm:LODF.1}
Let $\hat \ell = (\hi, \hj)$ be a non-bridge outage that does not disconnect the power network $G=(V,E,\bm{b})$.
%Suppose a non-bridge $\hat \ell = (\hi, \hj)$ trips so that the surviving graph $G^{\{\hat \ell\}} = (V, E\!\setminus\! \{\hat \ell\})$ remains connected.
For any surviving line $\ell = (i, j) \neq \hat \ell$ the corresponding LODF is given by
\begin{equation}
K_{\ell \hat \ell} = \frac{D_{\ell\hat \ell}} {1 - D_{\hat \ell \hat \ell}} \ \ = \ \ 
	\frac{ b_{\ell} \left(  L^\dag_{i\hi} +  L^\dag_{j\hj} -  L^\dag_{i\hj} -  L^\dag_{j\hi} \right) }{ 1 \ - \ b_{\hat \ell} \left(  L^\dag_{\hi\hi} +  L^\dag_{\hj\hj} - 2 L^\dag_{\hi\hj} \right) }
	  = \frac{ b_{\ell} \left( R_{i\hj}-R_{i\hi}+R_{j\hi}-R_{j\hj}\right)}{2(1-b_{\hat \ell} R_{st})}
\label{ch:lm; eq:LODF.1a}
\end{equation}
and can be equivalently be expressed in terms of the spanning forests of $G$ as
\begin{equation}
	K_{\ell \hat \ell} = \frac{b_{\ell}} {\sum_{\calE\in T\!\setminus\! \{\hat \ell\} }\, \beta(\calE)} \Big( \sum_{\calE\in T(\{i,\hi\}, \{j,\hj\})} \beta(\calE) - \sum_{\calE\in T(\{i,\hj\}, \{j,\hi\})}\, \beta(\calE) \Big).
\label{ch:cf; subsec:lodf; eq:Kllhat.1}
\end{equation}
\end{prop}
Identity~\eqref{ch:lm; eq:LODF.1a} can be equivalently derived using a rank-$1$ update of the pseudo-inverse $L^\dag$ as done by~\cite{Soltan2017b}. Each LODF accounts for all the alternative paths on which the power originally carried by line $\hat \ell$ can flow in the new topology and for how many of these the line $\ell$ belongs to. This dependence is made explicit in~\eqref{ch:cf; subsec:lodf; eq:Kllhat.1} in terms of the weighted spanning forests.

Recall that Proposition \ref{ch:lm; prop:PTDF.2} shows that $D_{\hat \ell \hat \ell} = 1$ if and only if line $\hat \ell$ is a bridge, which corroborates the fact that \eqref{ch:lm; eq:LODF.1a} is valid only for non-bridge failures.
We remark that, differently from the diagonal entries $(D_{\ell \ell}, \ell \in E)$ of the PTDF matrix, the factor $D_{\ell\hat \ell}$ can take any sign and thus so can $K_{\ell\hat \ell}$.
%
From~\eqref{ch:cf; subsec:lodf; eq:Kllhat.1} we immediately deduce that $K_{\ell\hat \ell}>0$ if $\ell$ and $\hat \ell$ share either the source node ($i = \hi$) or the terminal node ($j=\hj$), since in this case $T(\{i,\hj\}, \{j,\hi\}) = \emptyset$. 

We can also express LODF in \eqref{ch:lm; eq:LODF.1a} in matrix form and relate it to the PTDF matrix $D$ defined in Subsection~\ref{sub:PTDF}. Partition the edge set $E$ in two subsets, $E^\textup{b}$ and $E^\textup{n}$, by distinguishing between bridges and non-bridge lines and set $m_\textup{b}:=|E^\textup{b}|$ and $m_\textup{n}:=|E^\textup{n}|$. Consider the $m \times m_\textup{n}$ matrix $K^\textup{n} := \big( K_{\ell\hat \ell}\, , \, \ell \in E, \hat \ell \in E^\textup{n} \big)$ and $D^\textup{n} := \big( D_{\ell\hat \ell}\, , \, \ell \in E, \hat \ell \in E^\textup{n} \big)$ and rewrite them into two submatrices, possibly after permutations of rows and columns:
\[
	K^\textup{n} \ \ = \ \ \begin{bmatrix} K_\textup{bn} \\ K_\textup{nn} \end{bmatrix},  \qquad 
	D^\textup{n} \ \ = \ \ \begin{bmatrix} D_\textup{bn} \\ D_\textup{nn}  \end{bmatrix}
\]
%The partitions of $K$ and $D$ are illustrated in Fig. \ref{ch:cf; subsec:glodf; fig:Dpartition.1}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htbp]
%\centering
%%\includegraphics[width=0.45\textwidth] {figures-ee135Notes/ee135Notes-fig-PTDFDpartition0.pdf}
%\caption{Partitions of LODF and PTDF matrices $K$ and $D$.  Submatrices $K_\textup{bn}$ are shaded in light brown, $K_\textup{nn}$ in brown, and $K^\textup{n}$ as indicated; $D_\textup{bn}$, $D_\textup{nn}$ and $D^\textup{n}$ have the same structure.  We will later show that $K_{bn}=0$. $K^{\hat \ell}$ is the $\hat \ell$-th column of $K^\textup{n}$ without the diagonal element $K_{\hat \ell\hat \ell}$.}
%\label{ch:cf; subsec:glodf; fig:Dpartition.1}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The size $m-1$  vector $K^{\hat \ell}$ in \eqref{ch:cf; subsec:lodf; eq:defKlhatl.1b} is the $\hat \ell$-th column of $K^\textup{n}$ without the diagonal entry $K_{\hat \ell\hat \ell}$.
%
Note we implicitly extended the LODF definition to the case in which $\ell=\hat\ell \in E^\textup{n}$ as follows: the diagonal entries of the submatrix $K_\textup{nn}$ are defined as
\[
	K^\textup{n}_{\hat \ell \hat \ell} := \frac{D_{\hat \ell\hat \ell} }{ 1 - D_{\hat \ell \hat \ell} } \qquad \text{ for non-bridge line }\hat \ell \in E^\textup{n}
\]
and represents the change in power flow on line $\hat \ell$ if $\hat \ell = (\hi, \hj)$ is \emph{not} outaged but injections $p_{\hi}$ and $p_{\hj}$ are changed by one unit. 
% \chen{The definition makes sense, but this description does not seem right to me... $D_{\hat \ell \hat \ell}$ is the flow change per unit injections, while $K^n_{\hat \ell \hat \ell}$ is the ratio between flow change with respect to the $(1-flow change)$.} \alec{This is verbatim from Steven's lecture notes, I'd leave it as it is?} \chen{Sure!}
%As noted above $D_{\hat \ell \hat \ell}\in (0, 1)$ if and only if $\hat \ell$ is not a bridge according to Corollary \ref{ch:lm; corollary:PTDF.3}. 

%Then \eqref{ch:lm; eq:LODF.1a} in matrix form is:
%\begin{equation}
%	K^\textup{n} =  D^\textup{n} \left( I - \textup{diag}(D_\textup{nn}) \right)^{-1}
%\label{ch:lm; eq:LODF.1b}
%\end{equation}
% $D_{\hat \ell \hat \ell}=1$ if and only if $\ell$ is a bridge whose outage would separate the network into two islands.
% When $\hat \ell$ is outaged, the quantity $\tilde f_{\hat \ell}$ and hence $K_{\hat \ell \hat \ell}$ are not well defined.
%
To express the LODF \eqref{ch:cf; subsec:lodf; eq:Kllhat.1} in matrix form in terms of $L^\dag$, partition the matrices $B$ and $C$ into two submatrices corresponding to the non-bridge lines and bridge lines (possibly after permutations of rows and columns), i.e., $B =: \ \textup{diag} \left(B_\textup{b}, \, B_\textup{n} \right)$ and $C \ =: \ [  C_\textup{b} \ \  C_\textup{n} ]$. Let $\textup{diag} (D_\textup{nn})$ be the $m_\textup{n}\times m_\textup{n}$ diagonal matrix whose diagonal  entries are $D_{\hat \ell \hat \ell}$ for non-bridge lines $\hat \ell$. 
%\chen{Shall we define $K_{\hat\ell \hat\ell}$? It seems that $K^n_{\hat\ell \hat\ell}\neq -1$ in the following corollary...} \alec{Definition added in the previous paragraph}
\begin{cor}
\label{ch:cf; corollary:LODF.2}
With the submatrices defined above we have $D^\textup{n} \ = \ B  C^T L^\dag  C_\textup{n}$ and
\[
	K^\textup{n} \ = \ D^\textup{n} \left( I - \mathrm{diag}(D_\textup{nn}) \right)^{-1} \ = \ B  C^T  L^\dag  C_\textup{n} \left( I - \mathrm{diag} (B_\textup{n}  C_\textup{n}^T  L^\dag  C_\textup{n} ) \right)^{-1}.
\]
\end{cor}
Given a non-cut set $\calE$ of lines, let $-\calE := E\!\setminus\! \calE$. Consider the submatrix $K_{-\calE\calE} := \big( K_{\ell\hat \ell}, \, \ell\in -\calE, \hat \ell\in \calE \big)$ of $K^\textup{n}$ and the submatrices $D_{-\calE\calE} := \big( D_{\ell\hat \ell}, \, \ell\in -\calE, \hat \ell\in \calE \big)$ and  $D_{\calE\calE} := \big( D_{\hat \ell\hat \ell}, \, \hat \ell\in \calE \big)$ of $D^\textup{n}$. Corollary \ref{ch:cf; corollary:LODF.2} allows us to rewrite the line outage distribution factors in~\eqref{ch:lm; eq:LODF.1a} in matrix form as
\begin{equation}
	K_{-\calE\calE}  =  D_{-\calE\calE} \left( I - \textup{diag} (D_{\calE\calE}) \right)^{-1}.
\label{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}
\end{equation}
Equation~\eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}, despite looking similar to the formula~\eqref{ch:cf; eq:GLODF.1} for the GLODF matrix $K^\calE$ in Theorem~\ref{ch:cf; thm:LODF.3}, is fundamentally different since only the diagonal elements of $D_{\calE\calE}$ are used, while the full matrix $D_{\calE\calE}$ appears in~\eqref{ch:cf; eq:GLODF.1}.

It is important to stress that the LODF submatrix $K_{-\calE\calE}$ is \textit{not} the GLODF matrix $K^\calE$. Indeed the matrix $K_{-\calE\calE}$ is a compact way to write all the LODF factors $K_{\ell \hat \ell}$ corresponding to the \textit{individual} line outages $\hat \ell \in \calE$ and does \emph{not} give the sensitivity of power flows in the post-contingency network to a set $\calE$ of \textit{simultaneous} line outages. For this reason, each column of $K_{-\calE\calE}$ must be interpreted \emph{separately}: column $\hat \ell$ gives the power flow changes on each surviving line $\ell\in -\calE$ due to the outage of a \emph{single} non-bridge line $\hat \ell \in \calE$. Nonetheless, combining~\eqref{ch:cf; eq:GLODF.1} and~\eqref{ch:cf; sec:lodf; eq:K_{-FF}D_{-FF}}, we can show that in the case of a non-cut set $\calE$, the GLODF matrix $K^\calE$ and the LODF submatrix $K_{-\calE\calE}$ are still related as follows:
\begin{equation}
	K^\calE = K_{-\calE\calE} \left( I - \mathrm{diag}(D_{\calE\calE}) \right) \left( I - D_{\calE\calE} \right)^{-1}.
\label{ch:cf; eq:GLODF.1c}
\end{equation}
This expression shows that if $\calE = \{\hat \ell\}$ is a singleton, then the two matrices coincides, but in general $K^\calE \neq K_{-\calE\calE}$. 

\subsection{Islanding and GLODF for cut sets}
\label{sub:cut}

In this subsection we study the impact of cut set outages, extending the results of the previous subsection to the scenario where a set of lines trip simultaneously disconnecting the network into two or more connected components or islands. We first focus on the case of a general cut set outage and then later, in Subsection~\ref{sub:bridge}, specify our results in the case in which the cut set consist of a single line, i.e., the case of a bridge outage.

Consider a subset of lines $\calE \subset E$ that is a cut set for $G=(V,E)$, which means that the surviving network $G^\calE:=(V,E\bs\calE)$ consists of two or more islands $\calI_1,\dots, \calI_k$. A \textit{power balancing rule} needs to be invoked to rebalance power on each island after the contingency. We assume such operations on the islands are decoupled, so that we can study the power flow redistribution in each of them separately. Therefore, for the purpose of presentation, let us focus on one of these islands, say $\calI$. 
%the corresponding subgraph $\calI=(V_\calI,E_\calI)$ consisting of $n_\calI = |V_\calI|$ nodes. 

We can distinguish three types of failed lines and partition $\calE = \calE_\calI \cup \calE_{\partial \calI} \cup \calE_{\calI^c}$ accordingly as follows:
\begin{itemize}
	\item $\calE_\textrm{int} = \calE_\calI:= \set{(i,j)\in \calE ~:~ i\in\calI \text{ and } j\in\calI }$ is the subset of failed \textit{internal lines}, i.e., those both endpoints of which belong to $\calI$;
	\item $\calE_\textrm{tie} = \calE_{\partial \calI}:=\set{(i,j)\in \calE ~:~ i\notin\calI\text{ and }j\in\calI }$ is the subset of failed \textit{tie lines}, i.e., those that have exactly one endpoint in $\calI$; %\chen{Maybe we can fix the direction of tie line: $\calE_\textrm{tie}=\calE_{\partial \calI}:=\set{(i,j)\in \calE ~:~ i\notin\calI\text{ and }j\in\calI }$ so that the following $b_\calI$ is well-defined.} \alec{Possibly yes, but are other sums affected by this change? Check whether it is fine to work everywhere in this subsection with directed edges!} \chen{Checked and changed accordingly};
	\item $\calE_{\calI^c}$ is the subset of failed lines neither endpoints of which belongs to $\calI$.
\end{itemize}
Any outaged line in $\calE_{\calI^c}$ does not have a direct impact on the island $\calI$ and can thus be ignored and thus we can assume without loss of generality that $\calE = \calE_\textup{tie} \cup \calE_\textup{int}$. 

A main difference between a bridge outage and a cut-set outage is that in the former case $\calE = \calE_\textup{tie}$ consists of a single tie line, whereas in the latter case $\calE$ may contain internal lines in $\calE_\textup{int}$ as well. Since $\calI$ is connected, $\calE_\textup{int}$ is a non-cut set. The power flows on surviving lines in $\calI$ are impacted by both internal line outages in $\calE_\textup{int}$ and by tie line outages in $\calE_\textup{tie}$. 
%Let $G_{\calE_\textup{tie}} = ( N_{\calE_\textup{tie}}, E_{\calE_\textup{tie}})$ be a connected graph that models the topology of the \emph{pre-contingency} island, i.e., $E_{\calE_\textup{tie}}$ includes the outaged internal lines in $\calE_\textup{int}$ but not the outaged tie lines in $\calE_{\textup{tie}}$.

Denote by $\pp_I := (p_i, i \in \calI)$ the pre-contingency injections in $\calI$. The power injections $\pp_I$ may not be balanced inside the island, as there could be a non-zero total power imbalance 
\[
	\im := \bm{1}^T \pp_\calI = \sum_{i \in \calI} p_i  = -\sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}.%
\]
If $\im < 0$, then it means that pre-contingecy the island was importing power, while in the opposite case, the island was exporting power. In either case, if $\im \neq 0$, the network operator has to intervene with a \textit{balancing rule} that, by adjusting injections (generators and/or loads) in some of the nodes, ensures that the power balance is restored in $\calI$.

A popular balancing rule, named \emph{proportional control}, is to share the imbalance among a set of participating nodes with a fixed proportion. Specifically a proportional control $\mathbb G_{\a}$ is defined by a nonnegative vector $\a := (\alpha_i, i \in \calI)$ such that $\sum_{i \in \calI}\, \alpha_i = 1$, with the interpretation that, post contingency, each node $i \in \calI$ adjusts its injection by the amount $\Delta p_i := -\alpha_i \im$. The injection adjustments vector is then
\begin{equation}
	\Delta \pp_{\a} := ( \Delta p_i, i \in \calI) = -\im \sum_{i \in \calI} \alpha_i \ee_i,
\label{ch:cf; subsec:bridgeoutage; eq:Galpha.1}
\end{equation}
where $\ee_i$ is the standard unit vector of size $n_\calI$. We refer to each node $i \in \calI$ such that $\alpha_i>0$ as \textit{participating node}. All participating nodes adjust their injections in the same direction, whose sign depends on the sign of $\im$.
The injections are therefore changed from $\pp$ to a post-contingency vector $ \pp + \Delta \pp_\alpha$. The proportional control rebalances the power on $\calI$: the assumption $\sum_{i \in \calI}\, \alpha_i = 1$ guarantees that the post-contingency injections are zero-sum, as
\[
	\bm{1}^T ( \pp + \Delta \pp_\alpha) =\bm{1}^T ( \pp - \im \sum_{i \in \calI} \alpha_i \ee_i ) = \im -\im = 0.
\]

We now derive the impact of the cut set $\calE$ outage on the surviving lines in island $\calI$.
Let $\ff$ be the pre-contingecy power flows on the lines in $\calI$ and further partition $\ff = (\ff_{-\textup{int}}, \ff_\textup{int})$, where $\ff_\textup{int} := (f_\ell, \ell\in \calE_\textup{int})$ denote the pre-contingency power flows on the outaged internal lines, $\ff_{-\textup{int}} := (f_\ell, \ell\in E_\calI \!\setminus\! \calE_\textup{int})$ those on the surviving lines in $\calI$.
Let $B, C, L^\dagger$ denote the susceptance matrix, the incidence matrix and the graph Laplacian pseudo-inverse associated with the island $\calI$. We also partition the matrices $B, C$ according to surviving lines and outaged internal lines as $B =:  \textup{diag} \left(B_{-\textup{int}}, B_\textup{int} \right)$ and $C=:\begin{bmatrix} C_{-\textup{int}}, & C_\textup{int} \end{bmatrix}$.

When multiple lines are tripped from the grid simultaneously disconnecting the network, the aggregate impact in general is different from the aggregate effect of tripping the lines separately. Nonetheless, as the following result shows, the impact from balancing rule turns out to be separable from the rest.

\begin{thm}[GLODF for cut set with proportional control $G_{\a}$]
The net change on the surviving lines of the island $\calI$ due to a cut set outage $\calE=\calE_\textup{tie} \cup \calE_\textup{int}$ is given by
\begin{equation}
\Delta \ff_{-\textup{int}} =  K^{\calE_\textup{int}} \, \ff_{\textup{int}} +  \sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k\, \left( D_{-\textup{int}, k j(\hat \ell)} + K^{\calE_\textup{int}}\, D_{\textup{int}, k j(\hat \ell)} \right),
\label{ch:cf; subsec:bridgeoutage; eq:DeltaP.1}
\end{equation}
where $j(\hat \ell)$ is the endpoint of tie line $\hat \ell$ that lies in $\calI$.
\end{thm}
For a proof, the reader can look at~\cite[Theorem 5]{TPS2} and eq.~(12) therein. The RHS of~\eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} consists of two terms:
\[
\Delta \ff_{-\textup{int}} =  \underbrace{ K^{\calE_\textup{int}} \, \ff_{\textup{int}} }_{ \textup{int. line $\calE_\textup{int}$ outage} }
	\ \ + \ \ 	
	\underbrace{ \sum_{\hat \ell\in \calE_\textrm{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k\, \left( D_{-\textrm{int}, k j(\hat \ell)} + K^{\calE_\textrm{int}}\, D_{\textrm{int}, k j(\hat \ell)} \right)}_{ \text{tie line $\calE_\textrm{tie}$ outage} }.
\]
The first term on the RHS accounts for the impact of the outage of the non-cut set $\calE_\textup{int}$ of internal lines in $\calI$ through the GLODF $K^{\calE_\textup{int}} := B_{-\textup{int}} \, C_{-\textup{int}}^T \, L \, C_{\textup{int}} (I - B_{\textup{int}} \, C_{\textup{int}}^T \, L^\dagger \, C_{\textup{int}})^{-1}$ (cf.~Theorem \ref{ch:cf; thm:LODF.3}). The second term captures the impact of the proportional control $\mathbb G_\alpha$ in response to tie line outages in $\calE_\textup{tie}$, which also accounts for the mimicked power injection change due to the outaged tie lines $\hat \ell \in \calE_\textup{tie}$ at their endpoints $j(\hat \ell)$ in $\calI$. We stress that the impact of the proportional control $\mathbb G_\alpha$ through internal lines in $\calE_\textup{int}$ is scaled by the GLODF $K^{\calE_\textup{int}}$.
%\begin{equation}
%\Delta \pp_\textup{tie}  :=  \sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell} \ee_{j(\hat \ell)}
%\label{ch:cf; subsec:bridgeoutage; eq:P}
%\end{equation}
%We can rewrite~\eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} as
%\begin{subequations}
%\begin{equation}
%\Delta \ff_{-\textup{int}}  =  
%	\underbrace{ K^{\calE_\textup{int}}\, \ff_\textup{int} }_{\textup{int. line $\calE_\textup{int}$ outage}} \ + \ \
%	\underbrace{ \sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k\, \tilde D_{k j(\hat \ell)} }_{\text{tie line $\calE_\textup{tie}$ outage}}
%\label{ch:cf; subsec:bridgeoutage; eq:DeltatildeP.1a}
%\end{equation}
%where each of the vectors $\tilde D_{k j(\hat \ell)}$ is defined as
%\begin{equation}
%\tilde D_{k j(\hat \ell)} := \begin{bmatrix} I_{-\textup{int}}  K^{\calE_\textup{int}} \end{bmatrix} BC^T L^\dagger  \left( \ee_k -  \ee_{j(\hat \ell)} \right)
%\label{ch:cf; subsec:bridgeoutage; eq:DeltatildeP.1c}
%\end{equation}
%and $I_{-\textup{int}}$ is the identity matrix of size $|E_\calI \!\setminus\! \calE_\textup{int}|$.
%\label{ch:cf; subsec:bridgeoutage; eq:DeltatildeP.1}
%\end{subequations}

Note that if there are no tie line outages, i.e., $\calE_\textup{tie} = \emptyset$, then \eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} reduces to Theorem \ref{ch:cf; thm:LODF.3} for a non-cut set outage. 
If there are no internal lines $\calE_\textup{int} = \emptyset$, the first term of \eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} is zero and the second term simplifies, so that 
%and $\tilde D_{k j(\hat \ell)} = D_{-\textup{int}, k j(\hat \ell)}$ and, hence,
\[
\Delta \ff_{-\textup{int}}  = \sum_{\hat \ell\in \calE_\textup{tie}} f_{\hat \ell}  \sum_{k: \alpha_k>0} \alpha_k\, D_{-\textup{int}, k j(\hat \ell)}.
\]




\subsubsection{Bridge outage}
\label{sub:bridge}
Consider now the case of a cut set outage, in which the $\calE$ consist of a single line. This means that $\calE_\textup{int} = \emptyset$, $\calE_\textup{tie}=\{\hat \ell\}$, and $\hat \ell = (\hat i, \hat j)$ is a bridge. After the outage of line $\ell$, the power network gets disconnected into two islands, one containing node $\hat i$ and one containing node $\hat j$, which we denote by $\calI_{\hat i}$ and $\calI_{\hat j}$ respectively. 

If the pre-contingency power flow $f_{\hat \ell} = 0$ on the outaged line $\hat \ell$, then the operations of these islands, as modeled by the DC power flow equations, are decoupled pre-contingency and therefore remain unchanged post-contingency.
We henceforth consider only the case where $f_{\hat \ell}\neq 0$, which means that there is a nonzero power imbalance over each of the two islands post contingency. For example, if $f_{\hat \ell}>0$, i.e., the power flows from island $\calI_{\hat i}$ to island $\calI_{\hat j}$ pre contingency, then there is a power surplus of size $f_{\hat \ell}$ on $\calI_{\hat i}$ and a shortage of size $f_{\hat \ell}$ on $\calI_{\hat j}$ post contingency.
Like before, since the two islands operate independently post contingency, each according to DC power flow equations, we can focus only on one island, say $\calI_{\hat j}$. Let $\Delta \ff := (\Delta f_\ell, \ell\in E_{\calI_{\hat j}})$ be the vector of net power flows changes on all lines in island $\calI_{\hat j}$. Then, \eqref{ch:cf; subsec:bridgeoutage; eq:DeltaP.1} simplifies to
\[
	\Delta \ff = f_{\hat \ell}  \sum_{k\in \calI_{\hat j}} \alpha_k\, \Big( D_{E_{\calI_{\hat j}}, k \hat j} \Big).
	% f_{\hat \ell} \,  \sum_{k\in \calI_{\hat j}} \alpha_k \,  BC^T L^\dagger  \left( \ee_k - \ee_{\hat j} \right).
\]
More explicitly, for any line $\ell = (i,j) \in E_{\calI_{\hat j}}$ we have
\[
\frac{\Delta f_\ell} {f_{\hat \ell}}
	% \ = \ \sum_{k \in \calI_{\hat j}}\alpha_k \, b_\ell C_\ell^T L^\dagger \left( \ee_k - \ee_{\hat j} \right) 
	=  \sum_{k: \alpha_k>0} \alpha_k \, D_{\ell, k\hat j}
	=  \sum_{k\in \calI_{\hat j}} \alpha_k \, b_\ell \left( L^\dagger_{ik} + L^\dagger_{j\hat j} - L^\dagger_{i\hat j} - L^\dagger_{jk} \right),
\]
where the last equality follows from Theorem \ref{ch:lm; prop:PTDF.1}. Therefore the power flow change on line $\ell$ is the superposition of two factors: (i) injecting $\alpha_k f_{\hat \ell}$ at participating nodes $k\in \calI_{\hat j}$ and (ii) withdrawing $f_{\hat \ell}$ at node $\hat j$.
Using the last identity, we can thus extend the definition of LODF $K_{\ell\hat \ell}$ to allow for outages of any bridge $\hat \ell = (\hat i, \hat j)$ with nonzero flow $f_{\hat \ell}\neq 0$ under the proportional control $\mathbb G_{\a}$ as follows
\begin{align}
K_{\ell\hat \ell} :=  \frac{ \Delta f_\ell } { f_{\hat \ell} } = \sum_{k ~:~ \alpha_k>0}  \alpha_k\, D_{\ell, k\hat j},\qquad \text{for all } \ell\in E_{\calI_{\hat j}}.
\label{ch:cf; subsec:bridgeoutage; eq:Klhatl.1}
\end{align}

%\alec{Compared with \eqref{ch:cf; subsec:bridgeoutage; eq:Klhatl.1}, this means that, when no internal lines are outaged, the impact of simultaneous outage of a set $\calE_\textup{tie}$ of tie lines is simply the sum of the impacts of single line $\hat \ell$ outages \emph{as if} $\hat \ell$ was a bridge for $\calI$ (which it may not be).}

==> arxiv submission/spectralrepresentation.tex <==
\section{A spectral representation of power systems}
\label{sec:spectral}
A power transmission network can be described as a graph $G=(V,E)$, where $V=\set{1,\ldots, n}$ is the set of vertices (modeling \textit{buses}) and $E\subset V \times V$ is the set of edges (modeling \textit{transmission lines}). Denote by $n=|V|$ the number of vertices and by $m=|E|$ the number of edges of the network $G$. 
In this section we describe power network model that we consider throughout the paper and highlight an intimate connection between spectral graph theory and power flow physics. We first review in Subsection~\ref{sub:basic} some key notions from graph theory and some classical network decompositions that are crucial for our analysis. Then, in Subsection~\ref{sub:dcmodel}, we introduce the power flow model that we will focus on in this paper in spectral terms and present some immediate results that follow from this representation.

%In particular, using the relation between power injections and power flows in terms of the pseudo-inverse of the graph Laplacian, we show that the eigenvectors of the same matrix can also be used to identify the islands of the power network (i.e., its connected components), and that the power balance condition for each island has an immediate interpretation in spectral terms. 
%Furthermore, one of the two methods that we propose later in Section~\ref{sec:optimization} to mitigate failure propagation in a power network by adaptively changing its topology is also fundamentally spectral in nature.
%We assume $G$ to be simple. \alec{Is this assumption realistic for power systems? Does it affect our proposed heuristic?}

\subsection{Network decompositions and substructures}
\label{sub:basic}
%We start by giving some basic graph theory definitions and describing the power network model in spectral terms.
Due to power flow physics, the topology of a power transmission network plays a central role in the way power flows on its lines. In fact, the power flows are intrinsically determined by the network physical structure via Kirchhoff's laws once that the power injections are fixed. This also means that the power flow redistribution after a contingency and possible cascading outages are intimately related to the network structure. It comes as no surprise that to study the robustness of a power network makes uses of advance graph theory notions and algorithms. We now briefly review some useful network decompositions and substructures that will play a crucial role in our analysis in the next sections. 

In this subsection we look at a transmission power network in purely topological terms as an undirected and unweighted graph $G$, thus temporarily ignoring the physical and electrical properties of its transmission lines. The $k$-\textit{partition} of a network $G=(V,E)$ is a finite collection $\calP=\set{\calV_1,\calV_2,\cdots, \calV_k}$ of nonempty and disjoint subsets of $V$ such that $\bigcup_{i=1}^k \calV_i=V$. 
%\ale{KEEP OR REMOVE?\\Without loss of generality, we assume that every partition $\calP$ is in \textit{standard form}, i.e., that each one of its clusters induces a connected subgraph of $G$ (if this was not the case, we can always split the clusters in its connected components and add all them separately to $\calP$). In the rest of the paper, we will tacitly assume that every partition is in standard form.}
Denote by $\Pi_k(G)$ the collection of $k$-partitions of $G$ and by $\Pi(G) := \bigcup_{i=1}^{|V|} \Pi_i(G)$ the collection of all its partitions.
%$$\Pi_{\leq k}(G) = \bigcup_{i=1}^k \Pi_i(G) \quad \text{ and } \quad \Pi(G) = \Pi_{\leq |V|}(G) =\bigcup_{i=1}^{|V|} \Pi_i(G).$$
Given a partition $\calP$, each edge of the network $G$ is either a \textit{cross edge} if its two endpoints belong to different clusters of $\calP$ and \textit{internal edge} otherwise. We denote the collections of cross edges and internal edges as $E_c(\calP)$ and $E_i(\calP)$, respectively.
There is a natural partial order $\succeq$ on the collection $\Pi(G)$ of partitions, defined as follows: given two partitions $\calP^1=\set{\calV_1^1,\calV_2^1,\cdots,\calV_{k_1}^1}$ and $\calP^2=\set{\calV_1^2,\calV_2^2,\cdots,\calV_{k_2}^2}$, we say that $\calP^1$ is \emph{finer} than $\calP^2$, denoted as $\calP^1\succeq \calP^2$, if each subset in $\calP^1$ is contained in some subset in $\calP^2$. More precisely, $\calP^1\succeq \calP^2$ if for every $i=1,2,\ldots, k_1$, there exists some $j(i)\in \set{1,2,\ldots, k_2}$ such that $\calV_i^1\subseteq \calV_{j(i)}^2$. 

Each partition $\calP$ induces a \textit{quotient graph} $G/\calP$, which is the undirected graph whose vertices are the clusters in $\calP$ and two distinct clusters $\calV_i, \calV_j \in \calP$, are adjacent if and only if there exists at least one cross edge in the original graph $G$ whose endpoints belong one to $\calV_i$ and one to $\calV_j$. 
%In other words, the edge set of $G/\calP$ is $\{(\calV_i,\calV_j) : \exists \, v \in \calV_i, \, v' \in \calV_j \text{ such that } (v,v') \in E\}.$
A slight variation of the quotient graph is the \textit{reduced graph} $G_\calP$, which is defined as the (multi)graph whose vertices are still the clusters in $\calP$, but in which we draw an edge between two distinct clusters for every cross edge between them. The reduced graph $G_\calP$ can thus have multiple (parallel) edges, and coincides with the quotient graph only when it is simple.

It is well known that any equivalence relation on the set of vertices of the network $G$ induces a partition. We now briefly review three canonical decompositions of an undirected graph that have been introduced in the graph-theory literature (see, e.g.,~\cite{Harary1971,Westbrook1992}) using specific equivalence relations. 

First of all, consider the partition $\calP_\mathrm{path}=\{\calI_1,\dots, \calI_k\}$ in which two vertices are in the same subset if and only if there is a path connecting them. In this case $E_c(\calP_\mathrm{path})=\emptyset$ by definition, the quotient and reduce graphs trivially coincides and and have no edges. 
%Let $G_i$ be the subgraph induced by $\calI_i$, for $i=1,\dots,k$. that is the graph with vertex set $\calI_i$ and edge set $E_i \subseteq E$ consisting of all the edges incident to vertices in $\calI_i$. 
The subgraphs $G_1,\dots,G_k$ induced by $\calP_\mathrm{path}$ are the \textit{connected components} of $G$, also referred to as \textit{islands} in the power systems literature. A graph is \textit{connected} if it consists of a single connected component, i.e.~$|\calP_\mathrm{path}|=1$. In general, a power network $G$ may not be connected at all times, either due to operational choice or as a result of severe contingencies).

The notion of graph connectedness allows to introduce two more notions that will be crucial for our network analysis. A subset $\calE \subset E$ is a \textit{cut set} of $G$ if the deletion of all the edges in $\calE$ disconnects $G$. If the cut set consists of a single edge, we refer to it as \textit{bridge} or \textit{cut edge}. A \textit{cut vertex} of $G$ is any vertex whose removal (together with its incident edges) increases the number of its connected components.

A second network decomposition can be obtained by looking at the network circuits. Recall that a circuit is a path from a vertex to itself with no repeated edges. We consider the partition $\calP_\mathrm{circuit}(G)$ such that two vertices are in the same class if and only if there is a circuit in $G$ containing both of them.
%\chen{Should we require simple cycles? Otherwise it will be the same as connected components. Am I missing anything?} \alec{There is no mistake. The dycothomy is: cycles (possibly with repeated vertices) $\longleftrightarrow$ bridge-blocks, simple cycles $\longleftrightarrow$ blocks}
%For every cluster in $\calP_\mathrm{cycle}$, we consider the corresponding subgraphs with vertex set $R_i$ and all the edges that have both endpoints in $R_i$. 
The subgraphs induced by the subset of nodes in each of the equivalence classes of $\calP_\mathrm{circuit}(G)$ are precisely the connected components of the graph obtained from $G$ by deleting all the bridges and, for this reason, they are called \textit{bridge-connected components} or \textit{bridge-blocks}. We will refer to the partition $\calP_\mathrm{circuit}(G)$ as \textit{bridge-block decomposition} of $G$ and denote it by $\mathcal{B}\mathcal{B}(G)$.

The next lemma summarizes the intuitive fact that the bridge-block decomposition of a graph becomes finer if some of its edges are removed. This result is the cornerstone of the strategy to improve the network reliability that is presented in Section~\ref{sec:optimization}.
\begin{lem}[Removing edges makes bridge-block decomposition finer]\label{lem:finer}
For any graph $G=(V,E)$ and subset of edges $\calE \subset E$, the bridge-block decomposition of the graph $G^\calE:=(V,E\setminus \calE)$ obtained from $G$ by removing the edges in $\calE$ is always finer than that of $G$, i.e.,
$$\calBB(G^\calE) \succeq  \calBB(G).$$
\end{lem}
\begin{proof}
Consider the partition $\calBB(G)=\calP_{\mathrm{circuit}}(G)$ and recall that two vertices belong to the same equivalence class (bridge-block) if and only if there exists a circuit that contains both of of them. By removing a subset of edges $\calE$ from $G$, each of the equivalence classes either remains unchanged or gets partitioned in smaller equivalence classes. This readily implies that for every new bridge-block $B \in \calBB(G^\calE)$ obtained after the edge removal there exists a bridge-block $B'$ of the original network, i.e., $B' \in \calBB(G)$, such that $B \subseteq B'$. 
\end{proof}

A third network decomposition can be obtained by considering the network cycles, which are the circuits in which the only repeated vertices are the first and last ones. More specifically, we consider the equivalence relation for edges of being contained in a cycle and denote by $\{E_1,E_2,\dots,E_k\}$ to be the resulting partition of $E$. Let $R_i=(V_i,E_i)$ be the corresponding subgraph of $G$, consisting of the edges in $E_i$ and the vertices $V_i$ that are the endpoints of these edges. We refer to each subgraph $R_i$ either as \textit{block} and to $\mathcal{B}(G)=\{V_1,\dots,V_k\}$ as the \textit{block decomposition} of $G$. Every block is a maximal biconnected (or 2-connected) subgraph, since the removal of any of its vertices does not disconnect it. A vertex could appear in more than one block and, since its removal disconnects $G$, this is an equivalent characterization of cut vertices. The block decomposition $\mathcal{B}(G)$ thus is not a partition of the vertex set $V$, but nonetheless for any pair of vertices there is either no block or exactly one block containing them both. We distinguish two types of blocks, \textit{trivial blocks} and \textit{nontrivial blocks}, depending on whether they consist of a single edge or not. A trivial block consists of an edge that is not contained in any cycle; such an edge must then be a bridge since its removal disconnects the graph, cf.~\cite[Chapter 3]{Harary1971}. Two nontrivial blocks either share a cut vertex or are connected by a bridge, i.e., a trivial block. %\chen{Shall we add some reference for the block decomposition?} \alec{\cite{Westbrook1992}, which is already cited above is one, but maybe we should repeat it}

We remark that a statement similar to Lemma~\ref{lem:finer} holds also for the edge partition $\{E_1,E_2,\dots,E_k\}$ corresponding to the block decomposition of a graph $G$ and for the block decomposition $\calB(G)$ itself. However, for the strategy to improve network reliability that we present in Section~\ref{sec:optimization}, it turns out that $\calB(G)$ is less convenient to work with than the bridge-block decomposition $\calBB(G)$ since the block decomposition $\calB(G)$ is not a proper vertex partition (recall that the cut vertices always appear in two or more blocks).

%A third decomposition can be obtained by looking at how cycles partition vertices. More specifically, we partition the vertex set $V$ into equivalence classes $V_1,\dots,V_j$ such that two vertices are in the same class if and only if there is a cycle (not necessarily simple) in $G$ containing both of them. \chen{Should we require simple cycles? Otherwise it will be the same as connected components. Am I missing anything?} \alec{There is no mistake. The dycothomy is: cycles (possibly with repeated vertices) $\longleftrightarrow$ bridge-blocks, simple cycles $\longleftrightarrow$ blocks} For every class $V_i$, consider the corresponding subgraphs with vertex set $R_i$ and all the edges that have both endpoints in $R_i$. The subgraphs $R_1,\dots,R_j$ are precisely the connected components of the graph obtained deleting all the bridges and, for this reason, they are called \textit{bridge-connected components} or \textit{bridge-blocks}. \chen{Same here, we may add some references.}

Both the block and bridge-block decompositions of a graph $G$ are unique. We can informally say that the block decomposition is finer than the bridge-block decomposition, since each bridge corresponds to a trivial block, while every bridge-block consists of several non-trivial blocks connected by cut vertices. Such a nested structure of the block and bridge-block decompositions is illustrated for a small graph in Fig.~\ref{fig:networkdec}. Another visualization of these network decompositions for an actual power network can be found later in Section~\ref{sec:localization}, see Fig.~\ref{fig:influencegraph_pre}.

A graph naturally decomposes into a tree/forest of blocks called its \textit{block-cut tree/forest}, depending on whether the original graph is connected or not. More specifically, in such a block-cut tree/forest there is a vertex for each block and for each cut vertex, and there is an edge between any block and cut vertex that belongs to that block. Similarly, also the bridge-blocks and bridges of $G$ have a natural tree/forest structure, called \textit{bridge-block tree/forest}, depending if $G$ is connected or not. Such a tree/forest is the graph with a vertex for each bridge-block and with an edge for every bridge. We refer the reader to~\cite[Chapter 3]{Harary1971} for further details.

\begin{figure}[!h]
\centering
% \subfloat[]{\includegraphics[width=.25\textwidth]{cut_demo_original_graph.png}
% }\hspace{3cm}
% \subfloat[]{\includegraphics[width=.28\textwidth]{cut_demo_decomposed.png}
\subfloat[]{\includegraphics[width=.26\textwidth]{original_graph_col.png}}
\hspace{1cm}
\subfloat[]{\includegraphics[width=.26\textwidth]{bridgeblock_decomposition_col.png}}
\hspace{1cm}
\subfloat[]{\includegraphics[width=.3\textwidth]{block_decomposition_col.png}}
\caption{An undirected graph $G$ in (a) with its bridge-block decomposition in (b) and with its block decomposition in (c). Edges $(2, 6)$ and $(3, 7)$ are bridges. Vertices $2, 3, 7$ are the cut vertices of $G$ and appear in multiple blocks.}
\label{fig:networkdec}
\end{figure}
\FloatBarrier


The problems of finding the blocks and bridge-blocks of a given graph are well understood: sequential algorithms that run in time $O(n + m)$ were given in~\cite{Hopcroft1973,Tarjan1972} and logarithmic-time parallel algorithms are given in~\cite{Awerbuch1987,Tarjan1985}.
%Given the tree partition of a graph, both the endpoints of every bridge are cut vertices, which readily implies that the block decomposition is finer than the tree partition (more specifically, the partition of the edge set $E$ induced by it). The block decomposition of a graph always exists and can be found in linear time as proved by~\cite{Tarjan1985}.
Later in Section~\ref{sub:PTDF} we also give a precise spectral characterization for bridges (cf. Corollary \ref{ch:lm; corollary:PTDF.3}).

Another complementary powerful tool to study the topology of power networks is using its spanning trees, which will play a crucial role in the study of distribution factors in Section~\ref{sec:distfactor}. A spanning tree of $G$ is a subgraph that is a tree with a minimum possible number of edges that includes all of the vertices of $G$. Let $T_\calE$ be the collection of all spanning trees of $G$ consisting only of edges in $\calE\subseteq E$ and $T = T_E$ the set of all spanning trees of $G$. We further denote by $T\!\setminus\! \calE := T_{E\!\setminus\! \calE}$ the collection of all spanning trees of $G$ consisting of edges in $E\!\setminus\! \calE$. For any pair of disjoint subsets of vertices $V_1, V_2\subset V$, we denote by $T(V_1, V_2)$ the collection of spanning forests of $G$ consisting of exactly two trees necessarily disjoint, one containing the vertices in $V_1$ and the other one containing those in $V_2$. Note that $T_\calE$ can be empty if the subset $\calE$ is too small and that $T(V_1, V_2)$ is empty by definition whenever $V_1$ and $V_2$ are not disjoint.

\subsection{Power flow model and its spectral representation}
\label{sub:dcmodel}
In this subsection, we present the classical DC power flow model and a few key spectral properties that are intertwined with the power flow dynamics.

In order to accurately model a power system, it is important to capture the physical properties of its transmission lines. When necessary, we thus look at $G=(V,E)$ as weighted graph, in which each edge $\ell=(i,j) \in E$ has a weight $b_\ell=b_{ij}=b_{ji}>0$ that models the \textit{susceptance} of the corresponding line. To stress the difference with its unweighted counterpart, we will refer to the weighted graph $G=(V,E,\bm{b})$ as \textit{power network} and to its edges as lines.

It is crucial for our analysis to capture the ``electrical properties'' of specific parts or components of the power network, in particular of its spanning trees. For this reason we introduce a nonnegative weight for any subset $\calE \subseteq E$ of lines by defining a function $\beta : 2^E\rightarrow \mathbb R_+$ as follows: 
\[
	\beta(\calE) := \prod_{\ell\in \calE}\, b_\ell, \qquad \calE \subseteq E.
\]
In other words, $\beta(\calE)$ is the product of the susceptances of all the lines in the subset $\calE$. For consistency we set $\beta(\calE) = 0$ if $\calE = \emptyset$ and $E\neq\emptyset$, but $\beta(\calE) = 1$ when the power network $G$ consists of a single vertex, i.e., $\calE = E = \emptyset$.

Let $B:=\mathrm{diag}(b_1,\dots,b_m) \in \R^{m \times m}$ be the diagonal matrix with the line susceptances (i.e., the edge weights) $b_1,\dots,b_m$ as entries, assuming a fixed order has been chosen for the edge set $E$. Aiming to describe line flows, it is necessary to introduce an (arbitrary) orientation for the edges, which is captured by the vertex-edge incidence matrix $C \in \{-1,0,+1\}^{n\times m}$ defined as
$$
C_{i \ell}=\begin{cases}
  1 & \text{if vertex }i\text{ is the source of }\ell,\\
  -1 & \text{if vertex }i\text{ is the target of }\ell,\\
  0 &\text{otherwise.}
\end{cases}
$$
The spectral representation of power systems relies on the \textit{weighted Laplacian matrix} of the power network $G$, that is the symmetric $n \times n$ matrix $L$ defined as $L:=C B C^T$ or, equivalently in terms of the susceptances, as
\begin{equation}
\label{eq:Laplaciandef}
    L_{i,j} :=
    \begin{cases}
    		\sum_{k \neq i} b_{i k} 		& \text{ if } i=j,\\
		- b_{ij}  							& \text{ if } i \neq j.
	\end{cases}
\end{equation}
Denote by $\l_1, \l_2 , \dots, \l_{n}$ its eigenvalues and by $\bm{v}_1,\bm{v}_2,\dots,\bm{v}_n$ the corresponding eigenvectors, which we take to be of unit norm and pairwise orthogonal. The next proposition summarizes some crucial properties of the weighted Laplacian matrix $L$ and its \textit{Moore-Penrose pseudo-inverse} $L^\dag$. The proof can be found in the appendix and we refer the reader to~\cite{RanjanZhangBoley2014,VanMieghem2011} for further spectral properties of graphs.

\begin{prop}[Laplacian matrix $L$ and its pseudo-inverse]
\label{ch:lm; eq:Laplacian-properties}
The following properties hold for the weighted Laplacian matrix of a power network $G = (V, E, \bm{b})$:
\begin{itemize}
\item[(i)] For every $\bm{x} \in\R^n$ we have $\bm{x} ^T L \bm{x}  = \sum_{(i,j)\in E}\, b_{ij} (x_i - x_j)^2 \geq 0$.
\item[(ii)] $L$ is a symmetric positive semidefinite matrix and, hence, has a real non-negative spectrum, i.e.,~$0 \leq \l_1 \leq \l_2 \leq \dots \leq \l_{n}$.
\item[(iii)] All the rows (and columns) of $L$ sum to zero and thus the matrix $L$ is singular.
\item[(iv)] The matrix $L$ has rank $n-k$, where $k\geq 1$ is the number of connected components $\calI_1,\dots, \calI_k$ of $G$. The eigenvalue $0$ has multiplicity $k$ and $\mathrm{ker}(L)=\mathrm{ker}(L^\dag)=\mathrm{span}(\bm{1}_{\calI_1},\dots,\bm{1}_{\calI_k})$, where $\bm{1}_{\calI_j} \in \{0,1\}^n$ is the vector which is $1$ on $\calI_j$ and $0$ elsewhere. Furthermore, the pseudo-inverse of $L$ can be calculated as
	\[
	    L^\dag = \sum_{j=k+1}^n \frac{1}{\lambda_j} \bm{v}_j \bm{v}_j^T = \left( L + \sum_{j=1}^k \frac{1}{|\calI_j|} \bmo_{\calI_j} \bmo_{\calI_j}^T \right)^{-1}  - \sum_{j=1}^k \frac{1}{|\calI_j|} \bmo_{\calI_j} \bmo_{\calI_j}^T.   
	\]
In particular, in the special case in which $G$ is connected, i.e., $k=1$, $\mathrm{ker}(L)=\mathrm{ker}(L^\dag) = \mathrm{span}(\bmo)$, where $\bm{1} \in \R^n$ is the vector with all unit entries and
	\[
		L^\dag = \sum_{j=2}^{n} \frac{1}{\l_j} \, \bm{v}_j \bm{v}_j^T = \left( L + \frac{1}{n} \bmo \bmo^T \right)^{-1} \ - \ \frac{1}{n} \bmo \bmo^T.
	\]
\item[(v)] $L^\dag$ is a real, symmetric, positive semi-definite matrix with zero row (and hence column) sums and its nonzero eigenvalues are $0 < \l_n^{-1} \leq \dots \leq \l_{k+1}^{-1}$. 
%and $\mathrm{ker}(L)=\mathrm{ker}(L^\dag)$.
%We have $LL^\dag  = L^\dag L = I  - \frac{1}{n} \bmo \bmo^T$, and, hence, for all $\bm{x}\in\mathbb R^{n}$ with $\bmo^T \bm{x} = 0$, we have $L^\dag L \bm{x} = \bm{x} = L L^\dag \bm{x}$.
\end{itemize}
\end{prop}

Denote by $\pp \in \R^{n}$ the vector of power injections, where the entry $p_i$ models the power generated (if $p_i>0$) or consumed (if $p_i<0$) at the bus corresponding to vertex $i$. We say that a power injection vector $\pp \in \R^n$ is \textit{balanced} if $\pp \in \mathrm{im}(L)$. Since $ \mathrm{im}(L^\dag) = \mathrm{ker}(L^\dag)^\bot=\mathrm{span}(\bm{1}_{\calI_1},\dots,\bm{1}_{\calI_k})^\bot$, a power injection vector $\pp$ is balanced if and only if the net power injection is equal to zero in every island $\calI_j$ of the network, i.e., $\sum_{i \in \calI_j} p_i = 0$.
%If $G$ is connected, the power injection vector is balanced if $\mathbf{1}^T p=0$. 

Transmission power systems are operated using alternating current (AC), but the equations describing the underlying power flow physics are non-linear leading to many computational challenges in solving them~\cite{Wood2013}. Therefore, linearization techniques are often used to approximate the power flow equations. We now introduce the so-called \textit{DC power flow model}, which is a first-order approximation of the AC equations that is commonly used to model high-voltage transmission system~\cite{Wood2013,Stott2009,Dorfler2013b}.

Given an (oriented) edge $\ell=(i,j) \in E$, we denote interchangeably as $f_\ell$ or $f_{ij}$ the power flow on that line. We set $f_{ji}=-f_{ij}$, with the convention that a power flow is negative if the power flows in the opposite direction with respect to the edge orientation. The so-called \textit{DC power flow model} is the system of equations
\begin{subequations}\label{eq:dc_model}
\begin{align}
& \pp = C \ff, \label{eq:conservation}\\
& \ff = BC^T \bt, \label{eq:kirchhoff}
\end{align}
\end{subequations}
%\begin{align}
%& p_j = \sum_{i \in N(j)} f_{ij} &\forall \, j \in V,\\
%&f_{ij} = \b_{ij} (\theta_i - \theta_j ) & \forall \, (i,j) \in E,
%\end{align}
%where $N(i) \subseteq V$ is the set of neighbors vertices of $i$ and $\theta_i$ is the \textit{phase angle} at node $i$
where $\bt \in \R^n$ is the vector of \textit{phase angles} at the network vertices and $\ff\in \R^m$ is the vector of line power flows. Equation~\eqref{eq:conservation} captures the flow-conservation constraint, while equation~\eqref{eq:kirchhoff} describes Kirchhoff's laws.
The DC model \eqref{eq:dc_model} has a unique solution $\ff$ for each balanced injection vector $\pp$. Indeed, from~\eqref{eq:dc_model} we can deduce that $\pp=CBC^T\bt = L \bt$, and, ultimately, obtain the following spectral representation for the power flows
\begin{equation}
\label{eq:flowsdc_model}
	\ff =BC^T L^\dag \pp.
\end{equation}
The power flows are thus uniquely determined by the injections and physical properties of the network. 
%The phase angle solution $\theta$, however, is not unique, since it is defined modulo constant shifts in each of the islands. In case of a connected power network, the issue is typically circumvented by setting the phase angle to $0$ in the so-called \textit{slack node}.
%\begin{figure}
%\centering
%\includegraphics[width=.275\textwidth]{spanning_forest.png}
%\caption{An example element in $\calT(\calV_1,\calV_2)$, where circles correspond to elements in $\calV_1$ and squares correspond to elements in $\calV_2$. The two trees containing $\calV_1$ and $\calV_2$ are highlighted as solid lines.}\label{fig:spanning_forest}
%\end{figure}
%\subsection{Line removal and consequent power redistribution}
In view of~\eqref{eq:flowsdc_model}, it is clear that the network operator does not directly control the power routing, which can be only indirectly changed by modifying the power injections or the network topology. This peculiar feature is one of the reasons why it is challenging to study and improve the reliability of power systems and their robustness against failures.

The interactions between components in a power network depend, not only on its topology, but also on the physical properties of its components and the way they are coupled by power flow physics. Such an ``electrical structure'' can be effectively unveiled and studied using spectral methods, more specifically looking at the so-called \textit{effective resistance}, which is formally defined as follows. The effective resistance $R_{i,j}$ between a pair of vertices $i$ and $j$ of the network $G$ is the non-negative quantity
\begin{equation}
\label{eq:effr}
	R_{ij} := (\mathbf{e}_i - \mathbf{e}_j)^T L^\dag (\mathbf{e}_i - \mathbf{e}_j) = L^\dag_{ii} + L^\dag_{jj} - 2 L^\dag_{ij},
\end{equation}
where $\mathbf{e}_i$ denotes the vector with a $1$ in the $i$-th coordinate and $0$'s elsewhere. $R_{ij}$ quantifies how ``close'' vertices $i$ and $j$ are in the power network $G$ and takes small value in the presence of many paths with high susceptances between them. The effective resistance is a proper distance on $V\times V$ and for this reason it is often referred to as \textit{resistance distance}~\cite{Klein1993}. 
%Any network has thus an equivalent description as a complete graph with the effective resistances as edge weights. 
The \textit{total effective resistance} of a graph $G$ is defined as $\rt(G)=\frac{1}{2} \sum_{i,j=1}^n R_{ij}$ and it is intimately related to the spectrum of $G$ by the following identity proved by~\cite{Klein1993}
\[
    \rt(G) = n \cdot \tr(L^\dag) = n \cdot \sum_{j=2}^n \frac{1}{\lambda_j}.
\]
The same quantity is also known as \textit{Kirchhoff index} in the special case when all the edges of the network $G$ have unit weights, i.e., $b_\ell=1$, $\ell=1,\dots,m$. The total effective resistance is a key quantity that measures how well connected the network is and for this reason has been extensively studied and rediscovered in various contexts, such as complex network analysis~\cite{Ellens2011} and probability theory~\cite{Doyle2000}.
The notion of effective resistances have been first introduced in the context of power networks analysis by~\cite{Cotilla-Sanchez2012} and~\cite{Cotilla2013} and since then have been extensively used to study their robustness, see e.g.,~\cite{Cetinay2018,Dorfler2018,Koc2014,Wang2014,Wang2015}, as well as to devise algorithm to improve their reliability, see e.g.~\cite{Ghosh2008,Johnson2010,Zocca2017}.

%In the case of power systems, $\rt(G)$ has been shown by~\cite{Ghosh2008} to be proportional to the average power dissipated in a resistive network and by~\cite{JohnsonChertkov2010} to be good approximation for \textit{total power loss} in AC power grids. Precisely for this reason, a generalized notion of total effective resistance has been proposed by~\cite{Zocca2017} to optimize participation factors of controllable loads. \cite{Lai2013,Guo2017} proved that $\rt(G)$ is monotone increasing along a cascade failure (as long as the network remains connected). 

==> modeldescription.tex <==
\section{Power network model description}

We describe a power transmission network as a directed graph $G=(V,E)$, where $V=\set{1,\ldots, n}$ is the set of nodes (modeling \textit{buses}) and $E\subset V \times V$ is the set of edges (modeling \textit{transmission lines}). Denote by $n=|V|$ the number of nodes and by $m=|E|$ the number of edges of the network $G$. 

We assume $G$ to be connected and simple. Each edge $e=(i,j) \in E$ has a weight $\b_e=\b_{ij}$, which models the \textit{susceptance} of the corresponding line. Denote by $B$ the $m \times m$ diagonal matrix with entries $\b_1,\dots,\b_m$, where an arbitrary but fixed order has been chosen for the edge set $E$. The vertex-edge incidence matrix of $G$ is the $n\times m$ matrix $C$ defined as
$$
C_{ie}=\begin{cases}
  1 & \text{if vertex }i\text{ is the source of }e,\\
  -1 & \text{if vertex }i\text{ is the target of }e,\\
  0 &\text{otherwise.}
\end{cases}
$$
The \textit{weighted Laplacian matrix} of the graph $G$ is the symmetric $n \times n$ matrix $L$ defined as $L=C B C^T$ or equivalently as
\[
    L_{i,j} :=
    \begin{cases}
    		\sum_{k \neq i} \b_{i k} 		& \text{ if } i=j,\\
		- \b_{ij}  							& \text{ if } i \neq j.
	\end{cases}
\]
Denote by $\l_1, \l_2 , \dots, \l_{n}$ its eigenvalues and by $v_1,v_2,\dots,v_n$ the corresponding eigenvectors, which we can take to be pairwise orthogonal. It is well-known that $L$ is a real symmetric positive semi-definite matrix, which means that it has a real non-negative spectrum, i.e.,~$0 \leq \l_1 \leq \dots \leq \l_{n}$. All the rows of $L$ sum up to zero and thus the matrix $L$ is singular. 

If $G$ is connected, the eigenvalue $\l_1=0$ has multiplicity one and the corresponding eigenvector $v_1$ is the vector with all unit entries, which we denote by $\bm{1} \in \R^n$. In this case, using the eigenspace structure of $L$, the \textit{Moore-Penrose pseudoinverse} $L^+$ can be calculated as
\[
	L^+ :=\left  (L+ \frac{\bm{1}\bm{1}^T}{n}\right )^{-1} -\frac{\bm{1}\bm{1}^T}{n}.
\]
The matrix $L^+$ is also real, symmetric, and positive semi-definite and its spectrum is $0 < \l_n^{-1} \leq \dots \leq \l_2^{-1}$. For further spectral properties of graphs, we refer the reader to~\cite{RanjanZhangBoley2014,VanMieghem2011}.

In general, a power network $G$ may not be connected graph at all times (either by operational choice or in response to severe contingencies). In this case, in the power system literature the connected components $G_1,\dots, G_k$ of $G$ are usually referred to as \textit{islands}.

Denote by $p \in \R^{n}$ the vector of power injections, where the entry $p_i$ models the power generated (if $p_i>0$) or consumed (if $p_i<0$) at node $i$. We say that a power injection vector $p \in \R^n$ is \textit{balanced} if in every island of the power network, the net power injection is equal to zero, i.e., $\sum_{i \in G_j} p_i = 0$, for $i=1\dots,k$. %If $G$ is connected, the power injection vector is balanced if $\mathbf{1}^T p=0$. 

Given an oriented edge $e=(i,j)$, we denote the power flow on that line interchangeably as $f_e$ or $f_{ij}$. Note that the power flow on a given line is negative if the current flows in the opposite direction with respect to the edge orientation; therefore, with a minor abuse of notation we have $f_e=f_{ij}=-f_{ji}$.

The power flows on the lines are uniquely determined by the injections and physical properties of the network. More specifically, denoting by $f \in \R^m$ the power flow vector, the DC power flow model can be written as
\begin{equation}
\label{eqn:dc_model}
	f =BC^T L^+ p.
\end{equation}
The slack bus phase angle in $\theta$ is typically set to $0$ as a reference to other buses. With this convention, the DC model \eqref{eqn:dc_model} has a unique solution $\theta$ and $f$ for each balanced injection vector $p$.

%\begin{figure}
%\centering
%\includegraphics[width=.275\textwidth]{spanning_forest.png}
%\caption{An example element in $\calT(\calV_1,\calV_2)$, where circles correspond to elements in $\calV_1$ and squares correspond to elements in $\calV_2$. The two trees containing $\calV_1$ and $\calV_2$ are highlighted as solid lines.}\label{fig:spanning_forest}
%\end{figure}

Therefore, differently from many other man-made networks, the network operator does not directly control the power flows routing, but we can only indirectly change them by modifying the power injections or the network topology. This peculiar feature is one of the reason why is particularly challenging to study and improve the reliability of power systems and their robustness against failures. Indeed, when a subset of lines $\calE$ is tripped or fails, the network topology changes and, as a consequence, the power flow redistributes on the surviving graph $G'=(V,E\bs\calE)$, possibly causing overloads in other lines, not necessarily adjacent to the removed ones in $\calE$. 

If the power injections are still balanced for $G'$, the new power flows can be calculated directly from~\eqref{eqn:dc_model} after having updated the matrices $B$, $C$, and $L$. If the removal of the lines in $\calE$ created a new island, then the network operator has to intervene and modify some of the power injections to ensure that they are balanced again.

%In the case of the failure of a single line, i.e. $\calE=\{e\}$, if $G'$ is still connected, then the branch flow change on any other line $\widetilde{e} \neq e$ is given as
%$$
%	\Delta f_{\hat{e}} = f_e \cdot K_{e\widetilde{e}},
%$$
%where $K_{e\widetilde{e}}$ is the \emph{line outage distribution factor} \cite{Wood1996} from $e$ to $\widetilde{e}$ \lguo{Do we want to do cut set and non-cut set failure here instead since $\calE$ is a set of edges? See part II of the TPS paper for the full theory in this case} \alec{Yes!}. It is known that the line outage distribution factors are independent of the original power injections $p$ and depend only on the network topology; in fact, they can be computed from the matrices $B$ and $C$ as showed in~\cite{Wood1996}.
%\alec{Need to explain cascade mechanism here and typical non-local failure propagation}
